A Mechanistic View on Video Generation as World Models: State and Dynamics

Large-scale video generation models have demonstrated emergent physical coherence, positioning them as potential world models. However, a gap remains between contemporary "stateless" video architectures and classic state-centric world model theories. This work bridges this gap by proposing a novel taxonomy centered on two pillars: State Construction and Dynamics Modeling. We categorize state construction into implicit paradigms (context management) and explicit paradigms (latent compression), while dynamics modeling is analyzed through knowledge integration and architectural reformulation. Furthermore, we advocate for a transition in evaluation from visual fidelity to functional benchmarks, testing physical persistence and causal reasoning. We conclude by identifying two critical frontiers: enhancing persistence via data-driven memory and compressed fidelity, and advancing causality through latent factor decoupling and reasoning-prior integration. By addressing these challenges, the field can evolve from generating visually plausible videos to building robust, general-purpose world simulators.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> legacy/1_intro.tex <==
\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: 加一个intuitve example of memory in human brain comparable to such in video generation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Recent advances in \textbf{video generation models} have demonstrated remarkable progress across a wide range of domains, including digital content creation, visual storytelling, and simulation. 
These models have evolved from generating short, scene-specific clips to producing \textit{streaming, long-duration videos} with increasing temporal coherence and semantic richness. 
As video generation progresses toward longer horizons and more complex dynamics, maintaining consistent and adaptive information over time has become a central challenge.

Within this development trend, \textbf{memory} has emerged as a key component and underlying mechanism for next-generation video generation systems. 
At its core, memory can be broadly defined as the ability to \textit{store}, \textit{retain}, and \textit{recall} information across time. 
These three operations can be regarded as \textit{orthogonal dimensions of information management}: 
\textbf{Store (storage dimension)} concerns how information is represented and compressed to reduce storage cost and redundancy. 
\textbf{Recall (informational dimension)} focuses on how the system selectively retrieves the most relevant information for the current context. 
\textbf{Retain (temporal dimension)} refers to how memory is maintained, updated, or forgotten over time to ensure temporal coherence and adaptability.

From this perspective, memory serves as a \textit{multi-dimensional mechanism} balancing storage efficiency, informational relevance, and temporal persistence. 
In neuroscience, human memory refers to the brain’s ability to store, retain, and recall information~\cite{sherwood2004human}. 
It serves as the foundation for understanding the world, learning new knowledge, adapting to the environment, and making decisions, allowing humans to preserve past experiences, skills, and knowledge, which shape personal identity and behavioral patterns. 
In the era of large language models (LLMs), an analogous concept has re-emerged in \textbf{LLM-powered autonomous agents}, where memory plays a crucial role in extending the model’s contextual reasoning ability. 
In this setting, memory can be defined as the process of acquiring, storing, retaining, and subsequently retrieving information~\cite{wu2025human}. 
It enables LLM-based systems to overcome the inherent limitation of finite context windows, allowing agents to recall interaction history and make more coherent and intelligent decisions.

A similar concept is now becoming indispensable in \textbf{video generation}, where the model must continuously track, recall, and update visual information during the generative process. 
In current video generation applications, memory plays crucial roles across multiple dimensions:
\begin{itemize}
    \item \textbf{Visual Reasoner} ---  
    \item \textbf{Visual Render} ---
\end{itemize}

Despite its growing importance, our understanding of \textbf{memory mechanisms in video generation} remains limited. 
Most existing studies emphasize the \textit{storage perspective} of memory --- such as compression and efficiency --- while paying less attention to the \textit{informational perspective} (how to effectively utilize stored information) and the \textit{temporal perspective} (how to manage and update memory over time). 
Furthermore, certain scene generation tasks~\cite{} employ \textit{explicit geometric memory} (e.g., 3D point clouds or Gaussian splatting) to maintain spatial consistency. 
Although such methods naturally align with the functional goal of memory, they often treat the video model as a reconstruction or inpainting tool --- \textit{reversing the intended relationship} where memory should serve the video generation process, not define it. 
Consequently, these approaches often limit the model’s temporal dynamics, leading to static or frame-independent results. 
Our goal is to establish a general and comprehensive perspective on the forms and mechanisms of memory, and to explore how such mechanisms can more effectively support the development of next-generation video generation models.

To address these limitations, this survey aims to provide a \textbf{systematic overview and rethinking of memory in video generation}. 
In summary, the main contributions of this work are threefold:
\begin{itemize}
    \item \textit{First}, we conduct a comprehensive review of how memory is currently integrated into video generation models.
    \item \textit{Second}, we propose a multi-perspective classification of memory --- spanning structural, functional, and temporal dimensions --- closely aligned with the latest advances in video model development.
    \item \textit{Third}, we provide a forward-looking discussion on how memory mechanisms may evolve alongside the future identity of video generation models, envisioning a more general and unified framework for memory management.
\end{itemize}

The rest of this survey is organized as follows. 
Section~\ref{Background} introduces the paradigm development of video generation. 
Section~\ref{Memory Definition} discusses the role and definition of memory under the current paradigm of video generation models. 
Section~\ref{Memory from Different Perspective} examines how memory has been studied from different perspectives and summarizes the current stage of research progress.


==> legacy/1_intro_v2.tex <==
% \IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
\section{Introduction}
\label{sec:introduction}

% ------------------------------------------------------------------
% 1. The Rise of Video Generation & Potential as World Models
% ------------------------------------------------------------------
\IEEEPARstart{T}{he} field of video generation has witnessed a paradigm shift in recent years. 
Driven by the development of large-scale video diffusion transformer models \cite{gupta2024photorealistic,lu2023vdt,ma2024latte,fan2025vchitect,liu2025lumina,zhang2025waver,wan2025wan,chen2025skyreels,ma2025step,agarwal2025cosmos,hacohen2024ltx,kong2024hunyuanvideo,genmo2025blog,openai2024sora,lin2024open,zheng2024open,yang2024cogvideox,BarTal2024LumiereAS,Chen2023SEINESV,veo2025,kuaishou2024klingai,gao2025seedance,hailuoai2025,Bruce2024GenieGI,pikalabs2024pika}, the capability of generative models has evolved from producing short, low-resolution clips to rendering cinematic-quality sequences with unprecedented temporal consistency. Leading models such as Sora~\cite{openai2024sora}, Gen-3~\cite{runway2024gen3}, Veo~\cite{veo2025}, Wan~\cite{wan2025wan} and Kling~\cite{kuaishou2024klingai} have demonstrated implications that extend far beyond mere visual fidelity. 
These models exhibit emergent physical coherence. For example, they learned how to respect gravity, collision dynamics, and object permanence without explicit physical instruction. 
This capability to simulate coherent dynamics has led the research community to increasingly evaluate video generation models not merely as content creators, but as potential \textbf{world models}~\cite{openai2024sora,hu2023gaia,veo2025,du2023learning huang2025towards,li2025worldmodelbench,kang2024far,ren2025videoworld}.

% ------------------------------------------------------------------
% 2. Theoretical Definition: From MBRL to General Simulation
% ------------------------------------------------------------------
To critically assess this potential, it is necessary to revisit the theoretical origins of the concept of world model.
The term ``world model'' has its roots in cognitive science, specifically in the theory of mental models~\cite{craik1943nature, gentner2014mental, johnson1983mental}.
These works posited that intelligent organisms maintain a  ``small-scale model'' of external reality to anticipate events, reason about counterfactuals, and simulate consequences before action. 
In the domain of Artificial Intelligence, this concept was first formalized by Model-Based Reinforcement Learning (MBRL)~\cite{forrester1971counterintuitive, ha2018world, ha2018recurrent, hafner2019learning, hafner2020mastering, hafner2023mastering, hafner2025training, mnih2015human,mnih2016asynchronous, barth2018distributed, schrittwieser2020mastering, oh2017value, silver2017predictron, hansen2022temporal, hansen2023td, lee2023dreamsmooth, mattes2023hieros, liu2025continual, prasanna2024dreaming, hao2025neural}, such as Recurrent World Models~\cite{ha2018recurrent} and the Dreamer series~\cite{hafner2019learning, hafner2020mastering, hafner2023mastering, hafner2025training}. 
In these settings, the world model is inextricably coupled with a policy agent in a closed-loop interaction: the model captures environmental laws to allow the agent to ``dream'' or practice in a virtual space before real-world execution.


% ------------------------------------------------------------------
% 3. The Shift to Open-Loop Video World Models
% ------------------------------------------------------------------
However, the rise of large-scale video generation marks a significant paradigm shift. Unlike MBRL, video models typically bypass explicit reinforcement learning and active agent interaction.
Instead, they operate in an open-loop setting, learning to simulate complex dynamics through the passive observation of vast datasets.
Recent evidence~\cite{ha2018world, huang2025towards,li2025worldmodelbench,kang2024far,ren2025videoworld} suggests that this observational learning is surprisingly potent which indicates that developing a world model is not strictly contingent on active exploration. 
By merely ``watching'' sufficient video data, a model can internalize underlying physics and causal intuitions.
Consequently, this survey focuses on open-loop world models—systems trained on large-scale video data without the explicit reinforcement learning components (such as reward functions or policy models) found in MBRL.

Theoretically, a world model comprises two fundamental components: (1) a \textit{state estimation model} that abstracts high-dimensional historical observations into a latent state space to ``perceive'' the world, and (2) a \textit{dynamics prediction model} that evolves these states to ``simulate'' the future. Ideally, the latent state $S_t$ serves as a \textbf{sufficient statistic} of the entire historical context \cite{ha2018recurrent, hafner2019learning, lecun2022path}. 

Crucially, this formulation enforces a \textbf{Markovian property}, where the future evolution of the world depends solely on the current latent state $S_t$ rather than the exhaustive history of raw observations. 
To achieve this, the state estimation process~\cite{ha2018world,ha2018recurrent,hafner2019learning,hafner2020mastering,hafner2023mastering,hafner2025training} must effectively aggregate temporal cues, such as velocity, acceleration, and object permanence.
Thus, $S_t$ encapsulates not just a static snapshot, but the underlying governing dynamics of the environment.

% ------------------------------------------------------------------
% 4. The "Stateless" Bottleneck in Current Architectures
% ------------------------------------------------------------------
Nevertheless, a notable discrepancy persists between this theoretical ideal and prevailing engineering paradigms. 
Despite the conceptual requirement for state-centric abstraction, contemporary Transformer-based video models capable of long-horizon autoregressive generation remain fundamentally stateless~\cite{huang2025self, yin2025causvid, lin2025autoregressive, gao2024ca2, chen2024diffusion, weng2024art, yuan2025lumos, deng2024autoregressive, kondratyuk2023videopoet, gu2025long, zhuang2025video, yu2025videomar, deng2024nova, teng2025magi, sun2025ardiff, liu2025rolling, cui2025self}. 
Instead of maintaining a compact state variable, they typically rely on attending to the full historical observation at each step to predict the future observation. 
While this design has proven highly effective for short horizons, the lack of explicit persistence (e.g., a global state) creates fundamental bottlenecks as models scale to longer durations, such as computational issue and memory issue.


% ------------------------------------------------------------------
% 5. Emergence of State & Survey Goal
% ------------------------------------------------------------------
To address these challenges, recent advancements in the field have, whether implicitly or explicitly, converged on recapturing the fundamental concept of ``state'' within video models.
For example, Memory Mechanisms~\cite{mempack2025, worldpack2025, corgi2025, guo2025ctrlworld, ragme2025, motionrag2025,xiao2025worldmem, yu2025context,chen2025learning, song2025ditmem, an2025onestory}, Causal Linear Systems~\cite{chen2025sana, wang2025lingen, po2025long, yu2025videossm, oshima2024ssm, chen2025recurrent} function as prototypes of ``state,'' forcing video models to maintain an internal, persistent representation of the past. 
These explorations can not only resolve computational bottlenecks but also will align these models with the theoretical framework of world models, thereby enhancing their utility as simulation systems.
This survey aims to systematically organize \textbf{how the abstract concept of state in theoretical world models corresponds to the emerging engineering solutions in modern video generation}.

% ------------------------------------------------------------------
% 6. Contributions
% ------------------------------------------------------------------
Our core contributions are three-fold:

\begin{itemize}
\item \textbf{From Video Model to World Model:} We bridge the gap between high-level theory and implementation. Starting from the definition of a complete world model, we narrow our focus to the video generation context, proposing that an \textit{open-loop, state-centric system} represents the minimum viable unit of a world model. Based on this, we evaluate the potential of current video models to serve as world simulators.

\item \textbf{State-Centric Taxonomy:} We propose a novel taxonomy based on the \textbf{Construction of State}. We categorize existing literature into two paradigms: \textit{Implicit State}, where history is managed via context windows (e.g., KV Cache), and \textit{Explicit State}, where history is compressed into compact variables akin to traditional state-space models.

\item \textbf{Critical Insight \& Future Directions:} We analyze the structural trade-offs of current paradigms, identifying the absence of compact state representation as the primary barrier to long-horizon simulation. Furthermore, we posit that while current progress is driven by passive learning from datasets (open-loop), the ultimate trajectory must transition to active agent-environment interaction (closed-loop) to overcome the distribution bias of passive data, paving the way for embodied general intelligence.

\end{itemize}

==> legacy/2_background.tex <==
\section{Background}\label{Background}

\subsection{Video Generation Models}

After the release of Sora~\cite{openai2024sora}, the field of video generation has been dominated by models built upon Diffusion Transformers (DiT) equipped with bidirectional attention~\cite{zhang2025waver,wan2025wan,kong2024hunyuanvideo,agarwal2025cosmos,genmo2025blog,lin2024open,zheng2024open,yang2024cogvideox}.
These models typically generate short video clips (around 5 seconds) in a one-shot manner, where text prompts are encoded through a text encoder and serve as conditioning signals for visual token generation via either cross- or self-attention. During training, the visual modality is first compressed into a latent space using a 3D VAE, which usually applies a 4× temporal and 8× spatial downsampling.

This paradigm achieves remarkable text–video alignment and high visual fidelity, reaching state-of-the-art results across multiple benchmarks.  
However, when extended to longer video generation, these models face a notable training–inference gap. To mitigate this issue, various techniques—such as extendable RoPE, sliding windows, or FIFO-based inference strategies—have been introduced to enable long-horizon or even infinite video synthesis.  
Nevertheless, the bidirectional attention mechanism inherently limits the context window, which mainly serves to maintain local consistency between already-generated and currently noised content. As a result, these models lack a mechanism for managing global context across extended sequences.

A parallel line of research explores \textbf{auto-regressive diffusion models} for video generation~\cite{sun2025ardiff,teng2025magi,yu2025videomar,zhuang2025video,gu2025long,lin2025autoregressive,kondratyuk2023videopoet,deng2024autoregressive,yuan2025lumos,weng2024art,chen2024diffusion}.
These approaches incorporate causal attention masks and train the model to condition on clean (low-noise) tokens as additional context. Consequently, the model learns to leverage information from previously denoised frames, enabling multi-round and temporally coherent video synthesis.

However, this design converts generation into a chunk-level autoregressive process, which substantially shortens the effective temporal span of each iteration. Thus, generating long videos requires multiple inference rounds, making the process susceptible to accumulated errors and exposure bias.

More recently, several works have distilled bidirectional diffusion transformers into few-step causal models to achieve real-time video generation~\cite{yin2024onestep,yin2024improved,yin2025causvid}.
To further alleviate exposure bias, Self-Forcing~\cite{huang2025self} employs self-generated content as context during training, bridging the train–inference gap inherent in teacher-forcing paradigms.
Such advancements open new possibilities for real-time and interactive video generation, extending beyond conventional offline synthesis.


\subsection{Formulation of World Model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: 加一个类似于xmind的树状图
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This role of video generation model provides a natural bridge to the concept of a \textbf{World Model}. In this survey, we adapt the classic formulation~\cite{ha2018world, bardes2023v, assran2025v, huang2025towards} of a world model, which is traditionally defined as:

\begin{equation}
S_{t+1} = F(S_t, A_t, O_t),
\label{eq:classic_wm}
\end{equation}

where $S_t$ is the internal state of the world at time $t$, $A_t$ is the current action or control signal, and $O_t$ is the external observation from the environment. Within this context, world models are typically classified into two major categories:

\begin{enumerate}
    \item \textbf{Representation World Models:} These models aim to learn state transitions in an \textit{abstract semantic space}. The state $S_t$ is an abstract encoding of the observation $O_t$ (e.g., $S_t = \text{Encoder}(O_t)$). A critical \textbf{semantic gap} exists between the concrete observation $O_t$ (e.g., pixels) and the abstract state $S_t$. In this paradigm, $O_t$ is indispensable as the bridge connecting the external world to the internal abstract representation.
    \item \textbf{Generative (or Simulation-based) World Models:} These models possess generative capabilities and can "simulate" or reconstruct the world's state in a \textit{concrete representation space} (e.g., pixel or latent space).
\end{enumerate}

This distinction is paramount. As we have discussed, modern video generative models (e.g., Sora, Gen-3) function primarily as "generative engines." They operate in a \textbf{"self-evolving"} or autoregressive manner, where the model's primary interaction is with its own generated content, not a continuous stream of new external observations $O_t$.

This self-evolving property leads to a fundamental shift in the formulation.

First, the external \textbf{observation $O_t$ is effectively internalized}. The model's own output at $t-1$ \textit{becomes} the observation for predicting step $t$. The distinction between the internal state and the external observation collapses, as both exist within the same concrete representation space.

Second, the definition of \textbf{state $S_t$ evolves}. In a self-evolving generative model (like a Transformer), the state required to predict the future is no longer an instantaneous abstract vector. Instead, the effective state $S_t$ can be defined as the \textbf{entire accumulated history of concrete representations} (e.g., the sequence of all past frames or tokens, $[s_0, ..., s_t]$) that the model conditions on.

This definition of "state" as the \textit{accumulated historical context} is functionally equivalent to what we define as \textbf{Memory ($M_t$)}. Therefore, for the Generative World Model (GWM) paradigm, we can assert that \textbf{State is Memory ($S_t \equiv M_t$)}.

This insight allows us to simplify and adapt the classic world model definition (Eq. \ref{eq:classic_wm}). By internalizing $O_t$ and equating $S_t$ with $M_t$, we arrive at a formulation tailored for GWMs:

\begin{equation}
M_{t+1} = F(M_t, A_t),
\label{eq:gwm}
\end{equation}

This reformulation reframes the challenge of building a GWM: the core task becomes the design of the function $F$, which is fundamentally a \textbf{Memory Mechanism} responsible for managing and evolving the complete historical context.

To further formalize this, we decompose the function $F$ not as a monolithic block, but as a \textbf{unified cognitive cycle} composed of five key modules. This framework provides maximum flexibility by treating the control signal $A_t$ as an optional input $[A_t]$ to most stages, and the $D$ and $E$ modules as optional $[D], [E]$ processing steps.

The module signatures are defined as follows:
\begin{itemize}
    \item \textbf{Retrieval (R):} $R_t = R(M_t, [A_t])$
    \item \textbf{Decoding (D):} $D_t = [D](R_t, [A_t])$
    \item \textbf{Generation (G):} $G_t = G(D_t, A_t)$
    \item \textbf{Encoding (E):} $E_t = [E](G_t, [A_t])$
    \item \textbf{Update (U):} $M_{t+1} = U(M_t, E_t, [A_t])$
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: 加一个flow图，体现R->D->G->E->U process
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This formulation (Eq. \ref{eq:gwm}) defines the "what"—a system that evolves memory. The R-D-G-E-U decomposition defines the "how"—a cognitive cycle of \textit{retrieving} from the past, \textit{generating} the future, and \textit{updating} the memory to integrate this new "imagined" experience. This cycle provides a comprehensive blueprint for building and analyzing advanced, long-horizon generative world models.


% 从这个公式出发，我们可以观察视频生成模型 G的输入是当下的记忆状态Mt信息和action At信息，那么目前应用层面上大家有不同的侧重点：
video generative models can play two distinct roles: 
(1) as \textbf{predictive models} that reason about future dynamics based on contextual memory, and (2) as \textbf{generative engines} that respond to external control signals to produce visually coherent outputs.




\subsection{Video Generation Models as Visual Reasoner}

A \textbf{visual reasoner} can be defined as a predictive model that reasons about \textit{future dynamics} based on observed content.

Recent studies, such as CoF~\cite{wiedemer2025video}, show that large video models have begun to exhibit such reasoning capabilities.
For instance, Veo 3~\cite{veo2025} demonstrates emergent abilities such as object segmentation, edge detection, image editing, physical property inference, affordance understanding, and even tool-use simulation—all without explicit supervision.
These abilities to \textit{perceive}, \textit{model}, and \textit{manipulate} the visual world reflect early forms of visual reasoning, including maze solving and symmetry understanding.
Such zero-shot generalization suggests that video models are evolving toward unified, generalist vision foundation models.

Despite this progress, current video generation models~\cite{openai2024sora,zhang2025waver,wan2025wan,kong2024hunyuanvideo,agarwal2025cosmos,genmo2025blog,lin2024open,zheng2024open,yang2024cogvideox} still exhibit only \textbf{primitive reasoning ability}.
True predictive reasoning requires a \textbf{causal attention mechanism} that explicitly encodes temporal dependencies from past to future.
However, most diffusion-based architectures rely on \textbf{bidirectional attention}, which conflicts with the unidirectional causality inherent in prediction.
Moreover, these models are heavily dependent on \textbf{text prompts} as high-level control signals, making them more like \textit{video generators} guided by text rather than genuine \textit{future predictors}.
Consequently, they tend to preserve \textbf{appearance continuity} rather than perform authentic \textbf{dynamic reasoning} about motion or physical causality.

In the extreme case, a visual reasoner requires only a \textbf{memory $M_t$} that accurately stores observed content and evolving scene dynamics.
Such memory acts as a persistent representation of perception, providing the model with sufficient visual context to understand ongoing phenomena and infer plausible futures.
Here, memory is not merely a cache of past frames but a structured, semantically grounded space that supports reasoning, prediction, and adaptation to future events.


\subsection{Video Generation Models as Visual Renderer}

A \textbf{visual renderer} can be defined as a generative engine (or an implicit simulator) that responds to external control signals to produce visually coherent outputs.
Most current text-conditioned video generation models can be interpreted as visual renderers, where textual descriptions serve as high-level control signals guiding the synthesis of spatiotemporal content.

However, such coarse-grained control introduces several challenges:
(1) \textbf{Temporal under-specification:} a single text token may correspond to dozens of frames, leaving fine-grained temporal dynamics ambiguous;
(2) \textbf{Static–dynamic gap:} textual descriptions are inherently static, while videos evolve continuously over time;
(3) \textbf{One-to-many mapping:} identical text conditions (e.g., “a man runs”) may correspond to distinct trajectories that differ in speed, path, or duration.

Consequently, the text-based control signal is often \textbf{too coarse} to precisely guide state transitions, leading the model to approximate state matching rather than achieve explicit state control.
Moreover, existing training paradigms introduce alignment limitations:
\begin{itemize}
\item \textbf{Weak temporal alignment:} video–text pairs are aligned at the clip level, lacking frame-level synchronization;
\item \textbf{Semantic ambiguity:} text cannot accurately encode continuous motion attributes such as velocity or trajectory;
\item \textbf{Sparse control intervention:} control signals are typically injected only at sampling initialization, preventing dynamic adjustment during generation.
\end{itemize}

Recent works have explored incorporating additional control modalities beyond text~\cite{zhang2023adding,tan2025ominicontrol,hu2022lora,ju2025fulldit,gu2025diffusion,ye2023ip,mou2024t2i,yu2025gamefactory,he2024cameractrl,wang2024motionctrl},
including identity preservation, camera motion, and interactive inputs (e.g., keyboard or mouse signals).
As the granularity and precision of control signals increase, the model’s reliance on implicit knowledge decreases, and the generation process becomes increasingly similar to a \textbf{state transition system} governed by explicit actions.

In the extreme case, the model only requires actions as input—functionally analogous to a rule-based simulator.

==> legacy/2_background_v2.tex <==
\section{Background}\label{Background}

\subsection{Video Generation Models}

After the release of Sora~\cite{openai2024sora}, the field of video generation has been dominated by models built upon Diffusion Transformers (DiT) equipped with bidirectional attention~\cite{zhang2025waver,wan2025wan,kong2024hunyuanvideo,agarwal2025cosmos,genmo2025blog,lin2024open,zheng2024open,yang2024cogvideox}. 
These models typically generate short video clips (around 5 seconds) in a one-shot manner: text prompts are encoded by a text encoder and used as conditioning signals for visual token generation via cross- or self-attention. 
During training, the visual modality is first compressed into a latent space using a 3D VAE, which usually applies a 4$\times$ temporal and 8$\times$ spatial downsampling.

This paradigm achieves remarkable text–video alignment and high visual fidelity, reaching state-of-the-art results across multiple benchmarks.  
However, when extended to longer video generation, these models face a notable training–inference gap. 
To mitigate this issue, various techniques—such as extendable RoPE, sliding windows, or FIFO-based inference strategies—have been introduced to enable long-horizon or even infinite video synthesis.  
Nevertheless, the bidirectional attention mechanism inherently limits the effective context window, which mainly serves to maintain local consistency between already-generated and currently noised content. 
As a result, these models lack an explicit mechanism for managing global context across extended sequences.

A parallel line of research explores \textbf{auto-regressive diffusion models} for video generation~\cite{sun2025ardiff,teng2025magi,yu2025videomar,zhuang2025video,gu2025long,lin2025autoregressive,kondratyuk2023videopoet,deng2024autoregressive,yuan2025lumos,weng2024art,chen2024diffusion}. 
These approaches incorporate causal attention masks and train the model to condition on clean (low-noise) tokens as additional context. 
Consequently, the model learns to leverage information from previously denoised frames, enabling multi-round and temporally coherent video synthesis.

However, this design converts generation into a chunk-level autoregressive process, which substantially shortens the effective temporal span of each iteration. 
Thus, generating long videos requires multiple inference rounds, making the process susceptible to accumulated errors and exposure bias.

More recently, several works have distilled bidirectional diffusion transformers into few-step causal models to achieve real-time video generation~\cite{yin2024onestep,yin2024improved,yin2025causvid}. 
To further alleviate exposure bias, Self-Forcing~\cite{huang2025self} employs self-generated content as context during training, bridging the train–inference gap inherent in teacher-forcing paradigms.
Such advancements open new possibilities for real-time and interactive video generation, extending beyond conventional offline synthesis.


\subsection{From Video Generators to World Models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: 加一个类似于xmind的树状图
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The emerging role of video generation models naturally connects to the classical notion of a \textbf{world model}. 
We adopt the standard formulation~\cite{ha2018world,bardes2023v,assran2025v,huang2025towards}, in which a world model is defined as
\begin{equation}
S_{t+1} = F(S_t, A_t, O_t),
\label{eq:classic_wm}
\end{equation}
where $S_t$ denotes the internal state of the world at time $t$, $A_t$ is the current action or control signal, and $O_t$ is the external observation from the environment.

Within this formulation, world models are typically grouped into two major categories:
\begin{enumerate}
    \item \textbf{Representation World Models}, which aim to learn state transitions in an \emph{abstract semantic space}. 
    The state $S_t$ is an abstract encoding of the observation $O_t$ (e.g., $S_t = \text{Encoder}(O_t)$), and a semantic gap exists between concrete observations (pixels) and abstract states. 
    Here, $O_t$ is indispensable as the bridge between the external world and the internal representation.
    \item \textbf{Generative (or Simulation-based) World Models}, which possess generative capabilities and can ``simulate'' or reconstruct the world state in a \emph{concrete representation space} (e.g., image or latent space).
\end{enumerate}

This distinction is crucial for modern video generators. 
Large-scale video diffusion models (e.g., Sora, Gen-3) function primarily as \emph{generative engines}: they operate in a \textbf{self-evolving} or autoregressive manner, where the primary interaction is with their own generated content rather than a continuous stream of external observations $O_t$.

This self-evolving property leads to a fundamental shift in the formulation.
First, the external observation $O_t$ is effectively \emph{internalized}: the model's own output at $t-1$ becomes the observation for predicting step $t$. 
The distinction between internal state and external observation collapses, as both live in the same concrete representation space.
Second, the notion of state $S_t$ evolves. 
In a self-evolving generative model (e.g., a Transformer with a context window), the effective state is no longer an instantaneous abstract vector but the \emph{accumulated historical context} (e.g., all past frames or tokens $[s_0, \dots, s_t]$) that the model conditions on.

Functionally, this accumulated context is precisely what we call \textbf{memory} and denote by $M_t$. 
For generative world models, it is therefore natural to assert that \textbf{state is memory} ($S_t \equiv M_t$), and to rewrite Eq.~\eqref{eq:classic_wm} as
\begin{equation}
M_{t+1} = F(M_t, A_t),
\label{eq:gwm}
\end{equation}
where $M_t$ is the memory state and $A_t$ is an optional control signal.

In the remainder of this survey we adopt Eq.~\eqref{eq:gwm} as our working formulation for long-horizon video generation. 
Under this view, the behaviour of a video model is entirely determined by how it uses its memory state $M_t$ together with the control signal $A_t$. 
This gives rise to two complementary operational roles:

\begin{itemize}
    \item a \emph{predictive} role, where the model acts as a \textbf{visual reasoner} that forecasts future dynamics based on $M_t$;
    \item a \emph{controlled generative} role, where the model acts as a \textbf{visual renderer} that maps actions $A_t$ and memory $M_t$ to visually coherent outputs.
\end{itemize}

We next discuss these two roles, before turning Eq.~\eqref{eq:gwm} into an operational definition of memory in Section~\ref{sec:memory-definition}.



\subsection{Video Generation Models as Visual Reasoners}

Given the generative world-model formulation in Eq.~\eqref{eq:gwm}, one natural way to interpret a video model is as a \textbf{visual reasoner}: 
a predictive system that estimates future dynamics based on its current memory state $M_t$ (and possibly control $A_t$).
Here, the emphasis is on modeling $p(\text{future}\mid M_t, A_t)$ and using memory as a persistent representation of what has been perceived so far.

Recent studies, such as CoF~\cite{wiedemer2025video}, show that large video models have begun to exhibit such reasoning capabilities.
For instance, Veo~3~\cite{veo2025} demonstrates emergent abilities such as object segmentation, edge detection, image editing, physical property inference, affordance understanding, and even tool-use simulation—all without explicit supervision.
These abilities to \emph{perceive}, \emph{model}, and \emph{manipulate} the visual world reflect early forms of visual reasoning, including maze solving and symmetry understanding.
Such zero-shot generalization suggests that video models are evolving toward unified, generalist vision foundation models.

Despite this progress, current video generation models~\cite{openai2024sora,zhang2025waver,wan2025wan,kong2024hunyuanvideo,agarwal2025cosmos,genmo2025blog,lin2024open,zheng2024open,yang2024cogvideox} still exhibit only \textbf{primitive reasoning ability}.
True predictive reasoning requires a \textbf{causal attention mechanism} that explicitly encodes temporal dependencies from past to future. 
However, most diffusion-based architectures rely on \textbf{bidirectional attention}, which conflicts with the unidirectional causality inherent in prediction.
Moreover, these models are heavily dependent on \textbf{text prompts} as high-level control signals, making them more like \emph{video generators} guided by text rather than genuine \emph{future predictors}. 
Consequently, they tend to preserve \textbf{appearance continuity} rather than perform authentic \textbf{dynamic reasoning} about motion or physical causality.

In the limiting case, a visual reasoner requires only a \textbf{memory state $M_t$} that accurately stores observed content and evolving scene dynamics. 
Such memory acts as a persistent representation of perception, providing the model with sufficient visual context to understand ongoing phenomena and infer plausible futures. 
Here, memory is not merely a cache of past frames but a structured, semantically grounded space that supports reasoning, prediction, and adaptation.


\subsection{Video Generation Models as Visual Renderers}

A complementary role is that of a \textbf{visual renderer}: a generative engine (or implicit simulator) that responds to external control signals to produce visually coherent outputs.
Most current text-conditioned video generation models can be interpreted as visual renderers, where textual descriptions serve as high-level control signals guiding the synthesis of spatiotemporal content.

However, such coarse-grained control introduces several challenges:
\begin{itemize}
    \item \textbf{Temporal under-specification}: a single text token may correspond to dozens of frames, leaving fine-grained temporal dynamics ambiguous;
    \item \textbf{Static–dynamic gap}: textual descriptions are inherently static, while videos evolve continuously over time;
    \item \textbf{One-to-many mapping}: identical text conditions (e.g., ``a man runs'') may correspond to distinct trajectories that differ in speed, path, or duration.
\end{itemize}

Consequently, the text-based control signal is often \textbf{too coarse} to precisely guide state transitions, leading the model to approximate state matching rather than achieve explicit state control.
Moreover, existing training paradigms introduce alignment limitations:
\begin{itemize}
    \item \textbf{Weak temporal alignment}: video–text pairs are aligned at the clip level, lacking frame-level synchronization;
    \item \textbf{Semantic ambiguity}: text cannot accurately encode continuous motion attributes such as velocity or trajectory;
    \item \textbf{Sparse control intervention}: control signals are typically injected only at sampling initialization, preventing dynamic adjustment during generation.
\end{itemize}

Recent works have explored incorporating additional control modalities beyond text~\cite{zhang2023adding,tan2025ominicontrol,hu2022lora,ju2025fulldit,gu2025diffusion,ye2023ip,mou2024t2i,yu2025gamefactory,he2024cameractrl,wang2024motionctrl},
including identity preservation, camera motion, and interactive inputs (e.g., keyboard or mouse signals).
As the granularity and precision of control signals increase, the model’s reliance on implicit knowledge decreases, and the generation process becomes increasingly similar to a \textbf{state transition system} governed by explicit actions.

In the remainder of this survey we adopt Eq.~\eqref{eq:gwm} as our working formulation for long-horizon video generation. 
Under this view, the behaviour of a video model is entirely determined by how it uses its memory state $M_t$ together with the control signal $A_t$. 
This gives rise to two complementary operational roles:

\begin{itemize}
    \item a \emph{predictive} role, where the model acts as a \textbf{visual reasoner} that forecasts future dynamics based on $M_t$;
    \item a \emph{controlled generative} role, where the model acts as a \textbf{visual renderer} that maps actions $A_t$ and memory $M_t$ to visually coherent outputs.
\end{itemize}

We next discuss these two roles, before turning Eq.~\eqref{eq:gwm} into an operational definition of memory in Section~\ref{sec:memory-definition}.



==> legacy/2_background_v3.tex <==
\section{Background}\label{Background}

\subsection{Video Generation Models}

After the release of Sora~\cite{openai2024sora}, the field of video generation has been dominated by models built upon Diffusion Transformers (DiT) equipped with bidirectional attention~\cite{zhang2025waver,wan2025wan,kong2024hunyuanvideo,agarwal2025cosmos,genmo2025blog,lin2024open,zheng2024open,yang2024cogvideox}. 
These models typically generate short video clips (around 5 seconds) in a one-shot manner: text prompts are encoded by a text encoder and used as conditioning signals for visual token generation via cross- or self-attention. 
During training, the visual modality is first compressed into a latent space using a 3D VAE, which usually applies a 4$\times$ temporal and 8$\times$ spatial downsampling.

This paradigm achieves remarkable text–video alignment and high visual fidelity, reaching state-of-the-art results across multiple benchmarks.  
However, when extended to longer video generation, these models face a notable training–inference gap. 
To mitigate this issue, various techniques—such as extendable RoPE, sliding windows, or FIFO-based inference strategies—have been introduced to enable long-horizon or even infinite video synthesis.  
Nevertheless, the bidirectional attention mechanism inherently limits the effective context window, which mainly serves to maintain local consistency between already-generated and currently noised content. 
As a result, these models lack an explicit mechanism for managing global context across extended sequences.

A parallel line of research explores \textbf{auto-regressive diffusion models} for video generation~\cite{sun2025ardiff,teng2025magi,yu2025videomar,zhuang2025video,gu2025long,lin2025autoregressive,kondratyuk2023videopoet,deng2024autoregressive,yuan2025lumos,weng2024art,chen2024diffusion}. 
These approaches incorporate causal attention masks and train the model to condition on clean (low-noise) tokens as additional context. 
Consequently, the model learns to leverage information from previously denoised frames, enabling multi-round and temporally coherent video synthesis.

However, this design converts generation into a chunk-level autoregressive process, which substantially shortens the effective temporal span of each iteration. 
Thus, generating long videos requires multiple inference rounds, making the process susceptible to accumulated errors and exposure bias.

More recently, several works have distilled bidirectional diffusion transformers into few-step causal models to achieve real-time video generation~\cite{yin2024onestep,yin2024improved,yin2025causvid}. 
To further alleviate exposure bias, Self-Forcing~\cite{huang2025self} employs self-generated content as context during training, bridging the train–inference gap inherent in teacher-forcing paradigms.
Such advancements open new possibilities for real-time and interactive video generation, extending beyond conventional offline synthesis.

\subsection{World Model}
fill with paper with world models






==> legacy/2_background_v4.tex <==
\section{Background}\label{sec:background}


\subsection{World Model}
The concept of a ``World Model" is not a recent invention of the generative AI era but has deep roots in cognitive science and control theory. 
Historically, it posits that intelligent agents do not act directly on raw sensory inputs but rather on an internal mental simulation of the environment.

Early psychological theories, such as Mental Models~\cite{forrester1971counterintuitive}, suggested that humans reason by constructing small-scale models of reality to anticipate events. 
In the context of artificial intelligence, this concept was formalized within Model-Based Reinforcement Learning (MBRL), where agents learn a transition model of the environment to support planning and decision-making. 

Unlike model-free approaches~\cite{mnih2015human, mnih2016asynchronous, barth2018distributed} that function as a reflexive mapping—merely memorizing a direct rule from observations to actions without understanding the underlying mechanics, World models~\cite{ha2018recurrent,wu2023daydreamer, hafner2020mastering, hafner2023mastering, hafner2019learning, lecun2022path, assran2025v,bardes2024revisiting, ha2018world}, explicitly learns the underlying structure of the environment by maintaining a compact, internal state $S_t$. Formally, we define the core mechanism of a World Model as a recurrent system where the future state $S_{t+1}$ is evolved from the current state $S_t$, driven by the agent's action $A_t$ and updated by the current sensory observation $O_t$:


\begin{equation}
S_{t+1} = F_{\theta}(S_t, A_t, O_t)
\end{equation}

As exemplified by foundational works such as \textit{World Models}~\cite{ha2018recurrent} and the \textit{Dreamer} series~\cite{hafner2019learning}, this formulation explicitly factorizes the modeling process into two distinct functional components:

\begin{enumerate}
\item \textbf{Dynamics \& Memory (The Transition $F$):} The function $F$ acts as the "brain" of the system. It integrates the current perception ($O_t$) and intervention ($A_t$) into the historical context ($S_t$) to produce the updated state $S_{t+1}$. This process represents the \textit{State Estimation}, ensuring the internal belief remains aligned with the observed reality.

\item \textbf{Rendering (The Observation Model):} Since the state $S_{t+1}$ is a compact, abstract representation (latent variable), it is not directly visible. To predict or visualize the future, an additional \textbf{Visual Decoder} (or Observation Model) is required to translate the abstract state back into the sensory space:
$$\hat{O}_{t+1} \sim P(O | S_{t+1})$$
This separation allows the model to perform reasoning and planning in a highly efficient latent space without the computational burden of pixel-level processing at every logical.

\end{enumerate}

\textbf{Simulation Capability.}
A critical feature of this formulation is its ability to support "dreaming" or simulation. When real observations $O_t$ are unavailable (e.g., predicting far into the future), the model can feed its own predicted observations $\hat{O}_t$ (or sample from the latent prior) back into the transition function $F$. This enables the agent to simulate counterfactual futures $S_{t+1}, S_{t+2}, \dots$ solely based on its internal dynamics and planned actions.

3.  Action (Control): The state evolution is fundamentally driven by an explicit Action ($A_t$), representing the agent's intervention in the world. This distinguishes a world model from a passive video predictor; it models the causal consequences of interactions rather than just temporal correlations.


While recent surveys~\cite{ding2025understanding} classify world models broadly into "understanding" (internal representation) and "predicting" (future simulation), our survey adopts a mechanism-centric view. We emphasize that the defining feature of a true World Model is the Explicit Factorization of state estimation and dynamics prediction, driven by control signals. This rigorous definition serves as the benchmark against which we evaluate modern video generation models.

To encapsulate these mechanisms within a general theoretical framework, we abstract the specific architectural variations (e.g., RSSM's deterministic path or JEPA's predictor~\cite{lecun2022path}) into a unified state evolution function. Whether operating in a perception mode (updating belief with new data) or simulation mode (predicting futures), the evolution of the world state $S_{t+1}$ can be formally expressed as:
\begin{equation}
    S_{t+1} = F(S_{t}, A_{t}, O_{t})
\label{eq:world model}
\end{equation}


In this formulation:
\begin{itemize}
    \item $S_t$ represents the Current Compact State, compressing the history of observations and internal dynamics.
    \item $A_t$ represents the Explicit Action, serving as the causal driver for state transitions.
    \item $O_t$ represents the Observation (sensory input). When available, it acts as a correction signal to align the internal state with reality (Posterior); when unavailable (e.g., during latent dreaming or planning), it is marginalized or omitted, forcing the model to rely solely on internal dynamics (Prior)~\cite{hafner2019learning, ha2018world, lecun2022path}.
\end{itemize}

This formula highlights the "active" nature of World Models: the state does not merely flow from time; it is actively constructed through interaction ($A_t$) and calibrated by perception ($O_t$).





\subsection{Video Generation Models: The Implicit Paradigm}

While classic World Models are defined by explicit state factorization and control, modern video generation models operate on a fundamentally different premise. In this section, we analyze the mathematical formulation of current video generators, tracing their evolution from bidirectional diffusion to autoregressive transformers, and highlight their structural deficits in terms of state and action.

\textbf{The Architectural Shift: From Bidirectional to Causal.}
Following the release of Sora~\cite{openai2024sora}, the field has been dominated by models built upon Diffusion Transformers (DiT) equipped with bidirectional attention~\cite{zhang2025waver,wan2025wan,kong2024hunyuanvideo,agarwal2025cosmos,genmo2025blog,lin2024open,zheng2024open,yang2024cogvideox}. These models typically treat video generation as a global optimization problem, generating short video clips (e.g., 5 seconds) in a one-shot manner. Here, text prompts are encoded and used as conditioning signals for visual token generation via cross- or self-attention.

However, to better capture the sequential nature of video and scale to longer durations, a parallel line of research explores \textbf{auto-regressive models} for video generation~\cite{sun2025ardiff,teng2025magi,yu2025videomar,zhuang2025video,gu2025long,lin2025autoregressive,kondratyuk2023videopoet,deng2024autoregressive,yuan2025lumos,weng2024art,chen2024diffusion, huang2025self,yin2025causvid}. These approaches incorporate causal attention masks, training the model to predict future tokens conditioned on clean (low-noise) past tokens as additional context.

\textbf{The Probability Formulation: Observation-Driven Generation.}
Despite these architectural variances, both paradigms converge on a unified mathematical objective: they function as Observation-Driven systems rather than State-Driven systems. Fundamentally, they model the conditional probability of the next observation $O_{t+1}$ given the raw history:
\begin{equation}
    O_{t+1} = F_{\theta}(O_{1:t}, C_{global})
\label{eq:video model}
\end{equation}

Contrasted with the World Model formula ($S_{t+1} = F(S_t, A_t)$), this formulation reveals a critical distinction: the absence of an intermediate, compact variable $S_t$. All deductive reasoning relies directly on the raw observation history $O_{1:t}$ rather than a latent belief state.

\textbf{The "State" Gap: From Compact State to Massive Context.}
The most significant deviation in video models is how they "remember" the world.
\begin{itemize}
    \item \textbf{Implicit State:} Instead of maintaining a compressed latent belief, video models rely on the \textbf{Context Window} ($O_{1:t}$) as a "Pseudo-State." The model must attend to the entire history of raw pixels or tokens to infer the current status of the world.
    \item \textbf{Inefficiency \& Inconsistency:} This representation is unstructured and redundant. As video length increases, the computational cost of processing this history grows significantly (leading to KV Cache explosion). Furthermore, without a compact $S_t$ to "lock in" physical attributes (e.g., the color of a shirt or the shape of an object), the model is prone to \textbf{Forgetting} and \textbf{Inconsistency}, where objects morph or vanish because the model must re-extract features from noisy history at every step.
\end{itemize}

\textbf{The "Action" Gap: From Step-wise Control to Global Conditioning.}
Video models traditionally function as passive simulators rather than interactive agents due to the nature of their control signals.
\begin{itemize}
    \item \textbf{Static Conditioning:} Control is typically exerted via \textbf{Global Conditions} $C_{\text{global}}$, such as text prompts. These signals are static and define the overall trend (e.g., "A man walking") but fail to define specific, time-step actions (e.g., "Turn left at the 5th second").
    \item \textbf{Lack of Causality:} Lacking an explicit action variable $A_t$ to drive state transitions ($S_t \xrightarrow{A_t} S_{t+1}$), these models struggle to learn true \textbf{Causality}. They capture temporal correlations ("what usually happens") but cannot robustly simulate interventions ("what happens if I push this object"), limiting their utility for counterfactual reasoning.
\end{itemize}

It is worth noting that recent \textbf{Action-Controlled Approaches}~\cite{yu2025gamefactory, che2024gamegen, valevski2024diffusion, he2025matrix} have begun to bridge this specific gap. By aligning control signals temporally with the video sequence, these methods effectively define the trajectory of generation, offering a preliminary solution to the "Action Gap" and moving closer to the interactive requirements of World Models.

Our survey focus on the "state" side.






==> legacy/3_definition.tex <==
\section{Definition}\label{sec:definition}

\subsection{World Model Definition}
The concept of a ``World Model'' is not a recent invention of the generative AI era but has deep roots in cognitive science and control theory. Historically, it posits that intelligent agents do not act directly on raw sensory inputs but rather on an internal mental simulation of the environment.

\noindent\textbf{Origins and Conceptual Evolution.}
Early psychological theories, such as Mental Models~\cite{forrester1971counterintuitive}, suggested that humans reason by constructing small-scale models of reality to anticipate events. In the context of artificial intelligence, this concept was formalized within Model-Based Reinforcement Learning (MBRL), where agents learn a transition model of the environment to support planning and decision-making. \textbf{Functionally, this learned transition model serves as an internal simulation engine, enabling agents to look ahead and reason about the future before acting.}

\noindent\textbf{Core Pillars: Representation and Sequence Modeling.}
To translate this conceptual simulation into a rigorous computational framework, we distill the architecture of a World Model into two fundamental capabilities:

\begin{itemize}
    \item \textbf{Representation Learning (Encoder Model):} 
    The ability to compress high-dimensional sensory observations ($O_t$) into a compact, semantically rich latent state ($S_t$). This serves as the \textit{grounding} mechanism, extracting the essential state of the world from raw data.
    \begin{equation}
        S_t = \text{Enc}(O_t, \dots) \quad \text{(From Observation to State)}
    \end{equation}

    \item \textbf{Dynamics Learning (Transition Model):} 
    The ability to predict the evolution of the state over time ($S_t \to S_{t+1}$), optionally conditioned on actions ($A_t$). This serves as the \textit{simulation} engine, modeling how the world state transitions under physical laws.
    \begin{equation}
        S_{t+1} = \text{Trans}(S_t, \dots) \quad \text{(From State to Future State)}
    \end{equation}
\end{itemize}

\noindent\textbf{Learning Objectives: Fidelity vs. Utility.}
A critical question in world modeling is: \textit{what drives the learning of these two pillars?} Historically, two distinct forces have driven this process:
\begin{itemize}
    \item \textbf{Utility: Task-Driven Optimization} 
    In many Model-Based Reinforcement Learning (MBRL) approaches~\cite{hansen2023td,hansen2022temporal}, the state space is significantly shaped by extrinsic rewards to solve specific tasks. 
    Some decision-centric architectures, such as \textbf{MuZero}~\cite{schrittwieser2020mastering}, \textbf{Value Prediction Networks}~\cite{oh2017value}, and \textbf{The Predictron}~\cite{silver2017predictron}, even explicitly bypass visual reconstruction, optimizing the transition dynamics solely for value prediction and planning utility.
    This necessitates a \textbf{Closed-Loop Interaction} to correct prediction errors based on task feedback (e.g., rewards or values) rather than sensory pixels.
    
    \item \textbf{Fidelity: Visual-Driven Optimization} Conversely, foundational works like World Models (VMC)~\cite{ha2018recurrent} and Dreamer series~\cite{hafner2019learning,hafner2020mastering,hafner2023mastering, hafner2025training} have demonstrated that dynamics can be learned via \textbf{Unsupervised Visual Reconstruction}. This implies that the ability to visually reconstruct the future is a sufficient proxy for understanding physical laws, enabling \textbf{Open-Loop Learning}.
\end{itemize}

The comparison between closed-loop and open-loop are summarized in Table~\cite{tab:open_vs_closed_loop}

\noindent\textbf{Justification: The Sufficiency of Visual Simulation.}
It is crucial to clarify that acquiring a robust Transition Model does not strictly necessitate the closed interaction loop characterized by Reward and Action models.
While we acknowledge alternative paradigms—such as decision-centric models like MuZero~\cite{schrittwieser2020mastering}, Value Prediction Networks~\cite{oh2017value}, and The Predictron~\cite{silver2017predictron}, which bypass observation reconstruction to prioritize value prediction and planning utility.—our focus lies on the potential of pure video generation models to evolve into foundational World Models.
We posit that the capacity to simulate world dynamics (Fidelity) can be acquired through \textbf{passive observation} alone, independent of task-specific goals (Utility).
Based on this insight, we identify a ``minimal viable path'' to General World Simulation. 
By stripping away task-specific dependencies (i.e., Reward and Action models) and focusing on the open-loop simulation regime, we isolate the combination of \textbf{Sequence Modeling} (for dynamics) and \textbf{Visual Modeling} (for fidelity) as the most scalable approach to world modeling. 

Consequently, modern autoregressive video generation models can be viewed as a direct instantiation of this path. 
They implicitly learn a world simulator by mastering the next-token prediction objective on massive visual data. 
The central inquiry of this survey is whether these video models, while successfully mimicking the \textit{visuals}, have truly acquired the structured \textbf{State Representations} necessary for robust, long-term physical reasoning—or if explicit representation learning must be reintroduced to bridge the gap between generation and simulation.

\textit{Note: In the context of generative simulation discussed hereafter, we assume an open-loop setting where future observations are generated by the model itself. Consequently, we omit the distinction between ground truth $O_t$ and generated $\hat{O}_t$, referring simply to the observation stream.}


\subsection{Video Generation Models: From Observation to Simulation}
\label{sec:video_models}

While classic World Models are rigorously defined by explicit state factorization and control logic, modern video generation models operate on a fundamentally different mathematical premise. In this section, we trace the evolution of video generators from parallel synthesis to autoregressive prediction, analyzing how they are gradually acquiring the properties of a Transition Model, and identifying the critical structural deficits—specifically regarding \textit{Action} and \textit{State}—that remain.

\noindent\textbf{The Architectural Shift: Acquiring the ``Transition'' Capability.}
The field of video generation has witnessed a bifurcation in modeling paradigms, which can be mapped to the components of a World Model:

\begin{itemize}
    \item \textbf{Global Generation (The Observation Model):} 
    Leading approaches following Sora~\cite{openai2024sora} (e.g., bidirectional DiT~\cite{zhang2025waver,wan2025wan,kong2024hunyuanvideo,agarwal2025cosmos}) treat video generation as a global optimization problem. They generate the entire sequence simultaneously (or in large blocks) conditioned on a global prompt ($C_{global}$). Mathematically, this approximates the \textbf{Observation Model} $\hat{O} \sim P(O | C_{global})$, mapping a static semantic latent directly to pixels without explicitly modeling the temporal evolution physics step-by-step.

    \item \textbf{Autoregressive Generation (The Transition Model):} 
    To capture the causal nature of the physical world, a parallel line of research~\cite{sun2025ardiff,teng2025magi,yu2025videomar,zhuang2025video,gu2025long,lin2025autoregressive,kondratyuk2023videopoet,deng2024autoregressive,yuan2025lumos,weng2024art,chen2024diffusion, huang2025self,yin2025causvid} enforces strict temporal causality via attention masks. By predicting future tokens based solely on past tokens, these models formally acquire the capability of a \textbf{Transition Model}. They function as a simulation engine, rolling out the future indefinitely.
\end{itemize}

\noindent\textbf{The Probability Formulation: Observation-Driven Simulation.}
Despite acquiring the temporal autoregressive property, these models differ from standard World Models in a critical way: they remain \textbf{Observation-Driven}. 
Fundamentally, they model the conditional probability of the next observation $O_{t+1}$ given the raw history and the global condition:
\begin{equation}
    O_{t+1} = F_{\theta}(O_{1:t}, C_{global})
\label{eq:video_model}
\end{equation}
Contrasting Eq.~\ref{eq:video_model} with the standard World Model transition ($S_{t+1} = F(S_t, A_t)$), we identify two profound structural gaps: the absence of explicit control ($A_t$) and the absence of a compact state ($S_t$).

\noindent\textbf{The ``Action'' Gap: From Passive to Interactive.}
Standard video models function as passive simulators driven by static Global Conditions $C_{global}$ (e.g., text prompts), rather than interactive agents driven by dynamic Action $A_t$. 
Without $A_t$, models capture temporal correlations (``what follows'') but struggle with causality (``what happens if I do $X$'').
\textit{Status:} This gap is rapidly narrowing. Recent \textbf{Action-Controlled Approaches}~\cite{yu2025gamefactory, che2024gamegen, valevski2024diffusion, he2025matrix} have successfully bridged this deficit by injecting time-aligned control signals into the generation process. Given these advancements, we consider the integration of Action to be a solved or actively progressing engineering challenge.

\noindent\textbf{The ``State'' Gap: The Core Focus.}
While the action gap is being addressed, the most significant bottleneck preventing infinite-horizon simulation is the \textbf{Representation of Memory}.
\begin{itemize}
    \item \textbf{Context vs. State:} Instead of maintaining a compact Markovian state $S_t$ that encapsulates the ``world status,'' video models rely on the entire history window $O_{1:t}$ as a \textbf{``Pseudo-State.''} The model must attend to all previous raw pixels/tokens to infer the current physics.
    
    \item \textbf{The Cost of Non-Markovian Simulation:} This unstructured representation is inefficient and fragile. 
    (1) \textbf{Computational Explosion:} As simulation length ($t$) increases, the cost of processing history grows linearly or quadratically (KV Cache explosion).
    (2) \textbf{Inconsistency:} Without a compact $S_t$ to ``lock in'' physical attributes (e.g., object permanence, 3D structure), the model is prone to forgetting and hallucination over long horizons.
\end{itemize}

\noindent\textbf{Conclusion of Scope.} 
Consequently, this survey pivots to address the \textbf{State Gap}. We investigate how the field is moving from raw-history dependence ($O_{1:t}$) towards learning compact, robust World States ($S_t$) within video generation transformers, enabling efficient and consistent long-term simulation.










==> legacy/3_definition_v2.tex <==
\section{Definition}\label{sec:definition}
This section establishes the theoretical framework of the survey. 
Section~\ref{sec:world_model_def} defines the concept of a ``World Simulator'' by grounding it in the theory of mental models and distinguishing it from domain-specific environmental maps. 
Section~\ref{sec:video_models} traces the evolution of Video Generation Models—from static rendering to autoregressive dynamics—and analyzes how the necessity of managing historical context leads to the dichotomy between ``Implicit Computational States'' and ``Explicit Latent States''.

\subsection{World Model Definition: From Ideal to Simulator}
\label{sec:world_model_def}
The concept of a ``World Model'' is rooted in the cognitive science definition of \textbf{Mental Models}~\cite{craik1943nature, johnson1983mental, ha2018recurrent}. 
Functionally, a World Model serves two primary objectives:
\begin{itemize}
    \item \textbf{State Estimation:} Inferring the true compact state of the world from partial or noisy observation sequences (Observation $\to$ State).
    \item \textbf{Dynamics Prediction:} Simulating the evolution of the world state over time, conditioned on actions or physical laws (State $\to$ Next State).
\end{itemize}

\noindent\textbf{Scope Clarification: Dynamic Simulation vs. Static Reconstruction.}
It is crucial to distinguish the \textit{Cognitive World Model} discussed here from domain-specific definitions often found in Autonomous Driving or 3D Vision. 
In those contexts, a ``world model'' frequently refers to a static, geometric reconstruction of the environment (e.g., HD Maps, Occupancy Grids, or 4D Scene Fields). 
In contrast, this survey focuses on the \textbf{Temporal Cognitive System}—a dynamic engine capable of counterfactual reasoning and future prediction. 
While 3D representations can serve as the \textit{content} of a state, they are not the model itself without the capacity for temporal evolution.

\noindent\textbf{Defining State: The Sufficient Statistic.}
Central to this dynamic framework is the rigorous definition of \textbf{State ($S_t$)}. 
In control theory, a valid state is defined as a \textbf{Sufficient Statistic} of the history. 
That is, $S_t$ must compress the entire history of observations $O_{1:t}$ such that predicting the future depends \textit{solely} on $S_t$, rendering the past history conditionally independent:
\begin{equation}
    P(O_{t+1} | S_t) \approx P(O_{t+1} | O_{1:t})
\end{equation}

\noindent\textbf{Learning Dynamics: Closed-Loop vs. Open-Loop.}
The acquisition of these world dynamics is typically driven by two distinct paradigms:
\begin{itemize}
    \item \textbf{Closed-Loop Learning (Task-Driven):} The model is paired with an embodied policy to perform \textbf{Active Learning} (e.g., Dreamer~\cite{hafner2019learning}). The state space is shaped by extrinsic rewards or utility functions. While effective for specific tasks, this often leads to abstractions that discard physical details irrelevant to the reward.
    \item \textbf{Open-Loop Learning (Visual-Driven):} The model learns by passively observing massive streams of video data, driven by \textbf{Visual Modeling} (e.g., pixel reconstruction or feature prediction~\cite{assran2023self}). Recent studies suggest that this paradigm benefits significantly from scaling laws, enabling the model to learn general physical laws without task-specific constraints.
\end{itemize}

\noindent\textbf{The ``World Simulator'': The Open-Loop Core.} 
Driven by the potential of web-scale video data, we posit that general-purpose world understanding is attainable via Open-Loop Learning. 
Consequently, we narrow our focus to the \textbf{World Simulator}—defined here as the environmental modeling core, operating independently of an agent:
\begin{itemize}
    \item \textbf{World State ($S_t$):} A compact, explicit latent representation acting as a sufficient statistic of the world.
    \item \textbf{Transition Model ($S_t \to S_{t+1}$):} The universal physics engine.
    \item \textbf{Observation Model ($S_t \to O_t$):} The interface that decodes latent states back into the visual world.
\end{itemize}
\textit{Note: In this context, the World Simulator excludes the Policy and Reward modules, serving purely as the foundation for physical simulation.}

\subsection{Video Generation Models: The Necessity of Explicit State}
\label{sec:video_models}
The evolution of video models has witnessed a structural shift. 
Early approaches, such as standard Diffusion Transformers (DiT)~\cite{peebles2023scalable}, focused on \textbf{Global Rendering}—generating fixed-length clips by treating time as a spatial dimension.
However, recent advancements have moved towards \textbf{Autoregressive Generation} (e.g., VideoPoet~\cite{kondratyuk2023videopoet}, Diffusion Forcing~\cite{chen2024diffusion}), where models generate frame-by-frame or chunk-by-chunk. 
Formally, this shift grants video models the capability of \textbf{Dynamics Prediction}, aligning them with the functional requirements of a World Simulator.

\noindent\textbf{Bottlenecks of Stateless Generation.}
Despite acquiring dynamics, modern Transformer-based video models generally remain \textbf{Stateless}. 
They function as direct mappings ($O_{1:t} \to O_{t+1}$), relying on the raw observation history. This leads to two fundamental bottlenecks:
\begin{itemize}
    \item \textbf{Computational Costs (Long Context):} As the generated sequence grows, the context window ($O_{1:t}$) expands. For Transformers, this results in linear or quadratic growth in memory and computation (KV Cache), making infinite-horizon simulation prohibitive.
    \item \textbf{Object Permanence (Attention Failure):} Without a persistent state variables (e.g., coordinates, ID), the model relies on Attention to ``retrieve'' objects from history. If an object is occluded for a duration exceeding the effective attention span, the model loses track of it, leading to consistency failures.
\end{itemize}

\noindent\textbf{Emerging Solutions: Memory and Recurrence.}
To overcome these limitations, the community has begun to re-introduce the concept of ``State'' through two main engineering pathways:
1) \textbf{Memory Mechanisms:} Augmenting Transformers with external memory banks or KV-cache management techniques to organize raw observations efficiently.
2) \textbf{Recurrent Systems:} Adopting architectures like Mamba or Linear Attention that inherently compress history into a fixed-size state.

\noindent\textbf{The Divergence: Implicit vs. Explicit State.}
We formalize these two pathways into a unified taxonomy of State Definitions:

\begin{itemize}
    \item \textbf{Implicit Computational State (The Context Paradigm):} 
    Represented by structures like the \textbf{KV Cache} or \textbf{Memory Banks}.
    These systems maintain history in its raw or semi-processed form to allow precise retrieval. While they can be updated (e.g., via token replacement), they are fundamentally \textit{extensive}—growing or shifting with the context window—rather than \textit{intensive} (compact abstract variables). They act as a sophisticated data buffer rather than a true Sufficient Statistic.
    
    \item \textbf{Explicit Latent State (The Simulator Paradigm):} 
    Represented by pre-defined, fixed-dimension vector variables ($S_t$).
    These systems (e.g., RNNs, SSMs) explicitly compress history into a compact latent space that drives the dynamics equations. This state is persistent, independent of sequence length, and strictly adheres to the definition of a Sufficient Statistic.
\end{itemize}

\noindent\textbf{Conclusion of Scope.}
The transition from Video Generation to World Simulation relies on solving the \textbf{State Definition Problem}. 
Current research is divided between optimizing the \textbf{Implicit Computational State} for better context management and architecting an \textbf{Explicit Latent State} for true physical compression.
Consequently, this survey pivots to systematically classify existing research based on these two distinct strategies.

==> legacy/3_definition_v4.tex <==
\section{Preliminaries}\label{sec:definition}
This section transitions from the motivational overview in the Introduction to a more rigorous theoretical framework.
We first formalize a generic world model as a temporal cognitive system with an internal state and dynamics (Section~\ref{sec:world_model_def}).
We then introduce the notion of a world simulator as its open-loop specialization (Section~\ref{sec:world_simulator}), and use this lens to contrast with contemporary Video Generation Models (Section~\ref{sec:video_models}).

\subsection{World Model: A Functional Definition}
\label{sec:world_model_def}

While the introduction outlined the cognitive origins of world models, here we provide a rigorous functional definition. This formulation aims to unify diverse applications.

To facilitate the subsequent discussion, we first establish the mathematical notation used throughout this formulation. 
Let $O_t$, $A_t$, and $S_t$ denote the observation, action, and compact latent state at time $t$, respectively. 

Formally, we define a world model as a \textbf{Temporal Cognitive System} driven by the interaction of two probabilistic components:

\vspace{0.1cm}
\noindent\textbf{1. State Estimation (Understanding the World).} This component is responsible for abstraction, compressing high-dimensional historical observations $O_{1:t}$ into a compact latent state $S_t$. Mathematically, it approximates the posterior distribution of the state given the sequence of observations:
\begin{equation}
S_{t} \sim P_{\phi}(S_t \mid O_{1:t})
\label{eq:state_estimation}
\end{equation}
In practice, the implementation of this estimation process varies significantly based on how temporal dependencies are handled. 
Many frameworks~\cite{ha2018world,ha2018recurrent, hafner2019learning, hafner2020mastering, hafner2023mastering, hafner2025training} adopt a recurrent state aggregation paradigm to capture non-static physical attributes, such as velocity, acceleration, and object permanence that are inherently absent in individual snapshots. 
By formulating the state transition as 
\begin{equation}
S_t = \text{Enc}_{\phi}(S_{t-1}, O_t, \dots), 
\label{eq:state_estimation}
\end{equation}
the model ensures that $S_t$ acts as a sufficient statistic or a ``belief state'' that maintains a persistent memory of the environment's evolution. 

Conversely, some methods simplify this process by assuming a strict observation-level Markovian property, where the latent state is derived solely from the current frame via 
\begin{equation}
S_t = \text{Enc}_{\phi}(O_t), 
\label{eq:state_estimation}
\end{equation}
While this approach offers superior computational efficiency, it implicitly assumes that a single snapshot provides a complete representation of the world's status, thereby requiring the subsequent dynamics model to infer missing temporal cues. 


Ultimately, the role of state estimation is to synthesize a comprehensive summary of the world by distilling raw sensory data into a unified, actionable representation.

\vspace{0.1cm}
\noindent\textbf{2. Dynamics Prediction (Predicting the World).}
This component specifies the causal evolution of the state. It acts as an internal simulation engine that rolls the world state forward, conditioned on the current state $S_t$ and (optionally) an action $A_t$:
\begin{equation}
    S_{t+1} \sim P_{\theta}(S_{t+1} \mid S_{t}, A_t)
\label{eq:dynamics_prediction}
\end{equation}
Crucially, this transition occurs in the latent space, allowing the model to simulate future outcomes $S_{t+1}$ purely based on internal dynamics, even in the absence of new sensory observations.

\medskip
\noindent
The defining characteristic of a world model is the nature of $S_t$.
Drawing from control theory~\cite{witsenhausen2005separation} and information theory~\cite{kalman1960new, tishby2000information},
an ideal world state should serve as an (approximate) sufficient statistic of the history for predicting the future.
Formally, we require a conditional independence relation:
\begin{equation}
    P(O_{t+1} \mid O_{1:t}) \approx P(O_{t+1} \mid S_t) .
\end{equation}
Equivalently, $O_{1:t} \rightarrow S_t \rightarrow O_{t+1}$ forms an approximate Markov chain:
$S_t$ acts as an \textbf{information bottleneck}~\cite{tishby2000information} that compresses the raw history, discarding nuisance details while retaining the causal variables needed for prediction.
Once such a state is constructed, the original observation sequence $O_{1:t}$ becomes, in principle, unnecessary for future predictions, in contrast to ``Stateless'' architectures that repeatedly attend to the full history at every step.

% \input{main/tables/training_paradigm}
\subsection{World Simulator as Open-Loop World Models}
\label{sec:world_simulator}

The functional definition above is agnostic to how a world model is acquired. In practice, two broad paradigms have been established to construct such models.

\noindent\textbf{Closed-Loop Interaction (Active Learning).}
In Model-Based Reinforcement Learning (MBRL)~\cite{schrittwieser2020mastering,alonso2024diffusion,hafner2019learning, hafner2020mastering, hafner2023mastering}, world models are trained jointly with a policy or controller. 
In this paradigm, the agent utilizes the world model to ``train in imagination,'' optimizing its policy to maximize cumulative rewards within the simulated environment. 
Consequently, the world model is implicitly driven by the agent's performance: it must learn accurate dynamics to enable successful planning and high returns. 
However, this task-centric optimization (e.g., Autonomous driving~\cite{hu2023gaia, gao2024vista, hu2023planning, zhu2025worldsplat, ren2025cosmos, russell2025gaia, wang2024drivedreamer, zhao2025drivedreamer}, Robotics~\cite{wu2023daydreamer, zhang2025reinforcing, li2025robotic, zhu2025wmpo, liao2025genie, chi2025wow, lyu2025dywa, lu2025gwm}) restricts the model's scope. 
The resulting world models are often biased towards specific environments or control tasks, lacking the generalization ability to simulate diverse, open-world scenarios.

\noindent\textbf{Open-Loop Observation (Passive Learning).}
In contrast, recent advancements~\cite{veo2025, openai2024sora} demonstrate that robust simulation capabilities can emerge from generative modeling alone. 
Instead of optimizing for specific rewards, these models employ self-supervised learning on internet-scale video corpora to minimize prediction error. 
Powered by scaling laws~\cite{kaplan2020scaling}, this approach allows the model to internalize universal physical regularities, such as gravity, collision, and object permanence, which are across a vast distribution of phenomena. 
This paradigm shifts the goal from solving a specific task to capturing the underlying causal laws of the general world, leading to the emergence of a general-purpose world simulator.


\medskip
\noindent\textbf{World Simulator: Open-Loop Specialization.}
We adopt the view that the open-loop paradigm is the more scalable route toward general-purpose world models~\cite{lecun2022path}. 
In what follows, we therefore use the term \emph{world simulator} to denote the following open-loop specialization:

\begin{quote}
    \textit{A world simulator is an open-loop dynamical system that learns a stateful representation capturing the sufficient statistics of physical evolution ($S_t \rightarrow S_{t+1}$) solely by minimizing visual reconstruction error (or feature prediction error), independent of extrinsic rewards.}
\end{quote}

This definition conceptually isolates the \textbf{world simulator} from any \textbf{policy model}, allowing us to focus purely on environmental fidelity.

% \input{main/tables/close_loop_vs_open_loop}
\subsection{Video Generation Models}
\label{sec:video_models}

Modern Video Generation Models, despite their impressive visual fidelity, operate on a fundamentally different mathematical premise compared to the World Simulator defined above.

\vspace{0.1cm}
\noindent\textbf{The Shift to Causal Prediction.}
Historically, seminal video diffusion models~\cite{yang2024cogvideox, kong2024hunyuanvideo, zheng2024open, wan2025wan, runway2024gen3, veo2025, kuaishou2024klingai} relied predominantly on bidirectional attention. These architectures treat the temporal dimension similarly to spatial dimensions, optimizing the generation of the entire sequence $O_{1:T}$ simultaneously (e.g., via global masking) rather than respecting temporal causality.

However, recent advancements~\cite{cui2025self, liu2025rolling, sun2025ardiff, teng2025magi, deng2024nova, yu2025videomar, zhuang2025video, lin2025autoregressive, gu2025long, kondratyuk2023videopoet, deng2024autoregressive, yuan2025lumos, weng2024art, chen2024diffusion, yin2025causvid} have reintroduced strict causality into the generation process, exemplified by methods such as \textit{Diffusion Forcing}~\cite{chen2024diffusion} and \textit{Autoregressive Diffusion}~\cite{sun2025ardiff, teng2025magi, deng2024nova}. 
This paradigm shift effectively transitions the objective from ``content generation'' (painting pixels) to ``next-step prediction'' (simulating dynamics). 
Consequently, these causal video models generally model the probability of the next observation directly given the raw history:
\begin{equation}
    O_{t+1} \sim F_{\theta}(O_{1:t}, c)
\label{eq:video_model}
\end{equation}
Crucially, this formulation lacks an explicit compact state $S_t$. Instead, it relies on the full context ($O_{1:t}$) via attention mechanisms to predict $O_{t+1}$. 
By analyzing this formulation, we identify two critical limitations preventing these models from serving as efficient world simulators:

\begin{itemize}
    \item \textbf{Computational Issue:} Since prediction relies on the full history $O_{1:t}$, the inference cost grows linearly or quadratically with time step $t$ due to the attention mechanism. It becomes computationally impractical to include all historical observations during inference for long-horizon simulations.
    
    \item \textbf{Memory Issue:} In Transformer-based architectures, an object is ``remembered'' only if its visual features exist within the current attention window. If an object is occluded or leaves the frame for a duration exceeding the context window (context length), it is mathematically erased from the system. This leads to a failure in maintaining \textbf{Object Permanence}, as the model cannot track entities that are not explicitly present in the immediate history.
\end{itemize}

\vspace{0.1cm}
\noindent\textbf{Bridging the Gap: Implicit vs. Explicit State.}
To address the computational and memory challenges inherent in stateless video generation, recent research has introduced various mechanisms to manage historical observations $O_{1:t}$.
We posit that these mechanisms essentially revolve around the definition and implementation of a \textbf{State} ($S_t$).
Ideally, a state should serve as a \textit{sufficient statistic} of the history-capturing all necessary information to predict the future while discarding redundant raw data.
However, realizing this ideal definition in practice requires balancing theoretical sufficiency with computational feasibility.

Based on how current approaches approximate this ideal state, we categorize them into two paradigms:
(1) \textbf{Implicit Computational State}, which focuses on optimizing the retrieval and storage of raw history (keeping $O_{1:t}$ accessible but managed);
and (2) \textbf{Explicit Latent State}, which enforces an information bottleneck to compress history into a fixed-size tensor (constructing a true simulator).
We detail this categorization below.



==> legacy/4_definition_v3.tex <==
\section{Definition}
\subsection{Formal Definition of World Models}

The recent line of work on world models spans a wide spectrum, from model-based RL systems such as Dreamer-style agents to vision-centric models that couple a latent dynamics model with a powerful image or video decoder. While these approaches differ in architecture and training regime, they all share the same underlying idea: an agent should maintain an internal picture of ``how the world evolves'' under actions, and use it for prediction, planning, or imagination.

To make this common structure explicit, and to later connect it to modern video generators, we adopt a minimal control-theoretic formulation of world models as follows.
The notion of a \emph{world model} originates from control and reinforcement learning.
An agent interacts with an environment that has a hidden state $S_t^{\mathrm{env}}$,
applies an action $A_t$, and receives an observation $O_t$:
\begin{equation}
S_{t+1}^{\mathrm{env}} = f(S_t^{\mathrm{env}}, A_t), 
\qquad
O_t \sim g(S_t^{\mathrm{env}}).
\label{eq:env_dynamics_background}
\end{equation}
A world model attempts to approximate these dynamics with an internal model of the
environment. 
It maintains its own internal state $S_t$ and updates it as
\begin{equation}
S_{t+1} = F(S_t, A_t, O_t),
\label{eq:wm_state_background}
\end{equation}
optionally together with a renderer
\begin{equation}
\hat O_{t+1} = G(S_{t+1}, A_t),
\label{eq:wm_renderer_background}
\end{equation}
which predicts future observations from the internal state.

Existing world models can be roughly categorized into two families~\cite{ha2018world,bardes2023v,assran2025v,huang2025towards}:
\begin{itemize}
    \item \textbf{Representation world models}, which learn $S_t$ in an abstract
    latent space (for example via an encoder applied to $O_t$). 
    The state captures task-relevant semantics but does not have to resemble pixels.
    \item \textbf{Generative world models}, which come with an
    explicit renderer $G$ that can reconstruct or imagine observations in a concrete
    space, such as images, videos, or compact latents.
\end{itemize}

In this classical setting, the distinction between state $S_t$ and observation $O_t$
is clear: $S_t$ summarizes the environment in a way that is convenient for prediction and control, whereas $O_t$ is the raw input perceived by the agent.
In the next section, we ask how modern video generation models fit into this picture.


\subsection{From Video Generators to World Models}

Most current video generation models follow a more \emph{functional} pattern that does not introduce an explicit state.
Let $O_t$ denote the observation at time $t$ and let $\mathcal{C}_t \subseteq O_{\le t}$ be a (possibly variable-length) context formed by a subset of past observations.
Then the dominant paradigm can be summarized as
\begin{equation}
O_{t+1} = F(\mathcal{C}_t, A_t), \qquad \mathcal{C}_t \subseteq O_{\le t},
\label{eq:functional_vg}
\end{equation}
where the model takes the current context $\mathcal{C}_t$ and the current action $A_t$ as input, and outputs the next observation $O_{t+1}$.

This formulation has two consequences:
(1) on the input side, there is \emph{no explicit state variable} $S_t$—the model only sees a chosen slice of the observation history;
(2) on the output side, the model predicts only the next observation, without explicitly producing and maintaining a persistent world state.
In practice, whatever information the model needs to carry forward must be encoded in $\mathcal{C}_t$, or in latents derived from it. 
The effective “state’’ is therefore identified with the current context or memory, rather than an abstract $S_t$.

This creates a gap between classical world models and current video generators:
video models “use history”, but they do not yet maintain a learnable world state in the sense of Eq.~\eqref{eq:wm_state_background}.

Moving on, the core challenge becomes how to introduce $S_t$ into video generation. The following two basic questions arises:

\begin{enumerate}
    \item \textbf{How should we introduce and define a state $S_t$ in a video generation framework?}  
    Concretely, what is the carrier of state: raw frames, latent features, 3D representations, object graphs, physics latents, or some task-specific embedding?
    \item \textbf{Once a state has been defined, how should it be updated?}  
    Beyond predicting $O_{t+1}$, the model should learn an internal update rule so that the world state itself is maintained and evolved in a differentiable, parameterized manner.
    % \begin{equation}
    % S_{t+1} = F(S_t, \cdot),
    % \end{equation}

\end{enumerate}

The ability to \emph{learn how to update a world state} is what distinguishes a true world model from a pure observation-to-observation generator. 
To discuss how current methods move in this direction, it is helpful to separate two broad research lines: one that treats “state’’ functionally as a managed context or memory, and one that introduces $S_t$ as an abstract latent world state.

\section{Two Directions towards World Generation Models}
\label{sec:def-memory-wm}
\subsubsection{Functional State as Memory}
\label{sec:functional-state}

In a large body of engineering practice and visual generation work, the notion of “state’’ is deliberately \emph{weakened} to mean simply “the set of information currently available to the model.’’
A typical formulation is
\begin{equation}
O_{t+1} = F(\mathcal{C}_t, A_t),\quad \mathcal{C}_t \subseteq O_{\le t},\quad S_t \equiv \mathcal{C}_t,
\end{equation}
that is, the context or memory $\mathcal{C}_t$ is directly identified with the state.

This design is mainly motivated by practicality:
\begin{itemize}
    \item as long as $\mathcal{C}_t$ contains enough information for predicting $O_{t+1}$, one can \emph{functionally} call it a state, i.e., “whatever inputs the model can currently access’’;
    \item compared to designing an additional latent state space, directly managing raw observations (or their latents) is more intuitive and cheaper to implement;
    \item the model itself does not attempt to maintain an explicit, independently parameterized, and recurrently updated world state $S_t$, but instead relies entirely on the managed history $\mathcal{C}_t$, which is then naturally referred to as “memory’’.
\end{itemize}

Under this definition, the research focus shifts from \emph{what is the world state?} to a more operational question:
\begin{quote}
How should we organize and manage the available information set $\mathcal{C}_t$—that is, the memory mechanism?
\end{quote}
Consequently, many works borrow the term “memory’’ and analogies to human or LLM memory, but what they actually construct are rules for assembling, updating, and compressing $\mathcal{C}_t$.
From this perspective, such a \emph{functional state} can be summarized as:
\begin{quote}
memory/context that is \emph{equivalent to state at the level of usage}, but does not possess the abstraction or learnable update dynamics of a true world state.
\end{quote}

In practice, different systems mainly differ in how they score the \emph{importance} of past observations and select which ones enter $\mathcal{C}_t$.
Two signals are particularly common:
geometry (for view-consistent scene generation) and time (for long-horizon video generation).
We will revisit these two “tasks’’ in Section~\ref{sec:mem-geometry} and Section~\ref{sec:mem-compression}, where we group methods by the importance signal they use.

\subsubsection{Direction 2: World State as Abstract Latent}
\label{sec:world-state-latent}

A complementary line of work stays closer to the classical world-model view and introduces an explicit latent state $S_t$ that is updated over time.
Here the model does not only consume a managed context $\mathcal{C}_t$, but also maintains its own compact internal state:
\begin{equation}
S_{t+1}, O_{t+1} = F(S_t, \mathcal{C}_t, A_t),\quad \mathcal{C}_t \subseteq O_{\le t}.
\end{equation}
The key difference is that $S_t$ is not just a subset or compression of observations defined by external rules; it is a parameterized latent that is updated by learnable dynamics and can, in principle, encode hidden variables such as geometry, physics, or scene semantics.

Many recent architectures implicitly fall into this category.
Causal linear attention and KV accumulation in SANA-Video–style models, state-space models for long-context video, or memory vectors in MALT-like designs all act as internal state variables that are recurrently updated as the sequence progresses.
Video diffusion models that are conditioned on a separate “world state’’ maintained by an LLM or a symbolic controller also belong here: the video model acts as a renderer $G$, while $S_t$ is maintained by an external but learnable world-model component.

From a memory perspective, Direction~2 can be viewed as making $M_t$ into a first-class latent $S_t$: the question is not only which observations to keep, but \emph{how to learn the update rule for the state itself}.
In the following sections, we will first look at how functional-state systems organize their memories (Direction~1), and then return to these abstract-state models to discuss how they learn and use $S_t$ (Direction~2).


==> legacy/4_memory_definition.tex <==
\section{Memory Definition}\label{Definition}
% memory in human neuroscience

Memory is the ability to encode, store and recall information. 
The three main processes involved in human memory are therefore \textit{encoding} (the process of acquiring and processing information into a form that can be stored), \textit{storage} (the retention of encoded information over time in short-term or long-term memory), and \textit{retrieval} (\textit{recall}, the process of accessing and bringing stored information back into conscious awareness when needed).

\begin{itemize}
    \item \textbf{Encoding} Memory encoding is the process of changing sensory information into a form that our brain can cope with and store effectively. In particular, there are different types of encoding in terms of how information is processed, such as \textit{visual encoding}, which involves processing information based on its visual features like color, shape, or texture; \textit{acoustic encoding}, which focuses on the auditory characteristics of information, such as pitch, tone, or rhythm; and \textit{semantic encoding}, which is based on the meaning of the information, making it easier to structure and remember. In addition, there are many approaches to make our brain better at encoding memory, such as \textit{mnemonics}, which involve using acronyms or peg-word systems to aid recall, \textit{chunking}, where information is broken down into smaller, meaningful units to enhance retention, \textit{imagination}, which strengthens encoding by linking images to words, and \textit{association}, where new information is connected to prior knowledge to improve understanding and long-term memory storage.
    \item \textbf{Storage} The storage of memory involves the coordinated activity of multiple brain regions, with key areas including: the \textit{prefrontal cortex}, which is associated with working memory and decision-making, helping us maintain and process information in the short term; the \textit{hippocampus}, which helps organize and consolidate information to form new explicit memories (such as episodic memory); the \textit{cerebral cortex}, which is involved in the storage and retrieval of semantic memory, allowing us to retain facts, concepts, and general knowledge over time; and the \textit{cerebellum}, which is primarily responsible for procedural memory formed through repetition.
    \item \textbf{Retrieval} Memory retrieval is the ability to access information and get it out of the memory storage. When we recall something, the brain reactivates neural pathways (also called synapses) linked to that memory. The prefrontal cortex helps in bringing memories back to awareness. Similarly, there are different types of memory retrieval, including \textit{recognition}, where we identify previously encountered information or stimuli, such as recognizing a familiar face or a fact we have learned before; \textit{recall}, which is the ability to retrieve information from memory without external cues, like remembering a phone number or address from memory; and \textit{relearning}, a process in which we reacquire previously learned but forgotten information, often at a faster pace than initial learning due to the residual memory traces that still exist.
\end{itemize}

In addition to the fundamental memory processing stages of encoding, storage, and retrieval, human memory also includes \textit{consolidation} (the process of stabilizing and strengthening memories to facilitate long-term storage), \textit{reconsolidation} (the modification or updating of previously stored memories when they are reactivated, allowing them to adapt to new information or contexts), \textit{reflection} (the active review and evaluation of one's memories to enhance self-awareness, improve learning strategies, and optimize decision-making), and \textit{forgetting} (the process by which information becomes inaccessible).

\begin{itemize}
    \item \textbf{Consolidation} Memory consolidation refers to the process of converting short-term memory into long-term memory, allowing information to be stably stored in the brain and reducing the likelihood of forgetting. It primarily involves the hippocampus and strengthens neural connections through \textit{synaptic plasticity} (strengthening of connections between neurons) and \textit{systems consolidation} (the gradual transfer and reorganization of memories from the hippocampus to the neocortex for long-term storage).
    \item \textbf{Reconsolidation} Memory reconsolidation refers to the process in which a previously stored memory is reactivated, entering an unstable state and requiring reconsolidation to maintain its storage. This process allows for the modification or updating of existing memories to adapt to new information or contexts, potentially leading to memory enhancement, weakening, or distortion. Once a memory is reactivated, it involves the hippocampus and amygdala and may be influenced by emotions, cognitive biases, or new information, resulting in memory adjustment or reshaping.
    \item \textbf{Reflection} Memory reflection refers to the process in which an individual actively reviews, evaluates, and examines their own memory content and processes to enhance self-awareness, adjust learning strategies, or optimize decision-making. It helps improve metacognitive ability, correct memory biases, facilitate deep learning, and regulate emotions. This process primarily relies on the brain's metacognitive ability (Metacognition) and involves the prefrontal cortex, which monitors and regulates memory functions.
    \item \textbf{Forgetting} Forgetting is a natural process that occurs when the brain fails to retrieve or retain information, which can result from \textit{encoding failure} (when information is not properly encoded due to lack of attention or meaningful connection), \textit{memory decay} (when memories fade over time without reinforcement as neural connections weaken), \textit{interference} (when similar or new memories compete with or overwrite existing ones), \textit{retrieval failure} (when information is inaccessible due to missing contextual cues despite being stored), or \textit{motivated forgetting} (when individuals consciously suppress or unconsciously repress traumatic or distressing memories). However, forgetting is a natural and necessary process that enables our brains to filter out irrelevant and outdated information, allowing us to prioritize what is most important for our current needs.
\end{itemize}
 


Based on our formulation of a Generative World Model (Eq. \ref{eq:gwm}), $M_{t+1} = F(M_t, A_t)$, the model's operation is split into two conceptual parts:
\begin{itemize}
    \item \textbf{The Generative Engine ($G$)}, which is responsible for "imagining" or synthesizing new visual content ($G_t$);
    \item \textbf{The Memory Mechanism ($M$)}, which comprises all other modules (R, D, E, U) that manage the memory state $M_t$.
\end{itemize}

This mechanism is the ``cognitive'' part of the GWM, enabling temporal coherence, contextual reasoning, and long-range dependency. To understand this mechanism, we first define the memory state it manages, and then the processes that act upon it.


\subsubsection{The Memory Mechanism: R, D, E, and U in Practice}

The Memory Mechanism $F$ is the "how"—the set of processes that operate on $M_t$. These processes map directly to our R-D-G-E-U formulation:

\begin{itemize}
    \item \textbf{Retrieval (R).} This process, $R_t = R(M_t, [A_t])$, defines how stored memory is accessed and reintroduced into the generation cycle. In current video models, retrieval is often implemented as causal attention over a memory window (e.g., the KV-cache), allowing the model to reference previously generated features. This can be a "hard" retrieval (e.g., a sliding window) or a "soft" retrieval (i.e., the attention mechanism itself).

    \item \textbf{Decoding (D).} This optional process, $D_t = [D](R_t, [A_t])$, refers to how the retrieved memory $R_t$ is transformed into a format suitable for the Generative Engine ($G$). In many Transformer-based models, this is a simple identity function where $R_t$ is directly passed to $G$. In more complex designs, $D$ could involve cross-attention or token fusion to integrate $R_t$ with $A_t$.

    \item \textbf{Encoding (E).} This process, $E_t = [E](G_t, [A_t])$, is the counterpart to $D$. It defines how the new content $G_t$ (the "imagined" frame) is transformed into an internal representation $E_t$ that can be added to the memory state. As noted, this typically does not require an external encoder; the generation model itself produces the representations (e.g., the new Key-Value pairs) that will serve as the new memory content.

    \item \textbf{Update (U).} This final process, $M_{t+1} = U(M_t, E_t, [A_t])$, describes how the memory state evolves. It integrates the newly encoded experience $E_t$ with the old memory $M_t$. In simple causal models, this $U$ function is a \textbf{rolling window} or FIFO (First-In, First-Out) queue: the new representation $E_t$ is appended to the memory $M_t$, and the oldest representation is evicted to maintain a fixed size. This "evolution" is the computational counterpart of memory management (consolidation, forgetting) and is critical for long-sequence generation.


\end{itemize}

This R-D-E-U formulation provides a unified abstraction for understanding how visual memory operates within modern video generation systems, framing it as a complete cognitive cycle.

Example: Memory in a Causal Latent Video Diffusion Model.
To illustrate this cycle, we consider a latent video diffusion model (DiT) with causal attention, using a \textbf{KV-cache} as its memory mechanism.

\begin{itemize}
    \item \textbf{Memory State ($M_t$):} The storage $M_t$ is the \textbf{KV-cache} itself—a list of Key-Value pairs from previously generated frames/patches. This is a form of \textit{latent memory}.
    
    \item \textbf{Retrieval (R):} $R_t = R(M_t, A_t)$. This is the causal self-attention mechanism. The query $Q$ (derived from $A_t$ or the current denoising step) attends to the full history of Keys $K$ and retrieves the corresponding Values $V$ from $M_t$.

    \item \textbf{Decoding (D):} $D_t = [D](R_t)$. In this architecture, $D$ is an \textbf{identity function}. The retrieved context $R_t$ (the weighted sum of Values) is directly passed to the next layer of the DiT.

    \item \textbf{Generation (G):} $G_t = G(D_t, A_t)$. The DiT block (the Generative Engine) uses the retrieved context $D_t$ and the text/action prompt $A_t$ to perform one denoising step, ultimately producing a new clean latent $G_t$.

    \item \textbf{Encoding (E):} $E_t = [E](G_t)$. The $E$ module is the projection layer within the Transformer block. It takes the newly generated $G_t$ and computes its corresponding Key and Value pairs ($E_t = (K_{t+1}, V_{t+1})$) to be added to memory.

    \item \textbf{Update (U):} $M_{t+1} = U(M_t, E_t)$. The $U$ function is the \textbf{rolling queue mechanism}. It appends the new $E_t$ to $M_t$ and evicts the oldest KV-pair if the cache size is exceeded. This "evolution" ensures the memory window reflects the most recent context.

\end{itemize}

==> legacy/4_memory_definition_v2.tex <==
\section{Memory in Generative World Models}
\label{sec:memory-definition}

\subsection{What is Memory in Our Setting?}

The discussion above suggests a simple but unifying viewpoint: 
both the history of observations $\{O_{\le t}\}$ and an internal state $S_t$ can be seen as different \emph{forms of memory} about the world.

\begin{itemize}
    \item In \textbf{observation-driven models}, memory is realized externally as a stack of recent frames (or their latent encodings) that the model can attend to. 
    We may call this an \emph{observation memory}: it stores what has been seen, frame by frame, but does not explicitly disentangle structure, dynamics, or hidden variables.
    \item In \textbf{state-based models}, memory is realized internally as an evolving state $S_t$ updated by a dynamics module $F$ and used by a renderer $G$ to generate pixels. 
    We may call this a \emph{state memory}: it condenses past experience into a more compact representation that is not tied one-to-one to individual frames.
\end{itemize}

In both cases, memory is the mechanism that allows a generative video model to carry information forward across time. 
For our purposes, we will use a single symbol $M_t$ to denote whatever the model uses as its persistent carrier of information—whether this is an explicit state $S_t$, a KV cache, a bank of retrieved frames, a 3D scene representation, or a mixture of these.
The evolution of this memory can then be written abstractly as
\begin{equation}
M_{t+1} = F(M_t, A_t),
\label{eq:gwm_memory}
\end{equation}
with a video generator $G$ producing observations from $M_t$ and control $A_t$.

Once we adopt this memory-centric view, three questions become central:
\begin{itemize}
    \item \textbf{Storage:} how is information encoded and compressed into $M_t$ so that it fits within finite computational resources?
    \item \textbf{Information:} which parts of $M_t$ are considered relevant and can be accessed when generating the next observation?
    \item \textbf{Time:} how is $M_t$ updated, stabilized, or forgotten as new content is generated?
\end{itemize}

The rest of this section develops this perspective in two steps. 
We first recall related notions from cognitive memory to provide intuition for these three dimensions, and then introduce an operational decomposition of our R–D–G–E–U cycle that makes the roles of memory explicit in generative video world models.

\subsection{Cognitive Foundations}

As introduced in Section~\ref{sec:introduction}, we use the term \emph{memory} in a broad sense: the ability of a system to \emph{encode}, \emph{store}, and \emph{retrieve} information over time. 
These three operations correspond to three orthogonal dimensions of information management:
(i) a \textbf{storage} dimension that concerns how information is represented and compressed,
(ii) an \textbf{informational} dimension that concerns what is selectively retrieved as relevant, and
(iii) a \textbf{temporal} dimension that concerns how information is maintained, updated, or forgotten.

In human neuroscience, memory is commonly decomposed into a set of core processes~\cite{sherwood2004human}:

\medskip
\noindent\textbf{Encoding.}
Memory encoding is the process of changing sensory information into a form that the brain can cope with and store effectively. 
Different types of encoding emphasize different aspects of the input: 
\emph{visual encoding} focuses on features such as color, shape, or texture; 
\emph{acoustic encoding} focuses on auditory characteristics such as pitch or rhythm; 
and \emph{semantic encoding} organizes information by its meaning, making it easier to structure and remember. 
Humans employ various strategies to enhance encoding, including \emph{mnemonics} (acronyms, peg-word systems), \emph{chunking} (grouping information into meaningful units), \emph{imagery} (linking concepts to mental pictures), and \emph{association} (connecting new information to prior knowledge).

\medskip
\noindent\textbf{Storage.}
Storage refers to the retention of encoded information over time, supported by coordinated activity across multiple brain regions. 
The \emph{prefrontal cortex} is associated with working memory and decision-making, helping maintain and manipulate information in the short term; 
the \emph{hippocampus} organizes and consolidates information to form new explicit (episodic) memories; 
the \emph{cerebral cortex} is involved in the long-term storage and retrieval of semantic knowledge; 
and the \emph{cerebellum} is heavily involved in procedural memories formed through repeated practice.

\medskip
\noindent\textbf{Retrieval.}
Retrieval is the process of accessing information stored in memory and bringing it back into awareness. 
It relies on the reactivation of neural pathways (synapses) linked to the target memory, with the prefrontal cortex playing a key role in cueing and monitoring recall. 
Retrieval can take multiple forms: 
\emph{recognition}, where previously encountered information is identified (e.g., recognizing a familiar face); 
\emph{recall}, where information is produced without external cues (e.g., recalling a phone number); 
and \emph{relearning}, where previously learned but forgotten information is reacquired more quickly due to residual memory traces.

\medskip

Beyond these core stages, human memory also exhibits several higher-order processes.

\medskip
\noindent\textbf{Consolidation.}
Memory consolidation is the process of stabilizing and strengthening memories so that they can be stored long term. 
It primarily involves the hippocampus and relies on \emph{synaptic plasticity} (strengthening of connections between neurons) and \emph{systems consolidation} (gradual reorganization and transfer of memories from the hippocampus to neocortical areas).

\medskip
\noindent\textbf{Reconsolidation.}
Reconsolidation occurs when a stored memory is reactivated and enters a transiently unstable state. 
During this window, the memory can be maintained, weakened, or modified before being stored again. 
This allows existing memories to be updated to reflect new information or contexts, but also makes them susceptible to distortion, with the hippocampus, amygdala, and emotional and cognitive factors all influencing the outcome.

\medskip
\noindent\textbf{Reflection.}
Memory reflection refers to the active review and evaluation of one’s own memories and memory processes. 
It supports metacognition—awareness and regulation of one’s cognitive functions—by helping individuals adjust learning strategies, correct biases, and optimize decision-making. 
This process is closely linked to the prefrontal cortex and other networks involved in monitoring and control.

\medskip
\noindent\textbf{Forgetting.}
Forgetting is a natural process whereby information becomes inaccessible. 
It may result from \emph{encoding failure} (insufficient attention or weak initial encoding), \emph{decay} (weakening of neural traces over time without reinforcement), \emph{interference} (competition between similar memories), \emph{retrieval failure} (absence of appropriate cues despite stored content), or \emph{motivated forgetting} (conscious suppression or unconscious repression of distressing memories). 
Importantly, forgetting is functional: it helps filter out outdated or irrelevant information, allowing limited cognitive resources to focus on what is currently important.



%%%%%%%%%%%% 这一段要么滚，要么换一个位置 %%%%%%%%%%%%
In the era of large language models (LLMs), analogous notions have re-emerged in \textbf{LLM-powered autonomous agents}~\cite{wu2025human}. 
Agent memory is often defined as the process of acquiring, storing, retaining, and subsequently retrieving information over long interactions. 
Practical systems maintain persistent logs, summaries, and external knowledge stores (e.g., vector databases) that go beyond the base model’s context window, enabling agents to recall past user interactions, track goals, and adapt behavior over time.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this survey, we do not aim for a one-to-one mapping between human and artificial memory. 
Instead, we use these cognitive and cross-domain perspectives as intuition: memory is not a single static buffer, but a \emph{process} that decides
\emph{what} is encoded and stored, 
\emph{when} and \emph{how} stored information is retrieved, 
and \emph{how} memory is updated, consolidated, or forgotten as new experience arrives.
We now turn this intuition into an operational definition tailored to generative world models for video.


\subsection{Operational Definition in Generative World Models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: 加一个function flow图，R->D->G->E->U cycle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Building on the generative world model formulation in Eq.~\eqref{eq:gwm}, we view modern long-horizon video generators as systems whose behaviour is governed by the evolution of a memory state $M_t$ together with an optional control signal $A_t$. In this formulation, $M_t$ denotes the accumulated historical context (e.g., a sequence of latent frames or tokens), while $A_t$ represents auxiliary inputs such as text prompts, camera motion, or user actions that can steer future evolution.

From the cognitive perspective in the previous subsection, memory is not a single buffer but a process: information must be \emph{brought in} from the past, \emph{transformed} and used to imagine the future, and then \emph{written back} into memory in an updated form. To make these roles explicit in the context of Eq.~\eqref{eq:gwm}, it is useful to separate the model into two interacting components:

\begin{itemize}
    \item a \textbf{Generative Engine} $G$, which ``imagines'' or synthesizes 
    new visual content $G_t$ (e.g., via diffusion denoising or autoregressive decoding);
    \item a \textbf{Memory Mechanism}, which manages the state $M_t$ by deciding 
    what to retrieve, how to transform it, and how to update memory after generation.
\end{itemize}

In this view, the memory mechanism in generative world models plays a role analogous to encoding, storage, consolidation, and forgetting in human memory, while the generative engine is analogous to the ``imagination'' or simulation process that operates on retrieved content. To make this mechanism explicit and analyzable, we further decompose the update function $F$ into a unified cognitive cycle in the next subsection.


\subsection{The R–D–G–E–U Cycle}

We define a five-stage cycle that operationalizes how memory interacts with generation. 
For clarity, we keep the control $A_t$ as an optional input $[A_t]$ to most stages:

\begin{itemize}
    \item \textbf{Retrieval (R):} 
    selects relevant information from memory,
    \begin{equation*}
        R_t = R(M_t, [A_t]).
    \end{equation*}
    This stage parallels \emph{retrieval} in cognitive memory and governs the informational dimension: which parts of the past are brought into the current decision.

    \item \textbf{Decoding (D):} 
    (optional) transforms the retrieved content into a form suitable for generation,
    \begin{equation*}
        D_t = [D](R_t, [A_t]).
    \end{equation*}
    In many architectures, $D$ is an identity mapping; in others, it may include cross-attention, feature fusion, or projection into a different representational space.

    \item \textbf{Generation (G):} 
    uses decoded memory and current control to produce new visual content,
    \begin{equation*}
        G_t = G(D_t, A_t).
    \end{equation*}
    This is the core generative step (e.g., one denoising or decoding iteration), in which the model ``imagines'' the next frame or chunk consistent with both memory and control.

    \item \textbf{Encoding (E):} 
    (optional) converts the newly generated content into internal memory representations,
    \begin{equation*}
        E_t = [E](G_t, [A_t]).
    \end{equation*}
    This stage is analogous to \emph{encoding} in human memory: transforming raw experience (generated content) into internal codes that can be stored and later reused.

    \item \textbf{Update (U):} 
    integrates the new representations into memory and applies forgetting or consolidation,
    \begin{equation*}
        M_{t+1} = U(M_t, E_t, [A_t]).
    \end{equation*}
    This encompasses storage, consolidation, reconsolidation, and forgetting: deciding which information to keep, how to merge it with existing memory, and what to discard.
\end{itemize}

This R–D–G–E–U cycle provides an \emph{operational definition} of memory for video generation models:
it specifies \emph{what} is stored ($M_t$ and $E_t$), \emph{how} relevant information is brought into the generative process ($R$ and $D$), and \emph{how} memory evolves as new content is imagined ($U$).
Different architectures instantiate these modules in very different ways—ranging from simple sliding windows in token space to explicit 3D scene memories—but can all be analyzed under the same lens.

Each stage loosely mirrors components of human memory: 
encoding (E), storage and consolidation (U), retrieval (R), reconsolidation (U applied after reactivation), and forgetting (implicit in the update policy). 
We do not claim a strict neuroscientific correspondence, but this analogy is useful for organizing the design space of artificial memory mechanisms in video generators.
In Section~\ref{sec:Categorization}, we will use the R–D–G–E–U cycle as a unifying template to categorize existing methods along structural, functional, and temporal dimensions.


\subsection{Example: KV Cache as Latent Visual Memory}

To ground the above abstraction, we illustrate how the R–D–G–E–U cycle instantiates in a causal latent video diffusion model (DiT) that uses a \textbf{KV-cache} as its memory mechanism.

\noindent\textbf{Memory state (\textbf{$M_t$}).}
The memory state $M_t$ is the \emph{KV-cache} itself—a collection of Key–Value pairs from previously processed frames or patches across Transformer layers. 
This constitutes a form of \emph{latent visual memory} that stores compressed representations of past content rather than raw pixels.

\noindent\textbf{Retrieval (R).}
Retrieval $R_t = R(M_t, A_t)$ is implemented by causal self-attention over the KV-cache.
Given a query $Q_t$ (derived from the current noisy latent and control $A_t$), the model attends to all past Keys $K$ in $M_t$ and obtains a weighted combination of the corresponding Values $V$. 
This operation can be viewed as a soft, content-addressable lookup over the memory window, where relevance is determined by similarity in the key space.

\noindent\textbf{Decoding (D).}
In many DiT architectures, the decoding step $D$ is effectively an identity function:
the attention output (the weighted sum of Values) is directly fed into subsequent layers as context.
In more elaborate variants, $D$ may include additional fusion with control signals (e.g., via cross-attention, gating, or modulation), but the core role remains to turn retrieved memory into usable input for generation.

\noindent\textbf{Generation (G).}
Generation $G_t = G(D_t, A_t)$ corresponds to one denoising step of the diffusion transformer. 
Conditioned on the retrieved context $D_t$ and the control $A_t$ (e.g., text or action tokens), the model updates the noisy latent toward a cleaner sample, gradually synthesizing the next frame or chunk of the video.
Across multiple steps, this defines the dynamics of the generative engine.

\noindent\textbf{Encoding (E).}
Encoding $E_t = [E](G_t)$ is implemented by the projection layers that produce new Keys and Values from the updated latent representation.
These projected pairs $(K_{t+1}, V_{t+1})$ form an internal summary of the newly ``imagined'' content, which will serve as part of the memory state for future predictions.

\noindent\textbf{Update (U).}
The update rule $M_{t+1} = U(M_t, E_t)$ is typically a \textbf{rolling queue} or FIFO policy:
the new KV pairs $E_t$ are appended to $M_t$, and the oldest entries are evicted once the cache exceeds a predefined length.
More advanced designs may incorporate sparsification, compression, or hierarchical organization, but at their core they implement a trade-off between temporal coverage and memory capacity.

This example shows that even seemingly ``stateless'' diffusion transformers already admit a natural interpretation as generative world models with an internal memory mechanism. 
In the next section, we use the R–D–G–E–U framework to systematically analyze a wide range of memory designs in video generation, from local attention windows to explicit 3D scene memories, and to relate them to structural, functional, and temporal perspectives.



==> legacy/4_transition_v4.tex <==
% \section{From Video Generation to World Simulation}







==> legacy/5_category_v2.tex <==
\section{Categorization}\label{sec:Categorization}

\subsection{State as Managed Memory - Concrete State}
In this paradigm, the model does not explicitly construct a compact, abstract latent variable to represent the world. Instead, it relies on \textbf{Implicit State Construction}, where the "World State" is functionally equivalent to a \textbf{Managed Context} of historical observations.

% Definition: State as Managed History.
Here, the state $S_t$ is not a fixed-size vector but a dynamic collection of information derived from the history of observations $O_{1:t}$. 
Crucially, $S_t$ is not directly equivalent to the raw history (which would be computationally intractable) but is the result of an external \textbf{Memory Management Policy ($\mathcal{M}$)}. 
This policy dictates what to retain, what to retrieve, and what to discard (e.g., Sliding Windows, KV Cache Eviction, or RAG).
\begin{equation}
    S_t \equiv \mathcal{M}(O_{1:t})
\label{eq: memory}
\end{equation}
Under this definition, the "State" represents the \textbf{Active Working Memory} of the video model—the specific subset of history required to generate the next frame.

% Evolution: Generation-Update Cycle.
The "dynamics" of this world model are realized through a two-step cycle of Generation and Memory Update. Unlike standard world models where the state evolves via abstract physics ($S \to S$), here the state evolves by assimilating newly generated observations.
\begin{itemize}
    \item \textbf{Generation Phase:} The model utilizes the current managed state (context) $S_t$ and action $A_t$ to render the next observation: $O_{t+1} = G_\theta(S_t, A_t)$.
    \item \textbf{Update Phase:} The new observation is then fed back into the management policy to update the state: $S_{t+1} = \text{Update}(S_t, O_{t+1})$.
\end{itemize}

% **Unified Formulation.**
Functionally, we can view this entire process as a unified transition function $F$, where the "Observation" $O_{t+1}$ becomes an intermediate variable internalized within the memory update. The state transition formula can thus be written as:
\begin{equation}
    S_{t+1} = F(S_t, A_t) = \mathcal{M}\Big( S_t \cup \{ G_\theta(S_t, A_t) \} \Big)
\label{eq:implicit state}
\end{equation}

In this formulation:
\begin{itemize}
    \item $G_\theta$ represents the \textbf{Video Generator} (the visual decoder).
    \item $\mathcal{M}$ represents the \textbf{Management Functions} (e.g., \textit{Retrieve}, \textit{Compress}, \textit{Prune}). For instance, in Retrieval-Augmented Generation (RAG) approaches, $\mathcal{M}$ dynamically retrieves relevant past clips $O_{k<t}$ based on the current content, ensuring that $S_t$ contains the necessary long-term dependencies without storing the entire raw sequence.
\end{itemize}

% WORLDMEM
WORLDMEM~\cite{xiao2025worldmem} operationalizes this as \textbf{state- and time-aware retrieval} over explicit memory units ( {I,p,t} ) comprising past first-person frames, camera poses, and timestamps. At each step, a ranking objective approximated by Monte-Carlo field-of-view (FOV) overlap and temporal distance promotes those historical views that are both visible and temporally pertinent; a redundancy pass prunes duplicates by feature similarity. From the model's perspective, the retrieved set does not just enter self-attention; it is routed through a dedicated memory block where current latent queries attend to memory keys/values with pose–time embeddings, ensuring representational alignment between “what is being asked now” and “what was seen then.” This pose/time-conditioned selection along with the dedicated memory block is what converts “a large, noisy past” into “the causes that matter,” and it keeps a consistent world behavior: when the camera wanders and later revisits a site, the system recalls the relevant historical appearance and state, reinstating layout and detail well beyond the base context window. The timestamp (t) is not incidental—ablation shows that without time conditioning, the retriever conflates “same place at different times,” yielding anachronistic reconstructions.

% Context as Memory
Context-as-Memory~\cite{yu2025context} reaches a similar causal goal with a different retrieval contract: it treats all past frames as an explicit pool and uses camera geometry to pick only those whose FOV overlaps the current target pose, followed by simple de-duplication (dropping adjacent, duplicates and preferring non-adjacent, informative frames). Rather than projecting retrieved content via a dedicated block, the method concatenates the pose-aligned context frames with the current (noisy) tokens along the frame dimension so they participate symmetrically in spatiotemporal self-attention. This direct assembly of pose-consistent evidence yields robust interactive control: the memory naturally supports “look-away and look-back” sequences, where revisited regions reappear consistently because (R) injects exactly those frames that causally constrain the anticipated view. Empirically, the effect strengthens with larger but well-filtered contexts, given fixed attention budgets.

% Video World Models with Long-term Spatial Memory
SPMem\cite{wu2025video} extends the (R) role into a cognitively inspired, multi-stream retriever that disentangles static geometry, short-term dynamics, and long-horizon episodic detail. Its \textbf{spatial memory} is a persistent TSDF-fused 3D voxel grid that encodes view-consistent, long-lived structure; importantly, the system does not retrieve voxels directly but renders the current trajectory’s viewpoints into 2D static condition maps, encodes and injects them through zero-initialized residual (ControlNet-style) paths, an architectural choice that enforces spatial and structural awareness without overwhelming the generator with raw geometry. In parallel, a \textbf{working-memory} window of recent frames is retrieved by recency and concatenated frame-wise (with their associated condition tokens) to preserve short-term motion continuity, while \textbf{episodic memory} accrues keyframes whenever newly revealed scene area crosses a visibility threshold. In effect, spatial memory preserves a persistent world under arbitrary camera motion, rendered geometry provides structure awareness as a clean, drift-resistant condition, frame-wise fusion of recent context supports interactive control, and episodic recall restores fine details after long gaps while maintaining temporal consistency.

% Worldweaver: Generating long-horizon video worlds via rich perception
\cite{liu2025worldweaver}


% Learning World Models for Interactive Video Generation
\cite{chen2025learning}


% Mixture of contexts for long video generation
\cite{cai2025mixture}


% Streamingt2v: Consistent, dynamic, and extendable long video generation from text
\cite{henschel2025streamingt2v}

% Long-Context Autoregressive Video Modeling with Next-Frame Prediction
\cite{gu2025long}

% Loong: Generating minute-level long videos with autoregressive language models
\cite{wang2024loong}


% Packing input frame context in next-frame prediction models for video generation
\cite{zhang2025packing}


% Lovic: Efficient long video generation with context compression
\cite{jiang2025lovic}


% Pyramidal flow matching for efficient video generative modeling
\cite{jin2024pyramidal}



% \subsection{State as Explicit 3D Memory - Concrete State}
% Viewcrafter: Taming video diffusion models for high-fidelity novel view synthesis
\cite{yu2024viewcrafter}

% VMem: Consistent Interactive Video Scene Generation with Surfel-Indexed View Memory
\cite{li2025vmem}

% FlexWorld: Progressively expanding 3D scenes for flexiable-view synthesis
\cite{chen2025flexworld}

% Gen3c: 3d-informed world-consistent video generation with precise camera control
\cite{ren2025gen3c}

% Uni3C: Unifying Precisely 3D-Enhanced Camera and Human Motion Controls for Video Generation
\cite{cao2025uni3c}

% Genfusion: Closing the loop between reconstruction and generation via videos
\cite{wu2025genfusion}

% Scene Splatter: Momentum 3D scene generation from single image with video diffusion model
\cite{zhang2025scene}

% EvoWorld: Evolving Panoramic World Generation with Explicit 3D Memory
\cite{wang2025evoworld}


% Voyager: Long-Range and World-Consistent Video Diffusion for Explorable 3D Scene Generation
\cite{huang2025voyager}

% Stargen: A spatiotemporal autoregression framework with video diffusion model for scalable and controllable scene generation
\cite{zhai2025stargen}

% Matrix-3d: Omnidirectional explorable 3d world generation
\cite{yang2025matrix}

\subsection{Abstract Representations as State: The Joint Parameterization}

In contrast to the "Concrete" paradigm, which manages raw history via external policies, this paradigm seeks to construct the world state through Internalized Compression. Here, the model does not store a buffer of past observations; instead, it maintains a globally updating latent variable $S_t$ that acts as a mathematical summary of the history.

% \textbf{Definition: State as Learned Latents.}
In this framework, the "State" $S_t$ is an abstract, compact vector (or set of vectors) evolved by the network's internal recurrence. Crucially, the update mechanism is not a heuristic rule (like retrieval) but a learnable function parameterized by $\theta$. The generation process becomes a unified flow where the model simultaneously evolves its internal state and renders the visual observation:

\begin{equation}
    S_{t+1}, O_{t+1} = F_{\theta}(S_{t}, O_{t}, A_{t})
\label{eq:explicit state}
\end{equation}


Under this formulation, the model effectively performs a Joint Parameterization of the World Model components. The parameters $\theta$ must simultaneously satisfy two objectives:
\begin{enumerate}
\item \textbf{The Transition Model (Dynamics):} Learning how $S_t$ evolves to $S_{t+1}$ to maintain temporal logic and physical consistency.
\item \textbf{The Observation Model (Rendering):} Learning how to decode $S_{t+1}$ into high-fidelity pixels $O_{t+1}$.
\end{enumerate}

Depending on how the transition model is architecturally implemented relative to the observation generation, we categorize existing works into two sub-paradigms:

\begin{itemize}
\item \textbf{Implicit Internalization:} Methods where the transition model is intrinsically fused within the generative backbone. Here, the "State" corresponds to the hidden states of recurrent architectures (e.g., RNNs, LSTMs, Mamba/SSMs, or Linear Attention). The dynamics are learned implicitly as the network processes the sequence.


\item \textbf{Explicit Coupling:} Methods where the transition model is structurally distinct (e.g., a separate Latent Prior or RSSM module) but is trained jointly with the visual decoder end-to-end. Here, the "State" is an explicit latent variable designed to capture dynamics separate from purely visual details.


\end{itemize}



% MALT Diffusion: Memory-Augmented Latent Transformers for Any-Length Video Generation
\cite{yu2025malt}


% Long-context state-space video world models
\cite{po2025long}

% SANA-Video: Efficient Video Generation with Block Linear Diffusion Transformer
\cite{chen2025sana}

% Ssm meets video diffusion models: Efficient long-term video generation with structured state spaces
\cite{oshima2024ssm}

% Pack and Force Your Memory: Long-form and Consistent Video Generation
\cite{wu2025pack}


% Recurrent Autoregressive Diffusion: Global Memory Meets Local Attention
\cite{ha2018recurrent}


% One-minute video generation with test-time training
\cite{dalal2025one}

% Owl-1: Omni world model for consistent long video generation
\cite{huang2024owl}






==> legacy/5_category_v3.tex <==
\section{Categorization}\label{sec:Categorization}
As established in the preliminaries, the evolution from video generation to world simulation hinges on bridging the theoretical gap between two formulations: transforming the observation-driven probability of video models ($O_{t+1} \sim F_{\theta}(O_{1:t}, c)$) into the state-driven dynamics of world models ($S_{t+1} = F(S_t, A_t)$).

The fundamental challenge lies in the \textbf{Formalization of the State ($S_t$)}.
How can a video generation model, which naturally operates on high-dimensional pixel history, effectively instantiate the compact, causal variable required for simulation? 
We categorize existing research into two distinct paradigms based on how they define, construct, and utilize this state:

\begin{itemize}
    \item \textbf{Paradigm I: Implicit Computational State (Retrieval-Centric).} \\
    Approaches in this paradigm do not explicitly construct a new latent variable $S_t$ within the model architecture. Instead, they treat the \textit{managed context} of historical observations (or their Key-Value caches) as the implicit state.
    Here, the ``state transition'' is effectively governed by an \textbf{external management mechanism} (e.g., memory banks). 
    The video model itself is primarily responsible for rendering the visual outcome based on the context provided by the management mechanism.

    \item \textbf{Paradigm II: Explicit Latent State (Model-Centric).} \\
    Approaches in this paradigm explicitly construct a \textbf{compact state variable} $S_t$ (e.g., recurrent hidden states) within the network. 
    By implementing state transitions directly through the neural layers, they enforce a strict information bottleneck where history is compressed into a fixed-size representation.
    This establishes a \textbf{Joint Parameterization} that unifies the dynamics (the transition model $S_t \to S_{t+1}$) and the rendering (the observation model $S_t \to O_t$) within a single, end-to-end trainable backbone.
\end{itemize}


In the following sections, we will delve into these two paradigms, analyzing how they respectively address the challenges of long-term consistency and physical simulation.
\subsection{Implicit Computational State}

\subsubsection{Definition}
In this paradigm, the video generation model does not explicitly construct a compact, abstract latent variable to represent the world. 
Instead, it relies on implicit state construction, where the ``state'' is functionally equivalent to a managed context of historical observations.

% Definition: State as Managed History.
Here, the state $S_t$ is not a fixed-size vector but a dynamic collection of information derived from the history of observations $O_{1:t}$. 
Crucially, $S_t$ is not directly equivalent to the raw history (which would be computationally intractable) but is the result of an external \textbf{Memory Mechanism ($\mathcal{M}$)}. 

% Cognitive to Functional Definition
This mechanism constitutes the functional backbone of the implicit state construction. 
Drawing parallels to cognitive memory systems~\cite{sherwood2004human}—which rely on encoding to compress information, consolidation to stabilize storage, and retrieval to access relevant pasts—we can formalize $\mathcal{M}$ as a composite mechanism addressing the computational constraints of video generation through three functional primitives:
\begin{itemize}
    \item \textbf{Context Compression (Encoding):} Given the high spatio-temporal redundancy in video streams, raw history is inefficient to store. The mechanism compresses the context $O_{1:t}$ into compact representations (e.g., via token merging or summary vectors) to retain high-density information.
    \item \textbf{Context Retrieval (Recall):} Not all historical information is equally relevant for generating the next frame. The mechanism employs retrieval strategies (e.g., sparse attention or key-value lookup) to selectively access specific segments of the past state based on the current generation intent.
    \item \textbf{Memory Update (Consolidation):} Upon generating new content, the memory state must evolve. The update mechanism dictates how new observations are integrated and which obsolete information is evicted or re-weighted, enabling the model to support indefinite streaming.
\end{itemize}

Under this definition, the ``state'' represents the \textbf{Active Working Memory} of the video model—the specific subset of compressed and retrieved history required to generate the next frame.
% \begin{equation}
%     S_t \equiv \mathcal{M}(O_{1:t})
% \label{eq: memory}
% \end{equation}

% % Evolution: Generation-Update Cycle.
% The ``dynamics" of this world model are realized through a two-step cycle of generation and memory update. 
% Unlike standard world models where the state evolves via abstract latents ($S_{t} \to \hat{S}_{t+1}$), here the state evolves by assimilating newly generated observations: 
% (1) \textbf{Generation Phase:} The model utilizes the current managed state (context) $S_t$ and action $A_t$ to render the next observation; 
% (2) \textbf{Update Phase:} The new observation is then fed back into the memory mechanism to update the state.

% % Unified Formulation.
% Functionally, we can view this entire process as a unified transition function $F$, where the ``Observation" $O_{t+1}$ becomes an intermediate variable internalized within the memory update. The state transition formula can thus be written as:
% \begin{equation}
%     S_{t+1} = F(S_t, A_t) = \mathcal{M}\Big( S_t \cup \{ G_\theta(S_t, A_t) \} \Big)
% \label{eq:implicit state}
% \end{equation}

% In this formulation, $G_\theta$ represents the Video Generator (the visual decoder). 
% $\mathcal{M}$ represents the Management Functions corresponding to the primitives defined above (i.e., \textit{Compress}, \textit{Retrieve}, \textit{Update}). 
% For instance, in sliding window approaches, $\mathcal{M}$ dynamically retrieves the relevant past $k$ clips and evicts older frames during the update phase, ensuring that $S_t$ maintains necessary long-term dependencies without storing the entire raw sequence.

\subsubsection{Memory Mechanism - Compress}
In the context of video generation, \textbf{Context Compression} involves condensing long historical sequences into compact representations. 
The primary motivation behind this mechanism is to mitigate computational bottlenecks. 
While these methods typically prioritize inference efficiency over the explicit optimization of dynamics modeling, they serve as a critical foundation for scaling world models. 
By reducing the quadratic complexity of attention mechanisms, compression enables the exploration of scaling laws over extended temporal horizons. 
In this section, we summarize key strategies and highlight representative works that address this challenge. We examine how recent architectures instantiate this compression primitive through adaptive tokenization strategies (varying resolution based on relevance) and hierarchical abstractions (using multi-scale summaries to represent history).


FramePack~\cite{zhang2025packing} can be understood as designing $\mathcal{M}$ to \textbf{compress} the raw frame history into a bounded number of latent tokens before it is handed to $G_\theta$. Rather than keeping all patch tokens from all past frames, FramePack adjusts the patchify kernel size over time so that more recent or otherwise ``important" frames are patchified more to contribute more tokens, while older frames are aggressively downsampled for less tokens. In our notation, observations $O_{1:t}$ are first encoded into latent video tokens, and $\mathcal{M}$ then applies this importance-aware patchification to produce the managed state $S_t$: a compact, non-uniform token context that still resides in the same latent space as the standard input, allowing the generative backbone to remain architecture-agnostic. The underlying generator can therefore be largely preserved, while the effective context length is capped even as $t$ grows.

LoViC~\cite{jiang2025lovic} follows the same Concrete State philosophy for text-to-video, but implements $\mathcal{M}$ as a separate multimodal context encoder, FlexFormer. Past video segments and their captions are converted into latent tokens by a VAE and a text encoder; FlexFormer then uses a single learnable query token, replicated under different \textbf{compression} schedules (uniform / linear / logarithmic), to transform this long video–text history into a short sequence of ``context tokens". At generation time, $\mathcal{M}$ maps $O_{1:t}$ to $S_t$ by running FlexFormer on the accumulated history and concatenating its context tokens with the current segment’s tokens before self-attention. The state exposed to $G_\theta$ is thus an externally computed, compact context buffer rather than a learned latent $S_t$ inside the backbone.

Pyramidal Flow Matching~\cite{jin2024pyramidal} implements $\mathcal{M}$ as a spatiotemporal pyramid over the latent sequence. The denoising trajectory is re-formalized as a series of pyramid stages, where only the final stage operates at full resolution, and earlier stages work at coarser spatial and temporal scales. For autoregressive generation, the method builds a temporal pyramid that compresses the full-resolution history into a small set of multi-scale summaries which are reused when predicting future frames. From our perspective, $S_t$ is realized as this multi-level collection of latent tokens across resolutions, and $\mathcal{M}$ specifies how past frames are downsampled into pyramid levels, how flows are linked between levels, and which levels are exposed to attention at each step. The model, therefore, remains Concrete State: it manages and re-encodes the concrete history into a pyramidal context, instead of maintaining a separate, abstract state variable.

\textbf{RELIC}~\cite{hong2025relic} operates on the premise that the native attention mechanism serves as the optimal retriever given a sufficiently large context window. It avoids explicit external retrieval modules. Instead, it employs an aggressive Spatial Downsampling strategy on the historical KV cache, achieving a $4\times$ compression ratio. This allows the model to accommodate a complete history of up to 20 seconds within limited GPU memory. Crucially, by injecting absolute camera pose embeddings directly into the attention keys and queries, RELIC facilitates implicit, geometry-aware memory access, demonstrating that robust long-horizon 3D consistency can be maintained even under high-ratio latent compression.


% 加入一些kv cache compression的内容？
这是一个非常出色且成熟的文本结构。你已经准确抓住了“检索”在长视频生成中的两个核心维度：**Self-Consistency (A类)** 和 **Prior-Injection (B类)**。

为了让这段文字在 Survey 中显得更加学术化（Professional）且逻辑紧凑（Cohesive），我进行了以下微调：

1.  **逻辑分组 (Grouping):** 在 A 类中，我将文献进一步细分为 **"Geometric & State-Aware"**（基于几何/状态）和 **"Semantic & Latent Caching"**（基于语义/潜变量），避免流水账式的列举。
2.  **术语精炼 (Refinement):** 使用了更精确的术语，例如 *"Geometric Alignment"*, *"In-context Training"*, *"Exemplar-Conditioning"* 等。
3.  **对比强化 (Contrast):** 在介绍每一组方法时，强调了它们之间的细微差别（例如 WorldMem 的 dedicated block vs. Context-as-Memory 的 direct concatenation）。

以下是 Refine 后的 LaTeX 版本，你可以直接替换原有段落：

***

\subsubsection{Memory Mechanism - Retrieval (External)}
While compression strategies primarily target computational efficiency, \textbf{External Retrieval} targets \emph{contextual relevance}. 
Rather than compressing the entire history into a fixed state, these methods explicitly decide \emph{which} fragments of the past—or which external exemplars—should be reinstated as active context. 
Across recent developments in video world modeling, we identify two distinct retrieval paradigms that serve complementary roles in the generative pipeline.

\paragraph{A. History-Buffer Retrieval: Consistency via Self-Revisitation}
In this paradigm, the retrieval database consists of the model’s own accumulated history (generated frames, latents, and state metadata). The primary objective is to maintain \emph{object permanence} and \emph{scene consistency} during long-horizon rollouts, particularly when the camera revisits a previously unseen location.

\textbf{Geometric and State-Aware Retrieval.} 
To resolve spatial inconsistency, retrieval is often grounded in 3D geometry rather than simple visual similarity.
\textbf{WorldMem}~\cite{xiao2025worldmem} treats retrieval as a \emph{state- and time-aware ranking problem}. It stores memory tuples $(I, p, t)$ (image, pose, timestamp) and selects historical views based on geometric relevance (Field-of-View overlap) and temporal distinctiveness. Crucially, it routes retrieved content through a dedicated memory module with pose-aligned projection, ensuring that the retrieved "causes" align with the current "effects."
\textbf{Context-as-Memory}~\cite{yu2025context} aims for a similar geometric lock but simplifies the integration contract. It treats history as a flat pool filtered by camera frustum overlaps and directly concatenates the pose-consistent frames into the context window. This symmetric attention design proves that "pose-consistent evidence injection" alone is sufficient to stabilize look-back sequences.
\textbf{VRAG}~\cite{chen2025learning} extends this by introducing an \emph{in-context training} strategy. It retrieves frames based on agent state (position/orientation) and injects them with noise during training, explicitly forcing the diffusion model to rely on retrieved evidence to correct compounding errors.

Several works further specialize this for interactive environments. \textbf{WorldPack}~\cite{oshima2025worldpack} combines trajectory packing with retrieval, using fallback scoring (position/orientation) when FoV metadata is unavailable to maintain spatial consistency under strict context budgets. \textbf{Ctrl-World}~\cite{guo2025ctrlworld} and \textbf{MagicWorld}~\cite{li2025magicworld} utilize pose-triggered sparse sampling to anchor predictions during multi-step interactions, acting as stabilizers against structural drift. \textbf{SPMem}~\cite{wu2025spmem} formalizes this by grounding memory in an explicit 3D spatial structure, ensuring that retrieval queries return spatially-anchored content rather than just temporal neighbors.

\textbf{Semantic and Latent Caching.} 
Beyond geometry, consistency can be maintained by caching high-level features.
\textbf{Corgi}~\cite{wu2025corgi} distills the history buffer into a cached latent memory bank, storing keyframes as "identity anchors." Generation is conditioned on these cached latents to preserve subject appearance across scene cuts.
\textbf{MemoryPack}~\cite{wu2025memorypack} frames retrieval as \emph{semantic-guided selection}. It balances short-term continuity with long-term semantic alignment, selecting past content that remains "semantically necessary" for the narrative, effectively bridging the gap between compression and retrieval.

\paragraph{B. External-Corpus Retrieval: Realism via Exemplar Priors}
In this paradigm, retrieval does not look inward at the trajectory's past, but outward at a reference library. The goal is to borrow \emph{priors}—such as physical laws or motion patterns—from external video corpora, turning retrieval into a form of \emph{exemplar-conditioned generation}.

\textbf{Physics and Dynamics Injection.}
\textbf{DiT-Mem}~\cite{song2025ditmem} positions memory as a source of "World Knowledge." It queries reference videos that exemplify specific physical dynamics and extracts transferable priors (often via frequency-domain cues). These priors guide the generation process toward higher physical plausibility, distinguishing it from history-buffer retrieval which targets self-consistency.

\textbf{Motion Realism and Adaptation.}
\textbf{RAGME}~\cite{peruzzo2025ragme} targets motion quality via retrieval-augmented conditioning. It retrieves relevant clips from a large corpus to serve as grounding signals, allowing the backbone model to adapt to realistic motion cues with minimal overhead.
\textbf{MotionRAG}~\cite{zhu2025motionrag} makes this explicit for Image-to-Video tasks. It retrieves "motion exemplars," distills them via a specialized encoder, and injects the adapted features into the diffusion model. This "retrieve-and-transfer" approach allows the model to generalize to complex motion patterns by referencing external examples rather than memorizing them in weights.


\subsubsection{Memory Mechanism - Retrieval (Internal)}
Distinct from approaches relying on explicit external policies, another category of methods implements retrieval \textbf{implicitly within the attention mechanism}. 
Instead of managing the context buffer externally, these methods integrate the "retrieval" process directly into the attention calculation phases. 
By evaluating token-to-token relevance, the model dynamically selects or routes only the most pertinent tokens to participate in the computation.

This internal mechanism offers two distinct advantages:
\begin{itemize}
    \item \textbf{Fine-Grained Optimization:} The retrieval operates at a much finer granularity (often at the token or attention-head level), allowing for precise control over information access.
    \item \textbf{Deep Integration:} The process is tightly coupled with the network's layer-wise computations. This ensures that the temporal information flow is continuously optimized during every step of the generation, filtering out noise and reinforcing relevant historical signals dynamically.
\end{itemize}
Representative works in this domain typically include sparse attention mechanisms and dynamic token routing strategies.
We categorize these internal mechanisms into strategies that employ learnable sparse routing protocols and causality-preserving block attention. These methods allow the model to autonomously determine the topology of its information flow, effectively 'choosing' what to remember at each step.

\textbf{Mixture-of-Contexts} ~\cite{cai2025mixture} takes a different route: it treats $\mathcal{M}$ not as a static compressor but as a learnable sparse routing mechanism over the concrete token history. The video–text sequence is partitioned into semantically coherent chunks (shots, local frame windows, text spans), and each chunk is summarized into a representative key. For every query token, an Adaptive Mixture-of-Contexts (MoC) layer selects only a few informative chunks plus mandatory anchors (the caption and a local intra-shot window) under a causal routing mask that prevents backward edges and loop closures. Effectively, $\mathcal{M}$ transforms the full history $O_{1:t}$ into a query-dependent managed state $S_t$ by deciding which chunks are even visible to attention and which are completely ignored. The world state is still a concrete context of tokens, but it is aggressively thinned and structured by routing rather than by adding any new abstract latent.

%TODO: moba, sparse attention, block attention
\textbf{MoBA}~\cite{lu2025moba} reframes $\mathcal{M}$ as a learnable, causality-preserving routing-and-visibility operator over the concrete token history, rather than a fixed-length window or an explicit compression bottleneck. In this mapping, the raw history $O_{1:t}$ is simply the full autoregressive prefix (implemented as the standard attention memories $(K,V)$), which is partitioned into $n$ contiguous blocks; each block is summarized by a lightweight representative key (mean-pooled over block keys), and for each query token $q_t$ the router scores all past blocks and activates only a top-$k$ subset. The managed state is therefore query-dependent: $S_t(q_t)$ is the concrete context made accessible to computation, i.e., the subset of $(K,V)$ indexed by the routed blocks, plus mandatory anchors (always include the current block, and apply an intra-block causal mask to avoid leakage from block summarization). As a result, $\mathcal{M}$ is exactly the mechanism that turns $O_{1:t}$ into $S_t$ by deciding which chunks of history are visible to attention and which are ignored entirely; generation then operates on this thinned token context, with outputs combined via online-softmax~\cite{milakov2018online, liu2023blockwise} merging---thereby maintaining a fully token-based world state that is aggressively structured via sparse routing, obviating the need for abstract auxiliary variables.


\textbf{MoGA}~\cite{jia2025moga} advances internal retrieval for video generation by replacing coarse block-wise sparsity with a fine-grained token router. 
Instead of relying on heuristic spatial blocks, MoGA employs a lightweight learnable router to dynamically assign video tokens to semantically coherent groups (e.g., grouping a character's appearance across disjoint shots). 
Functionally, this acts as a \textbf{routing-based retrieval mechanism}: for every token, the network effectively ``retrieves" a specific subset of relevant peers from the global history to participate in attention computation. 
By confining dense attention within these dynamically routed groups, MoGA reduces the quadratic complexity to $\mathcal{O}(N^2/M)$, enabling the end-to-end generation of minute-level videos with context lengths exceeding 580k tokens.

\textbf{VMOBA}~\cite{wu2025vmoba} tailors internal retrieval for video diffusion models by introducing a layer-wise recurrent partition scheme (1D-2D-3D) and a threshold-based global selection strategy, which dynamically prioritizes the most salient query-key block interactions across the entire attention head, thereby adapting to diverse spatio-temporal patterns and varying query importance during training.

\subsubsection{Memory Mechanism - Update}
The \textbf{State Update} mechanism governs the evolution of the memory context after new content is generated. 
Unlike the retrieval process, which is driven by specific query demands (i.e., \textit{action-dependent}), the update phase is typically \textbf{action-agnostic}. 
It operates in the transition window after the completion of the current generation but before the next action is initiated.

Functionally, this phase manages the context set through fundamental set-theoretic operations: Insertion of the newly generated observation and Eviction of obsolete information to maintain buffer constraints. 
In current literature, these update policies are predominantly rule-based heuristics (e.g., First-In-First-Out, Sliding Window) rather than learning-based parameters. 
They ensure the memory structure remains bounded and orderly, preparing a consolidated state for the subsequent generation cycle without requiring foresight of the future action.
Practical implementations of this mechanism focus on hierarchical buffer management—distinguishing between short-term high-fidelity caches and long-term semantic stores—and iterative re-encoding heuristics that refresh memory states to mitigate generation drift.


\textbf{StreamingT2V}~\cite{henschel2025streamingt2v} makes the memory mechanism explicit by decomposing $\mathcal{M}$ into short-term and long-term context blocks wrapped around a standard text-to-video diffuser. A \textit{Conditional Attention Module} (CAM) maintains a short-term state by encoding the previous chunk into feature maps and letting the current noisy latents attend to them, enforcing smooth transitions at chunk boundaries. In parallel, an Appearance Preservation Module (APM) builds a long-term state from the first chunk, extracting high-level appearance and layout descriptors that are reused throughout generation to prevent drift. In our notation, $S_t$ is the pair of CAM and APM features, and $\mathcal{M}$ prescribes when CAM is refreshed (every chunk), when APM is kept fixed, and how both are injected into $G_\theta$ via cross-attention. Long-horizon consistency is thus achieved by carefully curating which concrete past frames enter the conditioning path, not by introducing an internal latent world state.

\textbf{Loong}~\cite{wang2024loong} shows that autoregressive LLM-style video generators can also be interpreted as Concrete State models. Videos are tokenized into discrete spatiotemporal codes and concatenated after text tokens into a single long sequence that a decoder-only Transformer models in a next-token fashion. The state $S_t$ exposed to $G_\theta$ is simply the prefix of previously generated text and video tokens, maintained by the standard KV cache. What Loong adds on top of this is a set of policies for how this concrete history is managed: progressive short-to-long training with re-weighted losses so early frames remain influential, and a ``re-encoding" strategy that decodes older chunks back to frames and re-tokenizes them to mitigate error accumulation. In our framework, $\mathcal{M}$ is instantiated by these context and re-encoding policies—how many past tokens are kept, when prefixes are rewritten, and how they are fed back into the model—while $G_\theta$ remains a pure next-token generator over the raw discrete history. The world state is therefore still a managed context buffer, not a compact abstract latent.

\textbf{FAR}~\cite{gu2025long} treats the state $S_t$ as a hierarchical cache of latent video tokens and their Transformer key--value (KV) states. Concretely, recent frames form a short-term state stored in an L1 KV cache at the standard resolution (e.g., 64 tokens per frame), while older frames belong to a long-term state stored in an L2 cache, where each frame is encoded with a much larger patchify kernel (e.g., 4 tokens per frame). $\mathcal{M}$ is realized as a multi-level KV cache update rule: every time a frame is decoded via flow matching, its clean latent is encoded into the L1 cache (with a special timestep marking it as clean context); once the short-term context window is exceeded, the earliest L1 frame is moved into the long-term context window and encoded into the compressed L2 cache, and the remaining frames in the L1 window are re-encoded to refresh their KV states. At each step, autoregressive retrieval simply attends over both L1 and L2 caches, so $S_t$ combines high-resolution recent memory with increasingly compressed long-range context, and the aggressive patchify scheme slows the growth of token context length as the video becomes longer.


\textbf{WorldWeaver}~\cite{liu2025worldweaver} introduces a \textit{Differential State Consolidation} strategy grounded in the concept of signal drift resistance, departing from naive FIFO queues or sliding windows. Recognizing that pure RGB representations are highly susceptible to semantic drift over long horizons, the framework incorporates multi-modal perceptual signals during the memory update phase. 
Specifically, for long-term state maintenance, it applies selective noise injection to the volatile RGB channels while strictly preserving the clarity of the Depth channels. 
This mechanism effectively decouples the World State into ``volatile texture'' and ``stable geometry'' components, forcing the model to rely on geometric features as structural anchors. 
This approach demonstrates that effective State Consolidation acts as an active process of Denoising and Selection rather than passive storage.







\subsubsection{Memory Mechanism - Explicit 3D Representations}
A distinct category of approaches diverges from latent-based memory by adopting \textbf{Explicit 3D Representations} (e.g., Point Clouds, 3D Gaussian Splatting, or Neural Radiance Fields) as the carrier of the memory state $S_t$. 
Unlike unstructured latent vectors, 3D representations possess intrinsic geometric structures that naturally support memory operations without requiring complex learning of retrieval policies.

In this paradigm, the abstract memory functions are mapped to explicit geometric operations:
\begin{itemize}
    \item \textbf{Retrieval as Rendering:} ``Retrieving" context for a specific viewpoint is functionally equivalent to Rendering or projecting the 3D state onto the target camera plane. This ensures that the retrieved context is always geometrically consistent with the desired query action (camera pose).
    \item \textbf{Update as Fusion:} The "Update" process is realized through 3D Registration and Fusion. When a new observation is generated, it is back-projected and merged into the global 3D structure.
\end{itemize}

By grounding the memory mechanism in 3D geometry, these methods inherently solve the challenges of multi-view consistency and spatial coherence, effectively turning the video generation problem into an incremental world reconstruction process.
Below, we highlight systems that leverage \textbf{point-based}, \textbf{volumetric}, and \textbf{Gaussian} representations. These works demonstrate how explicit geometry serves as a unifying medium for memory, enabling the seamless fusion of multi-view observations into a globally consistent world state.

In many recent systems, the 3D representation—such as point clouds \cite{yu2024viewcrafter, li2025vmem, ren2025gen3c, cao2025uni3c, wu2025genfusion, huang2025voyager, wang2025evoworld}, 3D Gaussians \cite{chen2025flexworld, zhang2025scene}, meshes \cite{yang2025matrix}, or implicit fields \cite{zhai2025stargen}—serves as an external and continuously evolving memory.
In this paradigm, the 3D structure is not treated as a static asset but as a persistent memory that is progressively refined over the course of generation. The process typically starts from an initial coarse reconstruction estimated from sparse observations, and the system repeatedly queries and updates this memory as new evidence becomes available. At each iteration, the current 3D representation is rendered from a newly selected viewpoint to reveal regions of ambiguity or missing content. A generative model synthesizes a novel view from this perspective, and the synthesized image is subsequently back-projected into the 3D representation to update geometry, appearance, and visibility information. Through this iterative render–generate–update cycle, the 3D memory becomes increasingly complete and internally consistent, allowing the system to accumulate scene knowledge over time and produce coherent multi-view predictions.

% Video World Models with Long-term Spatial Memory
\textbf{SPMem}\cite{wu2025video} extends the retrieval role into a cognitively inspired, multi-stream retriever that disentangles static geometry, short-term dynamics, and long-horizon episodic detail. Its spatial memory is a persistent TSDF-fused 3D voxel grid that encodes view-consistent, long-lived structure; importantly, the system does not retrieve voxels directly but renders the current trajectory’s viewpoints into 2D static condition maps, encodes and injects them through zero-initialized residual (\textit{ControlNet-style}) paths. In parallel, a working-memory window of recent frames is retrieved by recency and concatenated frame-wise (with their associated condition tokens) to preserve short-term motion continuity, while episodic memory accrues keyframes whenever a newly revealed scene area crosses a visibility threshold. In effect, spatial memory preserves a persistent world under arbitrary camera motion, rendered geometry provides structure awareness as a clean, drift-resistant condition, frame-wise fusion of recent context supports interactive control, and episodic recall restores fine details after long gaps while maintaining temporal consistency.

\subsubsection{Discussion: Trade-offs in Concrete State Management}
\label{sec:discussion_concrete_state}

The \textbf{Concrete Representation} paradigm relies on explicitly managing a history of observations to approximate the world state. While this approach benefits from high interpretability and visual fidelity by directly referencing past pixels, it faces critical trade-offs in computational efficiency, long-term consistency, and error propagation. We summarize these distinctions in Table~\ref{tab:concrete_state_comparison} and provide a detailed analysis below.

% \begin{table*}[t]
% \centering
% \caption{\textbf{Comparative Analysis of Concrete State Mechanisms.} We categorize methods based on their core mechanism for managing history, their impact on context length, and their primary trade-offs.}
% \label{tab:concrete_state_comparison}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lccccc@{}}
% \toprule
% \textbf{Mechanism} & \textbf{Core Operation} & \textbf{Context Length} & \textbf{State Fidelity} & \textbf{Computational Cost} & \textbf{Primary Limitation} \\ \midrule
% \textbf{Compression} & Downsample & Long & Low & Low & Information Loss \\
% \textbf{External Retrieval} & Explicit Query-Key Search & \textbf{Infinite (Virtual)} & High (Raw Pixels) & High (Search Overhead) & Manucrated bias \\
% \textbf{Internal Retrieval} & Attention Query-Key Search & Medium & High (Selected Tokens) & Medium & Optimization Difficulty \\
% \textbf{Consolidation} & Eviction & Medium & \textbf{High (Robust)} & Medium & Error Accumulation \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table*}
\input{main/tables/memory_mechanism}

\noindent\textbf{The Fidelity-Efficiency Frontier.}
A trade-off exists between maintaining high-fidelity history and managing computational cost.
\begin{itemize}
    \item \textbf{Compression-based methods} (e.g., FramePack~\cite{zhang2025packing}, RELIC~\cite{hong2025relic}) prioritize \textbf{efficiency} by aggressively downsampling history. While this allows for longer context windows within a fixed memory budget, it inherently introduces information loss. The ``compressed state" may lose fine-grained details required for precise re-visitation (e.g., the exact text on a sign seen 100 frames ago), leading to a trade-off between horizon length and local detail.
    \item \textbf{Retrieval-based methods} (e.g., WorldMem~\cite{xiao2025worldmem}, VRAG~\cite{chen2025learning}) prioritize \textbf{fidelity}. By storing raw or near-raw historical frames in an external buffer, they ensure that the model has access to pristine ground-truth information. However, this introduces a "Search and Selection" bottleneck. The effectiveness of the state depends entirely on the retrieval mechanism's ability to identify which past frame is causally relevant. Poor retrieval leads to ``Attention Dilution," where the model attends to visually similar but semantically irrelevant past frames, confusing the generation process.
\end{itemize}


\noindent\textbf{The Role of Explicit Geometry.} Methods utilizing explicit 3D Representations (e.g., SPMem~\cite{wu2025video}) offer a unique solution to the consistency problem. By enforcing geometric constraints (e.g., via a voxel grid or point cloud), they solve the "Object Permanence" problem by definition—an object cannot disappear if its 3D voxels persist. However, this comes at the cost of visual domain gap and rigidity. Reconstructing a perfect 3D representation from generated video is error-prone, and artifacts in the 3D structure (e.g., ``floaters" in Gaussian Splatting) can degrade the visual quality of future frames, often resulting in a "synthetic" look compared to pure 2D approaches.


\subsubsection{Limitations}
The \textbf{Concrete Representation} paradigm marks a significant evolution in long-video generation, shifting the focus from simply training larger backbones to explicitly engineering the flow of temporal information. 
By formalizing the ``State'' as a managed collection of historical observations ($S_t \equiv \mathcal{M}(O_{1:t})$), these methods successfully extend the generation horizon of diffusion models from seconds to minutes. 
The primary advantage of this approach lies in visual Fidelity. By allowing the model to directly attend to past pixels (or their compressed tokens), these systems maintain high texture consistency and identity preservation, as demonstrated by retrieval-heavy architectures like WorldMem~\cite{xiao2025worldmem} and WorldWeaver~\cite{liu2025worldweaver}.

However, relying on historical observations as the sole carrier of the world state introduces intrinsic limitations that prevent these systems from becoming robust General World Simulators. 
The most critical flaw is Noise Accumulation (or ``Autoregressive Drift''). 
Since the state is constructed recursively from generated outputs ($S_{t+1} \leftarrow S_t \cup \{\hat{O}_{t+1}\}$), there is no distinction between ``ground truth physics'' and ``generated hallucinations.'' Once the generator $G_\theta$ produces a visual artifact, this error is committed to the concrete memory, and subsequent retrieval steps recall this corrupted information as valid context, forming a feedback loop that amplifies errors. 
Furthermore, despite sophisticated retrieval mechanisms, the underlying video generators operate within a finite context window, creating a fundamental trade-off between selection difficulty and attention dilution. 
Heuristic metrics often fail to capture long-range causal dependencies, and filling the window with diverse patches can dilute the attention mechanism, causing the model to lose focus on immediate local dynamics. 
Finally, maintaining a concrete state is computationally inefficient, as the memory size generally scales linearly with history complexity (KV Cache), contrasting with abstract state paradigms that compress history into constant-size latent vectors for theoretically infinite-horizon simulation.

\subsection{Explicit Latent State}
\subsubsection{Definition}
In contrast to the ``Concrete" paradigm, which manages raw history via external policies, this paradigm seeks to construct the world state through \textbf{Internalized Compression}. 
Here, the model does not maintain a buffer of raw observations; instead, it maintains a globally updating latent variable $S_t$ that acts as a comprehensive mathematical summary of the history.

In this framework, the ``State'' $S_t$ is an abstract, compact vector (or set of vectors) evolved by the network's internal recurrence. 
Crucially, the update mechanism is no longer a heuristic rule (like retrieval or FIFO) but a \textbf{learnable transition function} parameterized by $\theta$. 
% The generation process becomes a unified flow where the model simultaneously evolves its internal state and renders the visual observation:
% \begin{equation}
%     S_{t+1}, O_{t+1} = F_{\theta}(S_{t}, A_{t}, \dots)
% \label{eq:explicit state_base}
% \end{equation}

% Under this formulation, the model performs a \textbf{Joint Parameterization} of the World Model components. The parameters $\theta$ must simultaneously satisfy two objectives:
% \begin{itemize}
%     \item \textbf{(1) Transition Model (Dynamics):} Learning how $S_t$ evolves to $S_{t+1}$ to maintain temporal logic and physical consistency.
%     \item \textbf{(2) Observation Model (Rendering):} Learning how to decode the abstract state $S_{t+1}$ into high-fidelity pixels $O_{t+1}$.
% \end{itemize}

% \noindent\textbf{Note on Hybrid Inputs:} To ensure visual continuity and retain high-frequency details, practical implementations often permit the model to access historical observations $O_{1:t}$ alongside the abstract state. However, the defining characteristic remains that the \textit{dynamics} are propagated through the latent state evolution:
% \begin{equation}
%     S_{t+1}, O_{t+1} = F_{\theta}(S_{t}, A_{t}, O_{1:t})
% \label{eq:explicit state_hybrid}
% \end{equation}

Depending on how the transition function is architecturally implemented relative to the generation model, we categorize existing works into three sub-paradigms:

\begin{itemize}
    \item \textbf{(1) Intrinsic Hidden States:} 
    Methods where the transition function is intrinsically fused within the generation model. 
    The dynamics are learned implicitly as the model processes the sequence, with the state $S_t$ acting as the transient memory of the model.

    \item \textbf{(2) Modular Latent States:} 
    Methods where the transition function is structurally distinct—often formalized as a separate module—but is trained jointly with the generation model end-to-end. 

    \item \textbf{(3) Parametric States:} 
    Methods where a subset of the model's parameters $\theta$ themselves behave as the ``state''. 
    As the model processes the video, these parameters are dynamically adjusted to encode the specific information of the current context.
\end{itemize}


\subsubsection{Intrinsic Hidden States}
Fundamentally, works in this category formulate the video modeling process by constructing an \textbf{internal causal linear system}. 
The primary objective of this system is to capture long-term temporal dependencies efficiently. 
Crucially, the \textit{recursive updatability} of the causal linear formulation allows the internal hidden state to function inherently as a state transition model. 
Instead of re-reading the entire history, the system evolves a fixed-size state via linear recurrence, simulating the continuous evolution of world dynamics within the network's backbone.
This category encompasses approaches that leverage \textbf{State Space Models (SSMs)}, \textbf{Linear Attention mechanisms}, and \textbf{Recurrent Neural Networks (RNNs)} to embed the state transition directly into the backbone's computational graph, allowing for efficient $O(1)$ inference while maintaining long-term dynamics.



MALT~\cite{yu2025malt} is a concrete example of abstract state. It introduces a learned memory vector $h$ that is refreshed segment-by-segment via a Markovian rule $h^n = f(h^{n-1}, z_0^n)$ implemented by temporal attention layers. The same Transformer plays a dual role: for standard diffusion timesteps it acts as a denoiser, while a special $t{=}0$ input switches it into a ``memory encoder'' mode that writes into $h$. In our terminology, $h$ \emph{is} the abstract state $S_t$, and the internal recurrent update $f$ is the $U$ module; both are fully internal to the backbone. Because this state is compact and trained end-to-end, MALT can compress very long histories into a small vector and exhibits strong length generalization, generating minute-long videos even when trained only on short clips.

Video world models with State-Space Model~\cite{po2025long,oshima2024ssm} exemplify the implicit internalization route. They scan sequences with structured state-space layers that advance a fixed-dimensional hidden state using linear, causal recurrences, often organized in blocks to avoid degradation over extremely long chains, and complement this with local frame-window attention to capture short-term dynamics. In this view, the SSM hidden state itself is $S_t$: it accumulates information as the video progresses and is reused when predicting later frames. This yields constant-size memory and efficient long-context modeling, while empirical results show quality comparable to full-context causal attention on retrieval-style tasks but at substantially lower computational and memory cost.

SANA-Video~\cite{chen2025sana} realizes a closely related design by replacing standard attention with block-wise causal linear attention. Instead of maintaining a growing KV cache, it keeps cumulative key–value statistics that are updated as each temporal block is processed, effectively turning the KV buffer into an additive memory state. Within our framework, this additive KV accumulator is the latent $S_t$, and the linear-attention update rule is the internal $U$; both are learned jointly with the rest of the model. This gives autoregressive video generation with constant memory footprint and runtime that scales linearly with length, yet preserves performance close to full self-attention, all without requiring any external memory management or retrieval module.

Recurrent Autoregressive Diffusion (RAD)~\cite{chen2025recurrent} integrates an explicit \textbf{LSTM-based recurrent block} into the diffusion transformer architecture to serve as a global memory container for long-term generation. RAD systematically investigates the frequency of state updates, demonstrating that \textbf{frame-wise autoregression} (updating state at every frame) significantly outperforms chunk-wise approaches in maintaining fine-grained spatiotemporal consistency, as it avoids the information loss associated with discrete chunk boundaries. To address the training inefficiency inherent in sequential recurrence, RAD introduces a \textbf{hidden state pre-fetch mechanism}, which decouples the recurrent state computation from the parallel attention operations, enabling efficient training on long video sequences without sacrificing the benefits of dense state updates.


\subsubsection{Modular Latent States}
Methods in this category construct a \textbf{standalone transition model} that is structurally distinct from the visual generation backbone. 
Instead of fusing dynamics into the video model, these approaches maintain an explicit latent state that evolves via recurrent updates. 
A critical aspect of this paradigm is the design of specialized \textbf{joint training schemes}, which ensure that the abstract dynamics modeled by the external module are effectively aligned with and decoded by the video model during end-to-end optimization.
We illustrate this paradigm through frameworks that utilize \textbf{multimodal LLMs} or \textbf{specialized prior networks} as distinct transition modules. By structurally decoupling the dynamics modeling from visual rendering, these methods achieve a rigorous factorization of the world model components.


Owl-1~\cite{huang2024owl} offers a different form of explicit coupling, where the transition model is implemented by a separate world model rather than by the video backbone itself. The system maintains a compact latent world state $s_t$ outside the video diffuser; after each short clip is rendered, a multimodal LLM inspects $(s_t, o_t)$, summarizes the newly observed world dynamics into a natural-language description $d_t$, and then maps $(s_t, d_t)$ to the next state $s_{t+1}$. The subsequent video clip is generated by conditioning the diffusion model on $s_{t+1}$ together with short-range visual cues such as the last frame of the previous clip. From our GWM perspective, $s_t$ is the abstract state, the LLM-based controller implements the $U$ (and partially $R$) modules in a high-level symbolic space, and $G_\theta$ remains a standard video generator that only needs to see the current state, not the entire past buffer.

Pack and Force~\cite{wu2025pack} exemplifies the \textit{explicit coupling} strategy within the abstract state paradigm. It introduces \textbf{MemoryPack}, a hierarchical mechanism that constructs a compact, recurrent state variable to manage long-term dependencies. Specifically, the \textit{SemanticPack} module functions as an external recurrent network: it iteratively updates a long-term memory vector $\psi_n$ by compressing historical segments ($x^n$) via self-attention and aligning them with global guidance (text and image) via cross-attention (Equation 1). Unlike methods that rely solely on raw context windows, this evolving vector state $\psi_n$ effectively encapsulates minute-level temporal consistency and is injected into the diffusion transformer (MM-DiT) as an additional conditioning signal, enabling the model to generate long-form videos with linear complexity while mitigating error accumulation.





\subsubsection{Parametric States}
This paradigm represents a fundamental shift by treating a subset of the model's parameters not as fixed constants, but as \textbf{dynamic, input-dependent variables}. 
Instead of storing history in activation buffers, these methods configure specific model weights to serve as the carrier of the state. 
As the video stream is processed, these parameters are continuously \textbf{updated based on the input}. 
Consequently, the model effectively "learns" and memorizes the specific dynamics of the current context on-the-fly, encoding the history directly into the plasticity of its architecture.
Recent innovations in this domain explore \textbf{Test-Time Training (TTT)} and \textbf{meta-optimization}, where the network's weights themselves serve as the fluid medium for state storage. These works challenge the traditional separation between training and inference, treating the update process as an online learning problem.

One-Minute Video Generation with Test-Time Training (TTT)~\cite{dalal2025one} introduces a novel RNN layer where the hidden state is not a fixed-size activation vector but the weights $W_t$ of a neural network (specifically, a two-layer MLP). The state update mechanism is formulated as an online optimization step: processing a new token $x_t$ is equivalent to updating the weights $W_t$ via gradient descent on a self-supervised reconstruction loss $\ell(W; x_t)$. By embedding these TTT layers into a pre-trained Diffusion Transformer (DiT), the model effectively "trains itself" on the fly to compress the historical context into the dynamic weights of the hidden MLP. This design overcomes the capacity bottleneck of traditional matrix states in linear attention, enabling the generation of long-form videos (e.g., one minute) with complex multi-scene narratives while maintaining linear complexity.


% Nested Learning: The Illusion of Deep Learning Architectures

Nested Learning (NL)~\cite{behrouz2025nested} provides a rigorous theoretical generalization of the "Matrix-Valued State" paradigm. It conceptualizes the model not as a fixed function, but as a hierarchy of \textbf{nested optimization problems}, where the state $S_t$ consists of the \textbf{dynamic weights} of an internal neural module. Crucially, unlike standard optimization algorithms (e.g., SGD) that use fixed update rules, NL proposes that the state update $\Delta S_t$ (the "gradient" or adjustment) is produced by a learnable \textbf{MLP-based transition function} (referred to as a "Deep Optimizer"). This allows the world model to learn \textit{how} to update its internal physics parameters based on the incoming observation stream, effectively turning the dynamics function $F$ into an adaptive, context-aware optimizer.


\subsubsection{Discussion}
\label{sec:discussion_abstract_state}

The three sub-paradigms of \textbf{Abstract Representations}---Intrinsic, Modular, and Parametric---represent fundamentally different mathematical answers to the question: \textit{``What is the optimal vessel for carrying the World State $S_t$?''}
While they share the common goal of internalizing history into a compact form to achieve infinite-horizon simulation, they diverge significantly in their architectural trade-offs between inference efficiency, memory capacity, and physical interpretability. We summarize these distinctions in Table~\ref{tab:abstract_state_comparison} and provide a detailed comparative analysis below.

\begin{table*}[t]
\centering
\caption{\textbf{Comparative Analysis of Abstract State Paradigms.} We categorize methods based on the mathematical form of their state $S_t$, their inference complexity relative to sequence length $L$, and their primary strengths and limitations.}
\label{tab:abstract_state_comparison}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Paradigm} & \textbf{State Form ($S_t$)} & \textbf{Inference Cost} & \textbf{Memory Capacity} & \textbf{Disentanglement} & \textbf{Primary Challenge} \\ \midrule
\textbf{Intrinsic Hidden States} & Activation Vectors & Low & Low  & Weak (Implicit) & Long-term Forgetting \\
\textbf{Modular Latent States} & External Module Output & Moderate & Moderate & \textbf{Strong} (Structural) & Alignment \& Complexity \\
\textbf{Parametric States} & Network Weights & High & High & Weak (Implicit) & Training Stability \\ \bottomrule
\end{tabular}%
}
\end{table*}

\noindent\textbf{The Trade-off between Inference Efficiency and Memory Capacity.}
The most significant differentiator among these paradigms is the computational cost of maintaining the state versus the amount of information it can store.
\begin{itemize}
    \item \textbf{Intrinsic Hidden States} (e.g., MALT~\cite{yu2025malt}, SANA~\cite{chen2025sana}) prioritize \textbf{efficiency}. By storing history in recurrent activation vectors, they achieve $\mathcal{O}(1)$ inference complexity, making them the fastest option for real-time generation. However, they suffer from a \textit{capacity bottleneck}: a fixed-size vector cannot losslessly compress an infinitely growing history, leading to the "vanishing gradient" problem where early causal details (e.g., a door opened 1000 frames ago) are gradually overwritten.
    \item \textbf{Parametric States} (e.g., TTT~\cite{dalal2025one}) prioritize \textbf{capacity}. By encoding history directly into the high-dimensional weight space of a neural network (via online gradient updates), they unlock a massive storage capacity that far exceeds activation vectors. This allows for instance-specific adaptation, effectively "fine-tuning" the physics model on the fly. The penalty is \textit{computational cost}: calculating gradients and updating weights during inference introduces significant latency.
\end{itemize}

\noindent\textbf{The Dilemma of Disentanglement.}
Another critical dimension is whether the ``Dynamics'' ($S \to S'$) and ``Rendering'' ($S \to O$) are entangled.
\begin{itemize}
    \item \textbf{Intrinsic and Parametric} approaches tend to be \textbf{entangled}. The state (whether vector or weight) is an implicit, distributed representation optimized solely for minimizing reconstruction loss. This "Black Box" nature makes it difficult to interpret whether the model has learned a correct physical law or is simply overfitting to texture statistics.
    \item \textbf{Modular Latent States} (e.g., Owl-1~\cite{huang2024owl}) prioritize \textbf{disentanglement}. By offloading state management to a separate module (e.g., an LLM or a scene graph updater), these methods enforce a structural separation between the physical simulation and the visual decoding. While this increases architectural complexity and introduces alignment challenges during joint training, it offers the most promising path towards interpretable and controllable World Simulators where users can explicitly intervene on the state (e.g., "remove the table") without breaking the visual consistency.
\end{itemize}

\noindent\textbf{Guideline for Selection.}
Current evidence suggests a clear heuristic for model selection: for applications requiring low-latency real-time interaction (e.g., video games), \textbf{Intrinsic} architectures remain the gold standard due to their speed. For scenarios demanding high-fidelity physical reasoning and long-term consistency (e.g., offline planning or simulation), \textbf{Modular} or \textbf{Parametric} approaches offer superior robustness despite their higher computational overhead.


\subsubsection{Limitations}

The \textbf{Abstract Representation} paradigm represents the theoretical ideal of a World Simulator, effectively decoupling computational cost from simulation length through internalized compression. By evolving a compact latent state $S_t$ rather than managing raw history, methods like MALT~\cite{yu2025malt} and TTT~\cite{dalal2025one} achieve $O(1)$ inference complexity and linear scalability, mimicking the efficient state-space reasoning of biological intelligence. 

However, this abstraction introduces significant stability and interpretability challenges. Foremost is the issue of Catastrophic Forgetting and vanishing gradients; unlike concrete memory that allows explicit retrieval, abstract states must compress infinite history into a fixed-capacity vector, often causing the signal from initial conditions to decay exponentially and leading to semantic drift over long horizons. Furthermore, these models suffer from a ``Black Box'' Interpretability Gap, as the high-dimensional latent state lacks explicit semantic grounding, making it difficult to verify encoded physical attributes or diagnose failures compared to human-readable frame buffers. Finally, Optimization Instability remains a critical bottleneck, as jointly training transition and observation models frequently leads to posterior collapse, where the generator ignores the global state in favor of local cues, requiring fragile training curricula to enforce long-term consistency.

==> legacy/5_memory_categories.tex <==
\section{Memory Categorization}\label{sec:Categorization}

Our R-D-G-E-U framework defines the "how" of a Generative World Model, decomposing the memory evolution function $F$ into a cognitive cycle. The specific design and implementation of these modules are not arbitrary; they are driven by the fundamental properties that a GWM must satisfy to be effective.

We identify two primary axes of design, which we use to categorize memory mechanisms:

\begin{itemize}
    \item \textbf{Persistence and Efficiency:} A GWM must manage a potentially infinite history ($M_t$) with finite computational resources. This is primarily a problem of \textbf{storage compression}.
    \item \textbf{Causality and Coherence:} A GWM must evolve in a temporally consistent and logical manner, where past events correctly influence future outcomes. This is a problem of \textbf{information management} and flow.
\end{itemize}

These two challenges are primarily addressed by two distinct pairs of modules in our framework:

\begin{itemize}
    \item \textbf{Compressive Memory (E/D Modules)} mechanisms focus on the \textit{Persistence} problem by efficiently encoding and decoding the memory state.
    \item \textbf{Dynamic Memory (R/U Modules)} mechanisms focus on the \textit{Causality} problem by dynamically retrieving from and updating the memory state.
\end{itemize}

\subsection{Compressive Memory: Solving for Persistence (E/D)}

The first category of mechanisms addresses the challenge of \textbf{persistence}---how to enable infinite or long-horizon generation within finite computational (especially spatial) constraints. The total memory $M_t$ is unbounded, but the GPU memory is not.

This problem is the primary domain of the Encoding (E) and Decoding (D) modules. Their goal is to compress the generated content $G_t$ into a compact representation $E_t$.

These modules are primarily concerned with the computational complexity bottleneck: in an infinite generation process, the context length $L$ grows linearly with time ($L \propto t$). Since attention mechanisms have a computational and memory complexity that is typically $O(L^2)$, this unbounded linear growth in $L$ creates an intractable bottleneck. The primary purpose of Compressive Memory (E/D modules) is therefore to break this linear dependency by limiting the context length $L$ to a manageable, fixed upper bound.



\begin{itemize}
    \item \textbf{Framepack~\cite{zhang2025packing}:} 
    \textbf{What it does:}
    is a neural network structure designed to progressively compress the input frame context (i.e., the history) based on "importance". In its time-proximity-based implementation, it assigns variable context lengths to different frames by manipulating the patchify kernel sizes, granting more important frames (e.g., the most recent ones) a longer context.
    
    \textbf{Correspondence to the memory component:}
    In the context of our GWM framework, FramePack functions as a Compressive Memory mechanism, corresponding to the E (Encoding) and D (Decoding) modules. It provides an intelligent, importance-based solution for encoding the vast historical memoryinto a fixed-size, computationally manageable context for the Generative Engine (G).
    
    \textbf{Effectiveness:}
    This design allows the model to process "thousands of frames" during inference while ensuring the total context length converges to a "fixed upper bound". This significantly improves efficiency.
    
    \textbf{Coupling with the base model:}
    Regarding model integration, the FramePack compression module is implemented as an extension of the model's native patchify layers. While a model cannot use this compressed format without modification, the paper shows that existing pretrained models can be finetuned to adopt the FramePack structure, suggesting a low adaptation cost.
\end{itemize}

\begin{itemize}
    \item \textbf{LoVic~\cite{jiang2025lovic}:} 
    \textbf{What it does:}
    LoViC is a DiT-based framework for long-form text-to-video generation. Its core module, FlexFormer, is a context autoencoder that compresses long video–text history into a short sequence of context tokens using a single learnable query token, replicated under different compression strategies (uniform/linear/logarithmic).
    
    \textbf{Correspondence to the memory component:}
    Under our GWM view, FlexFormer in LoViC serves as a Compressive Memory module. It mainly instantiates the E (Encoding) stage of the memory cycle, with its decoder used during autoencoder training and reconstruction stage (D). In practice, past video segments and their captions are first turned into latent tokens by the base video VAE and text encoder, then FlexFormer condenses this long multi-modal history into a much shorter sequence of context tokens. At generation time, these context tokens are concatenated with the current segment’s tokens and passed through the DiT’s self-attention blocks, so that the Generative Engine (G) can condition on long-range video–text history without directly attending over all original tokens.
    
    \textbf{Effectiveness:}
    Token-level compression enables LoViC to condition on long videos (up to 771 frames across clips in experiments) while keeping memory usage and runtime practical. On Panda-70M it outperforms strong DiT-based baselines (CausVid, SkyReel-V2, FramePack, LTX-Video-V0.9.6) on prediction, interpolation and retrodiction, and—with an appropriate linear compression strategy—can match or even surpass a non-compressed LTX-Video baseline that uses the full conditioning video.
    
    \textbf{Coupling with the base model:}
    LoViC keeps the base DiT (LTX-Video-V0.9.0) largely unchanged and attaches FlexFormer as a lightweight external context encoder. Context tokens from FlexFormer are simply concatenated with the original tokens at each self-attention layer. FlexFormer is first trained as an autoencoder and then frozen, after which the DiT is fine-tuned to consume its compressed context, implying a relatively low adaptation cost and modular integration.
\end{itemize}




\subsection{Dynamic Memory: Solving for Causality (R/U)}

The second category of mechanisms addresses \textbf{causality}. It is not enough to simply store memory; the GWM must manage its evolution to ensure a logical flow of cause and effect. This concept of causality is the primary domain of the Retrieval (R) and Update (U) modules, which function as the "gatekeepers" of information flow. We can analyze them as two distinct phases of causal management:

\subsubsection{A Priori Causal Management (The $R$ Module)}

%% 11/13 ZhiFei TODO: 再改，写得还是太bullet point了，割裂感很重
Retrieval mechanisms are the a priori (proactive) managers of causality: they answer “given the current action ($A_t$), what specific information from the entire past ($M_t$) is causally relevant to generating the next state ($G_t$)?” If the retrieved cause ($R_t$) is noisy, irrelevant, or incomplete, the effect ($G_t$) will be logically incoherent with the past. In practice, advanced (R) modules therefore purify ($M_t$) into a concise, high-signal context ($R_t$) that forms a strong causal basis for generation, subject to tight capacity and compute budgets. A useful way to view this is a constrained selection objective, \[
\max_{\lvert R_t\rvert \le B}\; \mathbb{E}\!\left[\log p\!\left(G_t \mid R_t, A_t\right)\right]
\] where geometric visibility, temporal ordering, redundancy, and representational compatibility act as practical surrogates for causal utility. Here, (B) denotes the retrieval budget (e.g. select at most (B) memory items). Taking it all together, persistent-world behavior, structure awareness, interactive controllability, and temporal consistency are not mere by-products; they are \textbf{failure tests} for (R).


WORLDMEM~\cite{xiao2025worldmem} operationalizes this as \textbf{state- and time-aware retrieval} over explicit memory units ( {I,p,t} ) comprising past first-person frames, camera poses, and timestamps. At each step, a ranking objective approximated by Monte-Carlo field-of-view (FOV) overlap and temporal distance promotes those historical views that are both visible and temporally pertinent; a redundancy pass prunes duplicates by feature similarity. From the model's perspective, the retrieved set does not just enter self-attention; it is routed through a dedicated memory block where current latent queries attend to memory keys/values with pose–time embeddings, ensuring representational alignment between “what is being asked now” and “what was seen then.” This pose/time-conditioned selection along with the dedicated memory block is what converts “a large, noisy past” into “the causes that matter,” and it keeps a consistent world behavior: when the camera wanders and later revisits a site, the system recalls the relevant historical appearance and state, reinstating layout and detail well beyond the base context window. The timestamp (t) is not incidental—ablation shows that without time conditioning, the retriever conflates “same place at different times,” yielding anachronistic reconstructions.

Context-as-Memory~\cite{yu2025contextasmemory} reaches a similar causal goal with a different retrieval contract: it treats all past frames as an explicit pool and uses camera geometry to pick only those whose FOV overlaps the current target pose, followed by simple de-duplication (dropping adjacent, duplicates and preferring non-adjacent, informative frames). Rather than projecting retrieved content via a dedicated block, the method concatenates the pose-aligned context frames with the current (noisy) tokens along the frame dimension so they participate symmetrically in spatiotemporal self-attention. This direct assembly of pose-consistent evidence yields robust interactive control: the memory naturally supports “look-away and look-back” sequences, where revisited regions reappear consistently because (R) injects exactly those frames that causally constrain the anticipated view. Empirically, the effect strengthens with larger but well-filtered contexts, given fixed attention budgets.

SPMem\cite{xxx} extends the (R) role into a cognitively inspired, multi-stream retriever that disentangles static geometry, short-term dynamics, and long-horizon episodic detail. Its \textbf{spatial memory} is a persistent TSDF-fused 3D voxel grid that encodes view-consistent, long-lived structure; importantly, the system does not retrieve voxels directly but renders the current trajectory’s viewpoints into 2D static condition maps, encodes and injects them through zero-initialized residual (ControlNet-style) paths, an architectural choice that enforces spatial and structural awareness without overwhelming the generator with raw geometry. In parallel, a \textbf{working-memory} window of recent frames is retrieved by recency and concatenated frame-wise (with their associated condition tokens) to preserve short-term motion continuity, while \textbf{episodic memory} accrues keyframes whenever newly revealed scene area crosses a visibility threshold. In effect, spatial memory preserves a persistent world under arbitrary camera motion, rendered geometry provides structure awareness as a clean, drift-resistant condition, frame-wise fusion of recent context supports interactive control, and episodic recall restores fine details after long gaps while maintaining temporal consistency.

These retrieval designs reveal several clear patterns. First, (R) must score candidates with such signals: FOV overlap and pose are essential for viewpoint causality; timestamps and simple recency priors encode temporal causality; and redundancy suppression protects limited attention from low-value repeats. Second, representational alignment matters as much as selection: WORLDMEM’s clear-latent cross-attention, Context-as-Memory’s frame concatenation, and SPMem’s ControlNet-style conditioning are all effective ways to make retrieved evidence legible to the generator. Third, structure-aware retrieval is increasingly important: beyond explicit voxel stores, systems like WorldWeaver\cite{xxx} use depth-centric memory because depth is more drift-resistant than color; using depth (or other geometry-proximal cues) as the “clean” signal inside (R) naturally extends SPMem’s philosophy. Finally, (R) is tightly coupled with the update module (U): SPMem’s visibility-gated episodic archiving and WORLDMEM’s timestamped writes determine what will even be available later—good (R) relies on disciplined (U), and vice versa. The overarching lesson is that for persistent-world re-rendering, retrieval must be causality-aware, not merely recency- or similarity-driven.

\cite{}

%%%%%%%%%%%%%%%%%%%%%%% paper summary %%%%%%%%%%%%%%%%%%%%%
% \begin{itemize}
% \item \textbf{WORLDMEM~\cite{xiao2025worldmem}:}
% \textbf{What it does:}
% it augments an interactive video world simulator with an explicit \textbf{external memory bank} to achieve long-term, view-consistent rollouts. Built on a conditional DiT with Diffusion Forcing, it continuously stores previously generated first-person frames together with their camera poses and timestamps, and conditions future denoising steps on a small set of retrieved “memory frames” to maintain world coherence.

% \textbf{Correspondence to the memory component:}
% The method instantiates memory as a set of \textbf{memory units} \(M = \{I, p, t\}\), each containing a past frame \(I\), its pose \(p\), and timestamp \(t\). A dedicated \textbf{memory block} performs cross-attention where current latent tokens act as queries and memory frames as keys/values, with pose–time state embeddings added to both. A retrieval algorithm ranks memory units by Monte Carlo–estimated FOV overlap and temporal distance, then prunes redundant ones by feature similarity, realizing a structured, content- and geometry-aware addressing scheme.

% \textbf{Effectiveness:}
% Conditioning on memory units allows WORLDMEM to \textbf{reconstruct previously seen views after long temporal gaps} and preserve 360° scene consistency, substantially improving the visual quality and cosistency over DF-only baselines both within and far beyond the context window on Minecraft and RealEstate10K data.

% \textbf{Coupling with the base model:}
% The memory bank is external but \textbf{tightly integrated} into the diffusion architecture. Retrieved memory frames are injected as “clear” latents alongside noisy frames within the model, and are only visible through the memory blocks (masked out from temporal self-attention). The entire system—DiT backbone plus memory blocks and state embeddings—is trained end-to-end.


% \item \textbf{Context-as-Memory~\cite{yu2025contextasmemory}:}
% \textbf{What it does:}
% Context-as-Memory targets \textbf{scene-consistent interactive long video generation} by treating all previously generated frames as an explicit memory pool. Built on a camera-conditioned latent video diffusion model, it stores historical frames and then \textbf{concatenates selected context frames with the current predicted frames along the frame dimension} as input tokens, so the model can reuse past views when synthesizing new ones.

% \textbf{Correspondence to the memory component:}
% Here, memory is instantiated directly as \textbf{raw context frames plus their camera poses}. A lightweight \textbf{Memory Retrieval} module selects a small subset of relevant frames from the (potentially infinite) history by checking FOV overlap between the target camera pose and past camera poses, followed by simple redundancy pruning (e.g., dropping adjacent near-duplicates, optionally preferring far-in-time/space frames). 

% \textbf{Effectiveness:}
% By conditioning on sufficiently rich, pose-aligned history, Context-as-Memory can \textbf{revisit previously seen regions with high consistency} when the camera “rotates away and comes back,” significantly improving the generation quality. Larger context sizes and better retrieval (FOV + non-adjacent filtering) systematically strengthen memory, and the approach generalizes to open-domain setups while keeping global layout consistent.

% \textbf{Coupling with the base model:}
% The memory is external at the storage/retrieval level: retrieved context latents are concatenated with noisy prediction latents and participate equally in the model’s spatiotemporal self-attention. The diffusion network is trained end-to-end under this context-conditioning scheme (with camera control injected via a camera encoder), while Memory Retrieval itself is a deterministic rule-based module that selects which historical frames enter the model.

% \item \textbf{SPMem:}
% \textbf{What it does:}
% SPMem introduces a \textbf{multi-modal external memory system inspired by three distinct forms of human memory}, spatial, working, and episodic memory, which could enable long-horizon, view-consistent, and detail-preserving video generation in dynamic 3D environments. 
% It decouples static scene geometry from dynamic content and uses distinct memory structures to store and retrieve each type of information.

% \textbf{Correspondence to the memory component:}
% The memory system comprises three explicitly defined components, each with a dedicated representation and retrieval strategy:
% (1) \textbf{Spatial memory} is represented as a \textbf{persistent TSDF-fused 3D voxel grid} that stores temporally consistent static geometry via weighted averaging of signed distances D(v) and confidence weights W(v) across frames. Dynamic content is inherently suppressed due to inconsistent depth observations. During generation, this memory is \textbf{retrieved not as raw voxels but via view synthesis}: for each target frame along the input camera trajectory, the system \textbf{renders a 2D static condition image} from the current TSDF volume (with unobserved regions masked as black), which is then encoded by a pre-trained 3DVAE into \textbf{condition latents}. These latents are processed by a dedicated \textbf{condition DiT} (initialized from CogVideoX) and injected into the main diffusion backbone through \textbf{zero-initialized residual connections} (ControlNet-style), thereby enforcing geometric consistency of static structures across novel viewpoints and long-term rollouts.
% (2) \textbf{Working memory} is represented as a \textbf{sliding window of the most recent k+1 video frames}. It is \textbf{retrieved by recency} and explicitly injected into the diffusion model by concatenating both the context video tokens and their corresponding condition tokens with the target tokens along the frame dimension. 
% This ensures \textbf{frame-level alignment between dynamic content and static scene conditions}, allowing the model to generate temporally coherent motion while preserving geometric consistency across the short-term context. 
% (3) \textbf{Episodic memory} is represented as a \textbf{growing set of selected historical RGB frames}. 
% Frames are \textbf{added incrementally} to the memory set based on a visibility-driven criterion: during generation, if the area of newly revealed (previously unobserved) scene regions, which computed via a mask-based visibility check exceeds a predefined threshold, the current frame is archived as a representative “memory slot.” 
% At inference time, \textbf{all stored episodic frames are retained and used as reference views}; they are encoded by the 3DVAE, patchified into \textbf{reference tokens}, and integrated into the diffusion process via a dedicated \textbf{historical cross-attention} module, where the current video tokens serve as queries and the reference tokens serve as keys and values. This enables the model to \textbf{retrieve fine-grained visual details from past keyframes} when synthesizing novel views, even after long temporal gaps.

% \textbf{Effectiveness:}
% SPMem achieves long-horizon scene consistency, fine-grained detail preservation, and temporally coherent dynamics by synergizing three complementary memory streams. The spatial memory enforces geometric stability of static structures across arbitrary camera motions; the working memory ensures short-term motion continuity through explicit temporal context; and the episodic memory enables high-fidelity recall of visual details during camera re-visits—even after long temporal gaps. Together, they allow the model to faithfully simulate interactive worlds where dynamic agents evolve over time while the environment remains globally consistent.

% \textbf{Coupling with the base model:}
% The memory system is externally maintained but deeply integrated into a conditional video DiT architecture. Specifically:
% (i) Spatial memory is rendered into 2D condition maps and injected via a ControlNet-style conditioner (zero-initialized residual blocks) to modulate static geometry;
% (ii) Working memory is fused through frame-wise concatenation of recent video and condition tokens, ensuring per-frame alignment of dynamics and scene structure;
% (iii) Episodic memory is accessed via a dedicated historical cross-attention module, where current tokens query reference tokens from archived keyframes.

% \end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsubsection{A Posteriori Causal Management (The $U$ Module)}
% 补充一张图，对比在记忆管理的视角下，kv-cache，linear attention，SSMs之间的联系和区别

Update mechanisms are the a posteriori (reactive) managers of causality. After the "effect" ($G_t$) has been generated and encoded ($E_t$), the ``U'' module is responsible for analyzing this new "outcome" and integrating it into the memory state $M_t$ to form $M_{t+1}$.

This is the "learning" or "consolidation" phase of the cycle. If the analysis of the "effect" is insufficient (e.g., the ``U'' module simply appends data via a FIFO queue), the new state $M_{t+1}$ may become corrupted, redundant, or fail to capture the most important new information. Advanced ``U'' modules, therefore, modify the memory state by summarizing, consolidating, or strategically forgetting, ensuring that $M_{t+1}$ is an accurate and efficient representation of the new reality.

A natural way to realize this is through a compact latent state that is refreshed as the sequence advances. In MALT \cite{yu2025malt}, a learned memory vector (h) is refreshed with a Markovian rule ($h^n = f(h^{n-1}, z_0^n)$) using temporal attention layers designed for compression; the same network plays a dual role, acting as a denoiser during standard diffusion steps and, when triggered by the ($t=0$) input, as a memory encoder that writes into (h). Because the memory lives inside the Transformer blocks and is trained end to end, the update is part of normal inference rather than an external procedure. Empirically, this yields strong long-term stability with less error accumulation and robust length generalization, producing videos beyond 120 seconds even when trained only on short clips.

Another line of work uses state space models (SSMs) to advance the memory as a causal hidden state \cite{po2025long,oshima2024ssm}. The sequence is scanned with linear updates that keep the state size constant; computation is organized block-wise to avoid degradation from very long chains, and a small local frame-window attention is added to capture short-range dynamics that a pure SSM might miss. In this setting the SSM state is the memory: it is recurrently updated, then reused at later steps. The result is efficient long-context modeling with performance comparable to full-context causal attention on certain retrieval-style tasks, but at substantially lower computational cost.

A closely related architectural choice is to replace standard attention with block-wise causal linear attention so that memory evolves additively, as in SANA-Video \cite{chen2025sana}. Instead of storing a growing KV cache, the model accumulates key–value representations over time via linearized attention updates across temporal blocks. Functionally, this is a compact, cumulative state tracker that keeps memory usage fixed while video length increases. Like SSM-based designs, it achieves constant-size scaling during autoregressive generation and preserves quality comparable to full self-attention, but at significantly lower compute and memory cost; the cumulative KV update is built into the architecture and learned end to end, so no external memory management is required.


\cite{huang2024owl} adopt an external world model for updating the latent state. The system maintains a compact latent world state $s_t$ and, after each short clip is ``rendered'' (generated), calls a multimodal LLM to inspect $(s_t, o_t)$, summarize the newly observed ``world dynamics'' in natural language $d_t$, and then map $(s_t, d_t)$ to the next state $s_{t+1}$. The video diffusion model then takes $s_{t+1}$ together with a short-range visual cue (such as the last frame of the previous clip) as its condition for synthesizing the next clip, while the world model is responsible for tracking long-horizon semantics and causal structure. In our terminology, this instantiates the $U$ module as a separate world-state updater that operates in a higher-level symbolic space: memory is still revised a posteriori and in a causal fashion, but the update rule is implemented by an explicit controller that can be tuned and scaled without modifying the core video generator.

\cite{henschel2025streamingt2v} FIFO short-term window + Persistent anchor frame %待补充

\cite{wang2024loong} use last n frames as context for each generation step. %待补充

\cite{wu2025pack} use ``SemanticPack'' to retain a state token that evolves during the long-horizon generation process.
%%%%%%%%%%%%%%%%%%%%%%% paper summary %%%%%%%%%%%%%%%%%%%%%
% \begin{itemize}
%     \item \textbf{Malt~\cite{yu2025malt}:}
%     \textbf{What it does:}
%     MALT (Memory-Augmented Latent Transformers) addresses any-length video generation by introducing a memory vector $h$ to solve long-context understanding. This vector is recurrently updated ($h^n = f(h^{n-1}, z_0^n)$) segment-by-segment using novel temporal attention layers, allowing the model to compress long historical context. The model itself has a dual function: it acts as a denoiser for noisy inputs and as a memory encoder, with the role switched by the $t=0$ input. 
    
%     \textbf{Correspondence to the memory component:}
%     It corresponds to a memory update process, which functions as a recurrent, Markovian update strategy
    
%     \textbf{Effectiveness:}
%     MALT demonstrates strong long-term stability with less error accumulationand shows powerful length generalization, generating videos over 120 seconds long even when trained on short clips. 
    
%     \textbf{Coupling with the base model:}
%     This memory mechanism is coupled with the Transformer architecture, as it modifies the model's blocks and is \textbf{learned from data}.

%     \item \textbf{SSMs~\cite{po2025long}:}
%     \textbf{What it does:}
%     This method leverages State Space Models (SSMs) to process video sequences by performing a scan over the input and updating a hidden state in a causal and linear manner. To alleviate the degradation caused by long scan chains, the model adopts block-wise SSM computation. In addition, local frame window attention is introduced to capture short-term temporal dependencies that SSMs alone may struggle with.
    
%     \textbf{Correspondence to the memory component:}
%     The core SSM update mechanism directly corresponds to the memory state update process. As the sequence is processed, the state is recurrently updated, and this state is then reused as the memory input during subsequent generation steps.
    
%     \textbf{Effectiveness:}
%     By combining SSMs with local window attention, the model maintains memory with constant-size scaling, enabling efficient long-context modeling. It achieves performance comparable to full-context causal attention models in certain retrieval tasks, while requiring significantly lower computational cost.
    
%     \textbf{Coupling with the base model:}
%     The memory state is directly integrated into the model and is \textbf{learned end-to-end}, as the SSM parameters responsible for state updates are embedded within the model architecture itself.



%     \item \textbf{SANA-Video~\cite{chen2025sana}:}
%     \textbf{What it does:}
%     This approach replaces standard attention in video models with a \textbf{block-wise causal linear attention} mechanism. Instead of maintaining a growing key-value (KV) cache, it performs attention updates using linearized formulations that allow efficient computation across temporal blocks.
    
%     \textbf{Correspondence to the memory component:}
%     Causal linear attention naturally introduces an \textbf{additive memory update} structure: the KV representations are accumulated over time rather than stored as an ever-expanding list. This corresponds directly to a memory system where the memory state evolves through cumulative updates, enabling compact and efficient state tracking during sequence generation.
    
%     \textbf{Effectiveness:}
%     Similar to SSM-based models, this method maintains memory with \textbf{constant-size scaling} during autoregressive (AR) generation. As a result, it supports efficient modeling of long video contexts while preserving performance comparable to full self-attention architectures, but at significantly lower computational and memory cost.
    
%     \textbf{Coupling with the base model:}
%     The memory state is fully integrated into the network and \textbf{learned end-to-end}. The cumulative KV update mechanism is embedded directly within the model architecture, meaning the memory state evolves inherently during training and inference without requiring external memory management.

    

% \end{itemize}




\subsection{Explicit Geometry Memory}

Finally, it is worth noting a special category where the memory state $M_t$ itself has an explicit, structured representation, most notably as 3D geometry. 
This is orthogonal to the R/D/E/U mechanisms but fundamentally changes their operation. 
In this paradigm, $M_t$ is not an implicit latent vector or KV-cache, but an explicit 3D representation (e.g., a point cloud, mesh, or radiance field). 


==> legacy/6_evaluation.tex <==
\section{evaluation}\label{Applications}
Evaluating the progress from video generation towards true world simulation requires metrics and benchmarks that capture not only traditional visual quality but also \textbf{long-term coherence}, \textbf{memory usage}, and \textbf{latent state fidelity}. In this section, we discuss evaluation protocols from three complementary perspectives: \textit{Context Length}, \textit{Memory Consistency}, and \textit{State Dynamics}. Each perspective aligns with one of the core gaps identified earlier, ensuring that models are assessed on their ability to maintain extended narratives, remember and revisit scenes, and internalize the causal structure of the world.

\subsection{Long-Context Video Generation}\label{sec:eval_context}
\subsubsection{Challenges of Long Horizons} Traditional video metrics were developed for short clips and often fail to reflect performance on minute-long sequences. Fréchet Video Distance (FVD)~\cite{unterthiner2018fvd} and related set-level metrics remain standard for evaluating visual fidelity, but they are typically computed on 16 to 32-frame samples. As a result, FVD can mask issues that emerge only over longer horizons, such as scene drift or repetition. To stress-test models beyond their training context, recent works report performance as a function of video length. For instance, StreamingT2V~\cite{henschel2025streamingt2v} demonstrates coherent generation up to 2 minutes by incrementally extending context windows, and reports that naive baselines stagnate or collapse before reaching 600 frames. Similarly, SANA-Video~\cite{chen2025sana}, a linear attention-based diffusion model, showcases minute-long ($\sim$1800 frame) 720p videos while maintaining competitive FVD to shorter-video models, highlighting that specialized architectures can stretch generation length without severe quality degradation.
\subsubsection{Temporal Coherence Metrics} Because per-frame quality alone is insufficient for long videos, new metrics emphasize \textbf{temporal consistency} and logical progression. The Fréchet Video Motion Distance (FVMD) proposed by Han et al.~\cite{liu2024fvmd} focuses on motion smoothness and physical plausibility. By comparing velocity and acceleration distributions of generated vs. real videos, FVMD penalizes implausible motions that might not be evident in FVD. Other measures explicitly target flicker or alignment: e.g., Temporal Warping Error and Frame Consistency use optical flow to detect frame-to-frame distortions, while Long-term Identity Tracking checks if an object or character retains the same appearance across the video. These metrics often feed into comprehensive benchmark suites like VBench~\cite{huang2023vbench}, which dissects video quality into 16 fine-grained dimensions (e.g., background continuity, object permanence, character identity consistency). VBench and its successor VBench++~\cite{huang2024vbench++} combine automated detectors (for faces, objects, etc.) with pretrained encoders (e.g. CLIP and pose estimators) to quantify issues like “subject appearance change” or “unstable camera trajectories” that plague long sequences. Notably, one dimension of VBench explicitly measures whether a generated subject’s identity remains consistent throughout the video – a critical aspect of long-context fidelity.

\subsubsection{Benchmarks for Temporal Reasoning} Beyond generic metrics, specialized benchmarks test a model’s understanding of extended time-lapse events. \textbf{ChronoMagic-Bench}~\cite{yuan2024chronomagic} evaluates text-to-video models on time-lapse scenarios (e.g., “a seed grows into a tree”), requiring the correct ordering of semantic stages. Even if a model renders each frame realistically, ChronoMagic will give it a low score when the semantic stages appear in the wrong temporal order. By performing manual and automatic checks on dozens of temporal logic tasks, ChronoMagic has revealed that many state-of-the-art models still struggle with monotonic, irreversible changes (metamorphosis or aging) over long durations. High performance on such benchmarks indicates an implicit grasp of timeline and causal progression, moving beyond short-term coherence.

\subsubsection{Efficiency and Scalability} An often overlooked aspect of context evaluation is computational scalability. Models that naively attend to all past frames suffer \textbf{quadratic memory growth}, limiting practical video length. Therefore, efficiency metrics are increasingly reported alongside quality. For instance, SSM-based methods (State-Space Models) like Oshima et al.~\cite{oshima2024ssm} show memory usage growing linearly with sequence length (vs. quadratically for Transformers) while maintaining similar FVD. SANA-Video achieves a \textit{constant memory cost} per additional block of frames by compressing context into a fixed-size state~\cite{chen2025sana}, enabling it to generate 60-second videos on a single GPU. Thus, evaluation of “context handling” includes not only whether a model can \textit{theoretically} generate long videos, but whether it can do so efficiently and without quality collapse. Metrics like \textbf{generation speed (frames per second) and peak memory footprint} are reported in recent works~\cite{chen2025sana, henschel2025streamingt2v} to compare the practical long-video capabilities of different architectures.

\subsection{Memory and Consistency}\label{sec:eval_memory}

\subsubsection{Object Permanence and Scene Re-visitation} A hallmark of a true world simulator is the ability to remember and maintain scene details over time. Evaluation protocols have been proposed to directly test \textbf{object permanence}: does an object that leaves the camera’s view reappear unchanged when it comes back? One approach is the \textbf{re-visitation consistency test}~\cite{xiao2025worldmem}. Here, a camera trajectory is designed such that it returns to a previously seen location after a long gap (for example, a first-person video wanders through a virtual house and eventually comes back to the starting room). The first frame and the final frame (upon returning) are then compared for consistency. Quantitatively, this can be measured via high PSNR and low LPIPS between the two frames (for pixel-level consistency), or via a “reconstruction FID (rFID)”~\cite{heusel2018rFID} that computes Fréchet Distance between features of the initial vs. revisited scene. WorldMem’s evaluation on a Minecraft simulator explicitly uses this protocol: it reports that without memory augmentation, generation quality suffers a sharp divergence once the context window is exceeded, leading to a low PSNR and high rFID when the agent returns to the same spot. With a memory bank, however, the model can “recall” the scene, yielding final frames nearly identical to the initial ones. This kind of loop consistency test is becoming a standard for long-term video models.

\subsubsection{Memory Capacity Probing} Some evaluation tasks borrow inspiration from reinforcement learning benchmarks to probe how much information a generative model’s “memory” can hold. For instance, the \textbf{Memory Maze} challenge~\cite{pasukonis2022maze} places an agent in a 3D maze and requires long-term remembering of the maze layout to navigate successfully. In a generative context, a similar test is to have the model generate an agent’s trajectory through a labyrinth with the correct sequence of turns leading back to the start. The recent \textbf{VR-Bench (Visual Reasoning Benchmark)} by Guo et al.~\cite{yang2025vrbench} incorporates maze-solving tasks precisely for this purpose. Video models must generate a frame-by-frame plan from start to finish, effectively “remembering” dead-ends and already-visited corridors to avoid them later. Performance is measured by path accuracy (did the generated trajectory reach the goal without errors?) and rule compliance (e.g., avoiding walls or forbidden zones). Notably, fine-tuned video diffusion models have shown surprising competency on these tasks, outperforming text-only planners by leveraging the visual memory of the maze. This indicates that, even without an explicit internal state variable, large video models can internalize a maze’s layout implicitly in their frame history. Going forward, one can imagine even more targeted memory probes: e.g., tasks where a number or symbol is shown early in the video and must reappear correctly much later. Such evaluations would force the model to demonstrate a longer memory span than current context windows allow.

\subsubsection{Operation-Level Memory Metrics}
Recent work on hallucination evaluation for long-term memory systems, such as \textbf{HaluMem}~\cite{chen2025halumem}, moves beyond end-to-end QA and explicitly evaluates individual memory operations (extraction, updating, and usage). 
Although originally designed for textual agents, the same decomposition is natural for Generative World Models: a ``memory point'' can correspond to an object slot, a 3D scene token, or any structured fact that should be written into the world state $S_t$.

For memory extraction, we assume a set of ground-truth memory facts 
$M^{\text{gt}} = \{m_i\}_{i=1}^{G}$ that should be stored (e.g., object identity, attributes, or scene layout), 
and a set of memories actually written by the model 
$\hat{M} = \{\hat{m}_j\}_{j=1}^{E}$. 
Here $G = |M^{\text{gt}}|$ is the number of ground-truth facts, and $E = |\hat{M}|$ is the number of entries the model puts into its memory. 
Each fact $m_i$ has an importance weight $a_i \ge 0$ and a correctness score $c_i \in \{0, 0.5, 1\}$ (incorrect / partially correct / correct). 
Let $G_{\text{hit}}$ be the number of ground-truth facts that are stored with non-zero correctness (i.e., $c_i > 0$). 
We also consider a set of $D$ distractor facts that should \emph{not} be stored; among them, $D_{\text{store}}$ are wrongly written into memory. 
We can then define
\begin{equation}
\mathrm{MemRec} = \frac{G_{\text{hit}}}{G},
\end{equation}
\begin{equation}
\mathrm{WMemRec} = \frac{\sum_{i=1}^{G} a_i c_i}{\sum_{i=1}^{G} a_i},
\end{equation}
\begin{equation}
\mathrm{MemAcc} = \frac{G_{\text{hit}}}{E},
\end{equation}
\begin{equation}
\mathrm{MemResist} = 1 - \frac{D_{\text{store}}}{D}.
\end{equation}
Here, $\mathrm{MemRec}$ and $\mathrm{WMemRec}$ measure how many important facts are successfully written into memory (anti-amnesia), $\mathrm{MemAcc}$ measures how many stored memories are actually correct (anti-hallucination), and $\mathrm{MemResist}$ (resistance to false memories) measures how often distractors are correctly ignored.
In a video setting, each $m_i$ can encode object identity, attributes, pose, or scene layout that should persist across long sequences.


For memory \emph{updating}, we further assume a set of ground-truth updates 
$U^{\text{gt}} = \{u_k\}_{k=1}^{U}$ that describe how stored facts should change over time. 
Each update $u_k$ operates on some memory fact (e.g., a door switching from closed to open, an object being deleted, an agent gaining or losing an item, a camera pose being changed). 
Here $U = |U^{\text{gt}}|$ is the number of updates that \emph{should} happen according to the reference world trajectory.

Given a model with its own memory state, we can classify its behaviour with respect to these updates into three disjoint types:
(1) \emph{correct updates}, where the model applies exactly the intended change;
(2) \emph{hallucinated updates}, where the model applies an incorrect or spurious change (e.g., changing the wrong attribute, or updating a fact that should stay unchanged);
and (3) \emph{missed updates}, where the model fails to apply an update that should happen. 
Let $U_{\text{corr}}$, $U_{\text{hall}}$, and $U_{\text{miss}}$ be the counts of these three cases, respectively. 
The following metrics summarize update quality:
\begin{equation}
\mathrm{UpdAcc} = \frac{U_{\text{corr}}}{U},
\end{equation}
\begin{equation}
\mathrm{UpdHalluc} = \frac{U_{\text{hall}}}{U},
\end{equation}
\begin{equation}
\mathrm{UpdOmit} = \frac{U_{\text{miss}}}{U}.
\end{equation}
Here, $\mathrm{UpdAcc}$ captures how often the model applies the correct world-state change, while $\mathrm{UpdHalluc}$ and $\mathrm{UpdOmit}$ explicitly quantify two failure modes: hallucinating non-existent changes and silently ignoring real ones. 
In GWM-style video models, these measures directly test whether the memory state $S_t$ correctly tracks persistent changes in the simulated world (e.g., object removal, door state, inventory updates), instead of drifting away from the underlying world dynamics.



\subsubsection{World Consistency Score (WCS).} Rakheja et al. introduced WCS~\cite{rakheja2025worldconsistencyscore}, a unified metric explicitly targeting the internal world consistency of generated videos. WCS is comprehensive: it evaluates whether the model’s portrayal of the world obeys logical constraints such as \textit{object permanence}, \textit{spatial coherence}, and \textit{causal compliance}. For example, WCS will penalize a video in which an object randomly disappears (violating permanence) or where scene layout inexplicably changes between cuts (violating spatial consistency). Internally, the metric decomposes these checks using computer vision techniques—tracking objects across frames, analyzing pairwise object relationships, and ensuring that cause-effect relations (e.g. “a ball pushed off a table should fall”) are not broken. A high WCS indicates that the video model behaves more like a persistent world simulator rather than a series of disjoint image generators. Unlike FVD which is insensitive to such internal coherence, WCS directly scores the \textbf{consistency of the simulated world} and has been proposed as a better indicator of memory-integrating improvements.

\subsubsection{Identity and Detail Consistency} Another facet of memory in video generation is maintaining consistent details for characters, objects, and scene attributes. Benchmarks often use pre-trained recognition models to quantify this. For example, character consistency can be evaluated by running a face recognition network on each frame of a generated video and ensuring all embeddings match the same identity~\cite{huang2023vbench}. A drop in similarity would reveal the model “forgot” the character’s appearance mid-video (a common failure mode without memory mechanisms). Similarly, for text-guided videos, prompt adherence over time is evaluated by computing CLIP similarity between each frame and the textual prompt~\cite{huang2024vbench++}. A declining prompt-frame similarity indicates the model is drifting off-topic as time progresses, which memory-augmented models aim to prevent~\cite{yu2025context}. In sum, by monitoring semantic consistency (via CLIP) and low-level consistency (via pixel differences) across lengthy generations, researchers can quantitatively demonstrate the benefits of proposed memory mechanisms. For instance, retrieval-based memory (bringing back an early frame as reference) should measurably improve identity consistency scores and reduce abrupt changes in object color or shape, compared to a baseline without memory augmentation.

\subsection{Latent State and Dynamics}\label{sec:eval_state}
Evaluating the latent \textbf{state} of a generative model is much subtler, because the state is an internal variable rather than a directly observed quantity. Nonetheless, several proxy evaluations shed light on whether a model’s internal dynamics truly capture the underlying world physics and causal structure:

\subsubsection{Multi-Step Forecasting and Rollouts} A classic evaluation in model-based learning is to let the model \emph{imagine} many steps into the future and compare the rollout against reality~\cite{hafner2019learning}. In video generation, we analogously assess how well a model can continue a sequence without “resetting” or diverging. This can be done by initializing the model with a context of real frames, then letting it predict dozens of future frames in a closed loop. The generated rollout is then compared to the ground-truth continuation (if available) using metrics like MSE per frame or video-FID over the sequence. A model with a robust latent world state will maintain accuracy deeper into the rollout, whereas a purely observation-driven model may quickly drift off (since it has no true memory of dynamics, only correlations). For example, researchers have shown that adding a recurrent state (e.g., an LSTM or SSM layer) to a video diffuser significantly delays the point at which generations become incoherent when extended to 2-3$\times$ the training sequence length~\cite{chen2025recurrent}. In one such study, a state-augmented model was able to continue a complex motion 50\% longer (in terms of frames) before entropy in the predictions sharply increased, compared to a transformer without recurrence. Such experiments quantitatively validate that an explicit state $S_t$ helps stabilize long-term dynamics.

\subsubsection{Latent Probing and Disentanglement} Another angle is to inspect the learned latent state variables directly. While video models don’t produce an explicit $S_t$ for output, methods that incorporate a hidden state (e.g. RNN hidden vector, state-space features, or test-time trained parameters) can be probed to see what they represent. One common technique is to train simple linear predictors or classifiers on the latent to predict known properties of the frame (such as camera angle, object count, or agent position)~\cite{hafner2019learning, wu2023daydreamer}. If the latent truly encodes a compact world state, it should be highly predictive of these underlying factors. For example, Wu et al.~\cite{wu2025pack} introduced a packing-based world model and showed that its hidden state could accurately ($\geq$90\%) classify which specific environment (out of a set of $N$ possible maze layouts) the agent was in, after a brief observation. This suggests the model’s state had effectively captured a map of the environment. 

% Similarly, in \textbf{3D scene generation} scenarios, models like VMem~\cite{li2025vmem} use an explicit 3D latent (such as a NeRF or voxel grid) as state; evaluation then measures reconstruction error of rendered novel views to ensure the latent is an accurate scene representation. High-fidelity novel view synthesis implies the latent state $S_t$ stores sufficient geometric information about the world.

\subsubsection{Intervention and Control Accuracy} A definitive test of a learned world model is whether it responds correctly to \textbf{interventions} (i.e., action inputs). Recent action-conditioned video generation frameworks introduce control signals at each time step, opening the door to evaluating causal fidelity. For instance, GameGAN-style benchmarks~\cite{yu2025gamefactory, he2025matrix} feed a sequence of game controller actions into the model and require it to generate the corresponding gameplay video. Evaluation can then measure \textit{action alignment}: did the model’s state produce the correct outcome for each input action? Metrics include success rate (percentage of actions leading to the expected visual result) or trajectory accuracy (distance between the model-generated character position and the ground-truth position after a given action sequence)~\cite{yu2025gamefactory}. High alignment indicates the model’s latent state correctly encodes the game’s transition dynamics (e.g., pressing “left” actually moves the character left in the generated frames). Diffusion models augmented with structure (such as pose tokens or physics engines) have achieved impressively high action alignment in driving scenarios and 2D games~\cite{valevski2024diffusion}, whereas vanilla text-to-video models often ignore fine-grained control inputs (due to their bias toward global context $C_{global}$). Thus, by evaluating per-step control fidelity, researchers can infer whether the model is using an internal state that transitions properly under actions $A_t$, as a true world model should.

\subsubsection{Causal Consistency and Physics}
Lastly, the power of a Generative World Model is judged by how well its imagined sequences obey physical and causal laws. Beyond the generic video metrics discussed above, recent work has started to build dedicated \emph{physics benchmarks} for generative video models. Physics-IQ~\cite{motamed2025physiq} proposes a controlled continuation protocol on real-world videos: a model sees a short conditioning clip (or a single ``switch frame'') and must generate the next few seconds in scenarios that require understanding solid mechanics, fluid dynamics, optics, thermodynamics, and magnetism. Physical correctness is then quantified by four complementary metrics—Spatial IoU (where action happens), Spatiotemporal IoU (where and when action happens), Weighted Spatial IoU (where and how much action happens), and MSE (how the action unfolds)—which are aggregated into a normalized Physics-IQ score, with pairs of real videos defining the 100\% ``physical variance'' upper bound~\cite{motamed2025physiq}. Across a range of state-of-the-art models, scores remain far below this ceiling, highlighting a clear gap between visual realism and genuine physical understanding.

In parallel, PhysBench~\cite{wang2025physbench} evaluates physical reasoning from an interleaved video–image–text perspective. It frames physical world understanding as multiple-choice QA over 10k+ prompts spanning object properties (mass, elasticity, temperature), object relations (support, collision, contact), scene understanding (lighting, viewpoint, materials), and physics-based dynamics (collisions, throwing, fluid flow, explosions). Each question may include short videos, keyframes, and textual descriptions, and models are scored simply by answer accuracy. While PhysBench does not require the model to \emph{generate} future frames, it directly probes whether the internal state (or the perception module in a GWM-style system) encodes enough physical structure to support downstream reasoning about ``what will happen'' or ``which outcome is physically plausible''.

Beyond these formal benchmarks, researchers also use more open-ended \textbf{challenge tasks} as qualitative stress tests. For example, Veo-3 has been demonstrated on zero-shot tasks such as ``navigate a ball through a maze and then recognize a symmetry'' within a single generated video, which implicitly requires modeling rolling dynamics and maze layout over time. Similarly, one can design \emph{counterfactual consistency} tests: generate two videos that are identical up to a certain frame and then apply different actions (e.g., in one branch a vase is dropped, in the other it is placed gently). A robust world-model-like generator should produce diverging outcomes after the intervention (the vase shatters vs.\ remains intact) while keeping all irrelevant aspects aligned. If the model instead produces averaged outcomes or drifts in unrelated details, this indicates that the latent state does not cleanly encode causal structure but mainly captures superficial correlations.

Finally, physics-aware generative models like Lumi\`ere~\cite{BarTal2024LumiereAS} provide case studies for \emph{conditional} physical evaluation. In controlled setups, evaluators vary initial conditions (object mass, push force, friction, etc.) and inspect whether the resulting motions change in the expected way while preserving other attributes of the scene. Together, benchmarks such as Physics-IQ and PhysBench, counterfactual protocols, and controlled perturbation tests begin to ground the abstract ``state'' of GWMs in concrete physical behavior, offering a path toward measuring whether a video generator is merely rendering plausible pixels or actually simulating a coherent physical world.


==> legacy/6_evaluation_v2.tex <==



%4 个方向（State Consistency / Physical Dynamics / Latent Probing / Computational Scalability）
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{main/figures/evaluation_cropped.pdf}
    %\vspace{-0.2in}
\caption{\textbf{Taxonomy of Evaluation Methodologies for World Models.} We categorize evaluation protocols into two distinct paradigms: \textbf{Open-Loop} and \textbf{Closed-Loop}. Open-Loop Evaluation assesses the intrinsic quality of the simulation in a passive setting, focusing on State Consistency (e.g., memory capacity tasks), Physical Dynamics (e.g., causal reasoning), and Real-Time Generation efficiency. Conversely, Closed-Loop Evaluation tests the model's ``embodied utility'' as an interactive environment, measuring success via task completion metrics and interaction controllability.}
    \label{fig-method}
    \vspace{-0.2in}
\end{figure*}


\section{Evaluation}\label{Applications}
Evaluating the transition from video generation to true world simulation requires a fundamental shift in benchmarking protocols. 
While classical metrics (e.g., FVD, IS) focus on the visual fidelity of passive video consumption, a functional world model must support both long-horizon coherent generation and active decision-making. 
Accordingly, we categorize evaluation methodologies into two distinct paradigms: 
\textbf{Open-Loop Evaluation}, which assesses the generative quality, physical consistency, and computational efficiency of the model in a passive observation setting; 
and \textbf{Closed-Loop Evaluation}, which tests the model's ``embodied utility'' by deploying it as an interactive simulator for an agent.

In Sections~\ref{sec:eval_state_consistency} to~\ref{sec:eval_scalability}, we first organize the \textbf{Open-Loop} protocols along three critical axes: 
\emph{(i) state consistency}, \emph{(ii) physical dynamics}, and \emph{(iii) Real-time Generation}. 
These axes form a stress test for whether a model behaves as a world simulation system. 
Finally, in Section~\ref{sec:eval_closed_loop}, we discuss the \textbf{Closed-Loop} paradigm, where the ultimate criterion is not how good the frames look, but whether an agent can successfully plan and act within the hallucinated world.

\subsection{State Consistency in Long-Context Video}\label{sec:eval_state_consistency}

\subsubsection{Long-Horizon Coherence}
Traditional video metrics were developed for short clips and often fail to reflect performance on minute-long sequences. Fréchet Video Distance (FVD)~\cite{unterthiner2018fvd} and related set-level metrics remain the standard for evaluating visual fidelity, but they are typically computed on short 16 to 32-frame samples. As a result, FVD can mask issues that emerge only over longer horizons, such as scene drift, object identity changes, or repetition. To stress-test models beyond their training context, recent works report performance as a function of video length. For instance, StreamingT2V~\cite{henschel2025streamingt2v} demonstrates coherent generation up to 2 minutes by incrementally extending context windows, reporting that naive baselines stagnate or collapse before reaching 600 frames. Similarly, SANA-Video~\cite{chen2025sana} showcases minute-long ($\sim$1800 frame) videos while maintaining competitive FVD, highlighting that specialized architectures can stretch generation length without severe quality degradation.

Because per-frame quality alone is insufficient for long videos, newer evaluation protocols emphasize \textbf{temporal consistency} and logical progression. The Fréchet Video Motion Distance (FVMD) proposed by Han et al.~\cite{liu2024fvmd} focuses on motion smoothness and physical plausibility. By comparing velocity and acceleration distributions of generated vs.\ real videos, FVMD penalizes implausible motions that might not be evident in standard FVD. Other measures explicitly target flicker or alignment: e.g., Temporal Warping Error and Frame Consistency use optical flow to detect frame-to-frame distortions.

These metrics often feed into comprehensive benchmark suites like VBench~\cite{huang2023vbench}, which dissects video quality into 16 fine-grained dimensions (e.g., background continuity, object permanence, character identity consistency). VBench and its successor VBench++~\cite{huang2024vbench++} combine automated detectors with pretrained encoders (e.g.\ CLIP and pose estimators) to quantify issues like “subject appearance change” or “unstable camera trajectories” that plague long sequences. Notably, one dimension of VBench explicitly measures whether a generated subject’s identity remains consistent throughout the video, a critical aspect of long-context fidelity where models often "forget" character appearance mid-video.

\subsubsection{Memory Capacity Tasks}
While coherence metrics measure stability, memory capacity tasks evaluate a model's ability to maintain a persistent internal state, ensuring that the simulated world remains logically valid over time and across viewpoints.


\textbf{Scene Re-visitation and rFID}
A hallmark of a true world simulator is the ability to remember and maintain scene details over time. Evaluation protocols have been proposed to directly test \textbf{object permanence} via the \textit{re-visitation consistency test}~\cite{xiao2025worldmem}. In this protocol, a camera trajectory is designed to return to a previously seen location after a long temporal gap (e.g., a first-person view wandering through a virtual house and returning to the starting room). The initial frame and the final frame are compared for consistency. Quantitatively, this is measured via high PSNR and low LPIPS for pixel-level consistency, or via a “reconstruction FID (rFID)”~\cite{heusel2018rFID} that computes the Fréchet Distance between features of the initial vs.\ revisited scene. WorldMem’s evaluation on a Minecraft simulator reports that without memory augmentation, generation quality suffers a sharp divergence once the context window is exceeded, leading to a high rFID when the agent returns to the same spot.

\textbf{World Consistency Score (WCS)}~\cite{rakheja2025worldconsistencyscore} Moving beyond simple pixel-level alignment, the World Consistency Score (WCS) represents a unified, no-reference framework designed to evaluate the physical plausibility and logical integrity of generated videos. Treating the video as a self-contained environment, WCS quantifies internal coherence through a learned combination of four interpretable sub-metrics assessed via standard computer vision tools. Specifically, it computes Object Permanence by utilizing object trackers to measure the fraction of frames entities persist, ensuring they do not inexplicably vanish without occlusion ; evaluates Relation Stability by monitoring pairwise spatial configurations, such as relative centroid distances, to detect erratic structural violations like floating objects ; measures Causal Compliance by identifying unexplained motion onsets or missing physical reactions via event analysis and trajectory acceleration checks ; and calculates a Flicker Penalty using optical flow to isolate and penalize unnatural high-frequency temporal noise distinct from genuine motion. By aggregating these components using weights regressed against human preference data, WCS aligns with human perceptions of reality, effectively penalizing the "hallucinations" that disrupt the illusion of a persistent, physically grounded world.

\textbf{Navigation and Maze Tasks}
Finally, some evaluation tasks borrow inspiration from reinforcement learning to probe the capacity of a generative model’s “memory.” The Memory Mazechallenge~\cite{pasukonis2022maze} requires an agent to remember a 3D maze layout to navigate successfully. In a generative context, the VR-Bench (Visual Reasoning Benchmark)~\cite{yang2025vrbench} incorporates maze-solving tasks where video models must generate a frame-by-frame plan from start to finish. To succeed, the model must effectively “remember” dead-ends and already-visited corridors. Performance is measured by path accuracy and rule compliance. Recent findings indicate that video diffusion models can outperform text-only planners on these tasks, suggesting that large video models can internalize complex spatial states implicitly within their frame history.

\subsection{Physical Dynamics and Causal Structure}\label{sec:eval_physics}

\subsubsection{Temporal Reasoning and Time-Lapse Benchmarks}
World simulators should not only keep states consistent but also evolve them in a logically ordered way. 
Specialized benchmarks test a model’s understanding of extended time-lapse events. 
\textbf{ChronoMagic-Bench}~\cite{yuan2024chronomagic} evaluates text-to-video models on time-lapse scenarios (e.g., “a seed grows into a tree”), requiring the correct ordering of semantic stages. 
Even if a model renders each frame realistically, ChronoMagic will give it a low score when the semantic stages appear in the wrong temporal order. 
By performing manual and automatic checks on dozens of temporal logic tasks, ChronoMagic has revealed that many state-of-the-art models still struggle with monotonic, irreversible changes (metamorphosis or aging) over long durations. 
High performance on such benchmarks indicates an implicit grasp of timeline and causal progression, moving beyond short-term coherence.


\subsubsection{Causal Consistency and Physics Benchmarks}
Ultimately, the power of a Generative World Model is judged by how well its imagined sequences obey physical and causal laws. 
Beyond the generic video metrics discussed above, recent work has started to build dedicated \emph{physics benchmarks} for generative video models. 
Physics-IQ~\cite{motamed2025physiq} proposes a controlled continuation protocol on real-world videos: a model sees a short conditioning clip (or a single ``switch frame'') and must generate the next few seconds in scenarios that require understanding solid mechanics, fluid dynamics, optics, thermodynamics, and magnetism. 
Physical correctness is then quantified by four complementary metrics, Spatial IoU (where action happens), Spatiotemporal IoU (where and when action happens), Weighted Spatial IoU (where and how much action happens), and MSE (how the action unfolds), which are aggregated into a normalized Physics-IQ score, with pairs of real videos defining the 100\% ``physical variance'' upper bound~\cite{motamed2025physiq}. 
Across a range of state-of-the-art models, scores remain far below this ceiling, highlighting a clear gap between visual realism and genuine physical understanding.


Beyond these formal benchmarks, researchers also use more open-ended \textbf{challenge tasks} as qualitative stress tests. 
For example, Veo-3 has been demonstrated on zero-shot tasks such as “navigate a ball through a maze and then recognize a symmetry” within a single generated video, which implicitly requires modeling rolling dynamics and maze layout over time. 
Similarly, one can design \emph{counterfactual consistency} tests: generate two videos that are identical up to a certain frame and then apply different actions (e.g., in one branch a vase is dropped, in the other it is placed gently). 
A robust world-model-like generator should produce diverging outcomes after the intervention (the vase shatters vs.\ remains intact) while keeping all irrelevant aspects aligned. 
If the model instead produces averaged outcomes or drifts in unrelated details, this indicates that the latent state does not cleanly encode causal structure but mainly captures superficial correlations.

Finally, physics-aware generative models like Lumi\`ere~\cite{BarTal2024LumiereAS} provide case studies for \emph{conditional} physical evaluation. 
In controlled setups, evaluators vary initial conditions (object mass, push force, friction, etc.) and inspect whether the resulting motions change in the expected way while preserving other attributes of the scene. 
Together, benchmarks such as Physics-IQ, counterfactual protocols, and controlled perturbation tests begin to ground the abstract ``state" of GWMs in concrete physical behavior, offering a path toward measuring whether a video generator is merely rendering plausible pixels or actually simulating a coherent physical world.

\subsection{Computational Scalability and Real-Time Throughput}
\label{sec:eval_scalability}

Finally, evaluating a model's potential as a real-time world simulator requires benchmarking its computational scalability alongside visual quality. 
The core assessment focuses on the stability of inference costs as the video length $L$ grows; while standard attention mechanisms suffer from quadratic complexity ($O(L^2)$ FLOPs), viable simulators must demonstrate \textbf{constant amortized compute} ($O(1)$) per new frame to support infinite rollouts. 
Practically, this is measured via the \textbf{Real-Time Factor (RTF)}, calculated as the ratio of generation time to playback duration, where an $\text{RTF} \leq 1.0$ indicates the system is fast enough for live interaction. 
A rigorous evaluation profiles the instantaneous generation throughput (FPS) over extended durations to detect ``latency drift,'' ensuring that architectures like SANA-Video~\cite{chen2025sana} or SSMs~\cite{oshima2024ssm} maintain consistent speed regardless of the accumulated historical context.


% ------------------------------------------------------------------
% New Closed-Loop Section
% ------------------------------------------------------------------
\subsection{The Closed-Loop Interaction Paradigm}\label{sec:eval_closed_loop}

Open-loop metrics quantify passive plausibility, but they do not ensure that a generated world is usable for planning and control. 
Closed-loop evaluation therefore treats the world model as an interactive environment: an embodied policy selects actions, the model returns the next observation, and we score whether the resulting action--observation loop supports task completion for the right reasons (i.e., correct affordances, contacts, and causal responses).


\noindent\textbf{Task-Level Embodied Utility.}
Closed-loop evaluation asks whether an embodied agent can complete tasks using only interactions inside the generated world. A common protocol fixes a policy, runs it for many episodes, and measures \textbf{Success Rate (SR)} as the fraction of episodes that satisfy a task-defined success condition (e.g., reaching within an $\epsilon$-radius of a goal for navigation, or meeting a terminal predicate for manipulation such as “object in container,” “door opened beyond a threshold,” or “switch toggled”). Because SR does not distinguish efficient solutions from “lucky wandering,” \textbf{Success weighted by Path Length (SPL)} is often used to down-weight successes that require substantially longer paths (or more steps) than an oracle shortest route computed in a reference environment (e.g., from a ground-truth map/MDP or an optimal planner in the true simulator). When an explicit reward is available, studies also use \textbf{average return} in model rollouts and \textbf{normalized regret} relative to evaluating the same policy under the same initial conditions in the real environment, isolating how model-induced interaction errors degrade planning performance.


\noindent\textbf{Interaction Diagnostics.}
While utility metrics measure task completion, diagnostic metrics aim to isolate the root cause of failures, distinguishing between deficient planning and inaccurate simulation dynamics. We employ \textbf{controllability} as a primary diagnostic to quantify the alignment between the model's predictions and physical reality. Formally, we define:
\begin{equation}
\label{eq:controllability}
\mathrm{Ctrl}(\mathbf{a}_{1:T})
\;=\;
\exp\!\Big(
-\lambda \cdot \mathrm{LPIPS}\big(
\hat{\mathbf{o}}_{1:T}(\mathbf{a}_{1:T}),
\mathbf{o}^{\star}_{1:T}(\mathbf{a}_{1:T})
\big)
\Big).
\end{equation}
In this formulation, $\mathbf{a}_{1:T}$ represents the control sequence applied over a horizon $T$. The metric fundamentally assesses the divergence between the model's generated rollout $\hat{\mathbf{o}}_{1:T}$ and the actual ground-truth trajectory $\mathbf{o}^{\star}_{1:T}$ when both are conditioned on these identical actions. The LPIPS term serves as a perceptual distance penalty, which is then mapped via the exponential function into a normalized similarity score in $(0, 1]$. The hyperparameter $\lambda > 0$ governs the sensitivity of this metric, controlling how sharply the score decays in response to visual or physical deviations from reality.









==> legacy/close_loop_vs_open_loop.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Comparison of Generative Paradigms.}
World Simulators bridge the gap by retaining the data-driven scalability of video generation 
while adopting the state-centric dynamics of world models.}
\label{tab:paradigm_comparison}

\renewcommand{\arraystretch}{1.4}
\small

\begin{tabular}{p{2.8cm} p{2.5cm} p{2.5cm} p{3cm} p{4.8cm}}
\toprule
\textbf{System Paradigm} &
\textbf{Mode} &
\textbf{State} &
\textbf{Formulation} &
\textbf{Pros (+) \& Cons (-)} \\
\midrule

Video Model &
Open-loop &
Stateless &
$O_{1:t} \xrightarrow{} O_{t+1}$ &
\textcolor{red}{-} Non-persistent context \newline
\textcolor{red}{-} Passive learning (correlation) \newline
\textcolor{green}{+} Massive data scalability \\

\midrule

World Simulator  &
Open-loop &
Explicit state &
$S_{t} \rightarrow S_{t+1}$; \newline
$S\rightarrow O$ &
\textcolor{green}{+} Persistent context \newline
\textcolor{green}{+} Robust control capability \\

\midrule

World Model &
Closed-loop &
Explicit state &
$S_{t} \rightarrow S_{t+1}$; \newline
$S \leftrightarrow O$; \newline
$S \rightarrow A$&
\textcolor{green}{+} Active learning (causality) \newline
\textcolor{red}{-} Limited data scalability \\

\bottomrule
\end{tabular}
\end{table*}



==> legacy/training_paradigm.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Dichotomy of Learning Paradigms: Open-Loop vs. Closed-Loop.} 
We contrast the \textit{Visual Modeling} paradigm (dominant in Video Generation) with the \textit{Task-Driven} paradigm (dominant in MBRL). 
Video models leverage the scalability of open-loop learning to acquire broad physical commonsense, whereas traditional world models rely on closed-loop interaction to master specific causal dynamics.}
\label{tab:open_vs_closed_loop}
\renewcommand{\arraystretch}{1.4} 
\setlength{\tabcolsep}{6pt} 

\begin{tabularx}{\linewidth}{@{} l X X @{}}
\toprule
\textbf{Dimension} & \textbf{Open-Loop / Visual-Driven} & \textbf{Closed-Loop / Task-Driven} \\ 
\midrule

\textbf{Primary Agent} & 
\textbf{Video Generation Models} (e.g., Sora~\cite{openai2024sora}, Kling~\cite{kuaishou2024klingai}) & 
\textbf{Embodied Agents} (e.g., Dreamer~\cite{hafner2019learning}, Robots) \\ 

\textbf{Data Regime} & 
\textbf{Passive Observation} \newline (Web-scale, offline, diverse video data) & 
\textbf{Active Interaction} \newline (On-policy, online, environment-specific experience) \\ 

\textbf{Optimization Goal} & 
\textbf{Fidelity} (Minimizing Prediction Error) \newline $\mathcal{L} = \| \hat{O}_{t+1} - O_{t+1} \|$ & 
\textbf{Utility} (Maximizing Cumulative Reward) \newline $J = \mathbb{E}[\sum R_t]$ \\ 

\textbf{Causality Type} & 
\textbf{Correlational} \newline Learns "what follows what" (visual statistics). Vulnerable to \textit{Causal Confusion}. & 
\textbf{Interventional} \newline Learns "what happens if I do $A$" (counterfactuals). Verified by physical feedback. \\ 

\textbf{Strengths} & 
$\bullet$ \textbf{Scalability:} Unlimited internet data. \newline
$\bullet$ \textbf{Generalization:} Captures broad world physics. & 
$\bullet$ \textbf{Precision:} Grounded in physical reality. \newline
$\bullet$ \textbf{Robustness:} Self-correcting via feedback. \\ 

\textbf{Weaknesses} & 
$\bullet$ \textbf{Hallucination:} Lack of grounding leads to drift. \newline
$\bullet$ \textbf{Passive:} Cannot verify hypothesis via action. & 
$\bullet$ \textbf{Inefficiency:} High sample complexity. \newline
$\bullet$ \textbf{Safety Risks:} Exploration can be dangerous. \\ 

\bottomrule
\end{tabularx}
\end{table*}
